Understanding Video Transformers for Segmentation: A Survey of Application and Interpretability

Video segmentation encompasses a wide range of categories of problem formulation, e.g., object, scene, actor-action and multimodal video segmentation, for delineating task-specific scene components with pixel-level masks. Recently, approaches in this research area shifted from concentrating on ConvNet-based to transformer-based models. In addition, various interpretability approaches have appeared for transformer models and video temporal dynamics, motivated by the growing interest in basic scientific understanding, model diagnostics and societal implications of real-world deployment. Previous surveys mainly focused on ConvNet models on a subset of video segmentation tasks or transformers for classification tasks. Moreover, component-wise discussion of transformer-based video segmentation models has not yet received due focus. In addition, previous reviews of interpretability methods focused on transformers for classification, while analysis of video temporal dynamics modelling capabilities of video models received less attention. In this survey, we address the above with a thorough discussion of various categories of video segmentation, a component-wise discussion of the state-of-the-art transformer-based models, and a review of related interpretability methods. We first present an introduction to the different video segmentation task categories, their objectives, specific challenges and benchmark datasets. Next, we provide a component-wise review of recent transformer-based models and document the state of the art on different video segmentation tasks. Subsequently, we discuss post-hoc and ante-hoc interpretability methods for transformer models and interpretability methods for understanding the role of the temporal dimension in video models. Finally, we conclude our discussion with future research directions.

==> BODY/Backup/chapter1.tex <==
        % \section{Temporal Sequence modelling}

% Background text...
Video data is one type of time-series data. Even though it differs greatly from other such data (\eg speech, text or stock prices) in spatial dimenstionality (\ie each frame of video is a 2-D matrix) and value distributions (i.e., video normally owns three red, green and blue (RGB) channels with ranges determined by the viewed scene and imaging processes), the temporal dimension of videos exhibits some common attributes with other time series, \eg casual relationships between past and future, periodic correlations and smooth transitions, albeit with occasional discontinuities. From this perspective, much work has focused on applying classical temporal sequential modelling to solve video processing tasks.

In this chapter, we review a few major temporal sequential modelling tools that have shown promising results in applications to video understanding. They are Markov Chains, Hidden Markov Models, Bayesian recursive filtering, Gaussian Processes, Auto-Regresstive Models and finally Recurrent Neural Networks. Significantly, the intuition behind these classic tools is greatly shared by the majority of modern approaches but in a more flexible form, which retrospectively underlines the importance of understanding fundamental ideas.

Along with the introduction of basic ideas, concrete cases studies of those methodologies with attention to video sequence data are provided.  

\section{Markov Chains}

Let a time series be defined as an ordered sequence
%Define a time-series data as an ordered sequence:
\begin{equation}
    y_{1:t} = y_{1}, y_{1}, \ldots, y_{t},
\end{equation} 
where one can consider the \textbf{past} and \textbf{future} in the sequence corresponding to ordered indices such as $(1, 2, \ldots, \mathrm{t})$.

A first-order Markov Chain is a standard approach to modelling series of random variables, subject to the constraint that each state depends only on the previous one
\begin{equation}
    p(y_{t} | y_{t-1}).
\label{eq:markov_chain}
\end{equation}
The probability distribution of state transitions is typically represented in terms of the Markov chain’s transition matrix, which often is a stochastic matrix whose entries in each row must add up to exactly one. For $M$ states in the Markov Chain, the transition matrix would be a $M \times M$ matrix.
%A quick example would be forecasting weather based on today's situation through transition matrices, which will be discussed jointly with Hidden Markov Models (HMMs). 

More generally, the model can be extended to ${N_{th}}$ order such that longer dependency is captured:
\begin{equation}
    p(y_{t} | y_{t-1}, y_{t-2}, y_{t-3}, ..., y_{t-N}).
\end{equation}

From the perspective of graphical probability theory, a Markov chain is a directed graph where each temporal state $y_{t}$ has inward connections from one of more previous states (\eg $y_{t-1}$) and outward connections to one or more future states (\eg $y_{t+1}$), as illustrated in Figure \ref{fig:markov_chain}.
\begin{figure}[ht]
    \centering
    \begin{minipage}{.45\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{Figures/HMMs.pdf}
        \subcaption{(a)}\label{fig:sub-a}
    \end{minipage}
    \begin{minipage}{.45\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{Figures/HMMs_2.pdf}
        \subcaption{(b)}\label{fid:sub-b}
    \end{minipage}
\caption{First- (a) and second-order (b) Markov Chain models.}
\label{fig:markov_chain}
\end{figure}

%Markov Decision Process (MDP) \cite{puterman2014markov}, an extension of Makov Chain, is often used in computer vision. MDP extends the vanilla sequential modelling equation \ref{eq:markov_chain} with two extra components: the action space $(a_1, a_2, \ldots, a_t)$ and reward space $(r_1, r_2, \ldots, r_t)$. The actions represent the policy that would decide the transition among observed states
%\begin{equation}
%    p(y_{t} | y_{t-1}).
%\end{equation}
\pagebreak

\section{Hiddens Markov Models (HMMs)}\label{Sec:Temporal_hmm}
A Markov chain is useful when we need to compute a probability for a sequence of observable events. In many cases, however, the events we are interested in are hidden: We do not observe them directly. For example, we might not normally observe the velocity directly from a walking pedestrian. Rather, we might be given geometric distance and time intervals, and must infer the velocity from the ratio of relative moving distance and aggregated time window. We view the velocity as a hidden state because it is not observed.

Formally, we define a Hidden Markov Chain in terms of a sequence of hidden states as $x_{1:T}$, where $T$ is the sequence length, and another sequence of observed variables as $y_{1:T}$. In particular, we define the hidden variable as the causal factor to observations and assume the Markov property for underlying hidden states:
\begin{equation} 
    p(x_{t} | x_{t-1})
\label{eq:1st_markov}
\end{equation}
and
\begin{equation}
    p(y_{t} | x_{t}) = p(y_{t} | x_{t}, x_{t-1}, ..., x_{1}, y_{t-1}, y_{t-2}, ..., y_{1}).
\end{equation}

The estimated probability for an observation at time $t$, $p(y_{t}|x_{t})$ (given its hidden state $x_{t}$), is called the \textbf{emission probability}, which can be used as the inference result when generating outputs. Again, the dynamics behind the hidden sequence is modeled by transition matrices (often denoted as $A$), which can be either invariant to time (\textbf{Homogenous}) or dependent on time (\textbf{Non-Homogenous}). Finally, since every output and state of a sequence is modeled as a probability, an HMM model can be described as generative modelling on sequences as follows
\begin{equation}
\begin{aligned}
    p(x, y) &= p(x_1, ..., x_t, y_1, ..., y_t) \\
            &= p(x_1)p(y_1 | x_1) \displaystyle\prod_{i=2}^{T} p(y_i | x_i) p(x_i | x_{i-1}),            
\end{aligned}
\end{equation}
where $p(x_1)$ and $p(y_1 | x_1)$ are the starting state and observation that are assumed to be independent. Figure \ref{fig:hmm} provides a brief view of this process.

\begin{figure}[htp]
    \centering
    \resizebox{.65\linewidth}{!}{\includegraphics[width=4cm]{Figures/hmm.pdf}}
    \caption{Probabilistic graph model for temporal Hidden Markov Model.}
    \label{fig:hmm}
\end{figure}

HMMs have been applied to a wide range of video understanding tasks, \eg video-based face, finger-spelling and activity recognition \cite{liu2003video,kim2013fingerspelling,raman2016activity}, tracking \cite{yang2016temporal,ullah2018directed} as well as action segmentation \cite{richard2018neuralnetwork, li2019weakly,richard2017weakly, kuehne2018hybrid}. Though these tasks arise in separate settings, research shares many common procedures in their applications. In general, there are three steps in the process. The universal first step involves feature extraction and selection. 
As examples, efforts have converted videos of faces to sequences of eigenvectors \cite{liu2003video}, represented sequences of human appearance as Histograms of Oriented Gradients (HOG) \cite{dalal2005histograms} and represented human motion sequences in terms of Improved Dense Trajectories (iDTs) \cite{wang2013action} with Fisher Vector (FV) encoding \cite{sanchez2013image}, all prior to HMM training.
%For instance, X. Liu \etal, convert the video face images into a sequence of eigenvectors, M. Yang \etal, advocate to use \textit{histogram of oriented gradients} (HOG) feature as an effective representation for human appearance and A. Richard \etal, adopt \textit{improved dense trajectory} (iDT) \cite{wang2013action} feature encoded with \textit{Fisher Vector} (FV) \cite{sanchez2013image} before perform the training of HMM.

The second step is to define a generative model that induces a training process for model parameters. There are three parts of an HMM that need parameter learning from training data: 

\begin{enumerate}
  \item The starting state probability $p(x_1)$; 
  \item The transition probability $A = p(x_i | x_{i-1})$;
  \item The emission probability $p(y_i | x_i)$ that maps hidden states to observations.
\end{enumerate}

The standard choice for initializing the former two components is the uniform distribution, while the standard choice for the third is the Gaussian Mixture Model (GMM) (\eg \cite{yang2016temporal}). Typically, these parameters are jointly learned through the Expectation Maximization (Baum-Welch) algorithm \cite{dempster1977maximum} with an objective to maximize a posterior (MAP).
\begin{figure}[htp]
    \centering
    \resizebox{.55\linewidth}{!}{\includegraphics[width=4cm]{Figures/neural_viterbi.png}}
    \caption{\textcolor{red}{Temporal HMM decoding for action segmentations}, with HMMs implmented as learnable neural networks \cite{richard2018neuralnetwork}.
    The class label for the $i_{th}$ segment is denoted as $c_i$ and the segment length denoted as $l_i$. The input video is forwarded through the network and the Viterbi decoding is run on the output probabilities. The frame labels generated by the Viterbi algorithm are then used to compute a framewise cross-entropy loss on which the network gradient is computed. Figure reproduced from \cite{richard2018neuralnetwork}.}
    \label{fig:hmm_decoding}
\end{figure}

\begin{figure}[]
    \begin{minipage}{\textwidth}
        \centering
        \resizebox{.625\linewidth}{!}{\includegraphics{Figures/hog_hmm.pdf}}
        \caption{Example of using HMMs for video human tracking. Appearance features (upper-row) for each detected pedestrian are extracted via Histogram of Oriented Gradient (HOG) and used for building an observation density shown as sphere nodes in lower graph. 
        The number on nodes $\{1, 2, 3, 4\}$ and blue arrow denote the temporal evolution of observations.
        The state transition is shown as edges between nodes as solid lines. An HMM is built for each pedestrian in the training set and tested on each detected pedestrians during testing. Figure reproduced from \cite{yang2016temporal}.}
    \label{fig:hmm_tracking}
    \end{minipage}
\end{figure}

The third step in applying an HMM to a (video understanding) problem is inferring the end-goal from the emission probability function; namely, \textbf{what is the most likely sequence label given an observed test sequence?} Since HMMs are generative models, instead of discriminative ones, there are two ways to achieve classifications. The first approach assumes the sequential hidden states can represent class labels and thereby the best-fit states would be taken as classification results (typically dubbed HMM decoding) via the Viterbi algorithm \cite{forney1973viterbi} according to:
\begin{align*}
    y* &= \operatorname*{argmax}_{y \in {y_1, \ldots, y_T}} p(x_1, ..., x_t, y_1, ..., y_T) \\
       &= \operatorname*{argmax}_{y \in {y_1, \ldots, y_T}} p(y_1)p(x_1 | y_1) \displaystyle\prod_{i=2}^{T} p(x_i | y_i) p(y_i | y_{i-1}).
\label{eq:hmm_decoding}
\end{align*}
However, this approach is not easily applicable to datasets that contain a large number of classes, where the number of states increase linearly in proportion to the size of categories. As a remedy, the second approach is through training HMMs for each class cateogory in the datasets of interest. In the classification phase, given a target video, we would first make an observation sequence and feed it into every HMM. By evaluating the probability for each HMM, the target video is assigned into a class based on the highest HMM probability.

%For recognition tasks, each HMM model learned on each class of training set would produce likelihood scores by fitting test data into the learned emission probability function and pick the maximum likelihood model. Typically, the best-among-N is taken as the class index. Temporal action detection is similar to recognition, except that at each time step the class of the performed action is to be preserved without aggregation. Tracking can be similarly framed as discrimination of each detected pedestrian with pre-trained HMM models.
Both classification methods have been applied to computer vision tasks. As an example for the HMM decoding approach, some work proposed a neural-network implemented Viterbi decoding HMM to infer the segment-wise action label \cite{richard2018neuralnetwork}; see Figure \ref{fig:hmm_decoding}. Similar work includes \cite{kuehne2018hybrid, li2020set, koller2017re}. As for the second approach, an effort has proposed to incorporate HMMs with appearance features (HOG) for pedestrians tracking \cite{yang2016temporal}; see Figure \ref{fig:hmm_tracking}. Each newly detected pedestrian is tested with all pre-trained HMMs to associate with an existing pedestrian template. 

%A. Richard \etal \cite{richard2018neuralnetwork} proposed a neural-network implemented viterbi decoding HMM to infer the segment-wise action label (see Figure \ref{fig:hmm_face} segment class denoted as $c_i$ and segment length denoted as $l_i$).
%As an example for the second approach, M. Yang \etal \cite{yang2016temporal} proposed to incorporate HMMs with appearance features (HOG) for pedestrians tracking, as shown in Figure \ref{fig:hmm_tracking}. Each newly detected pedestrian would be tested with all pre-trained HMMs to associate with existing pedestrian template. 

Other related work explores the possibility of extending the expressiveness of HMMs. One direction is to enrich the hidden states by stacking them in hierarchical fashion \cite{raman2016activity}. Another is to relax the assumption on prior distributions for learning parameters (the initial distribution, the transition matrix and the emission matrix). A currently trending approach to relaxing these assumptions is grounding the HMM as a learnable Recurrent Network Network (RNN) \cite{richard2018neuralnetwork, richard2017weakly, li2019weakly}.

%Abovementioned operations are necessary to properly execute HMMs which, on the other hand, reveals several limitations: \textbf{1.} expensive and slow to run optimization algorithms (EM algorithm run time increases dramatically with the number of hidden states); \textbf{2.} difficult to extend the dependency from lower order to higher; \textbf{3.} unable to perform online inference due to the prerequisite for fixed temporal data length during training.

Finally, it is important to note that the necessary operations to yield a classic HMM reveal several limitations. First, they can be expensive and slow to run their optimization algorithms (e.g., model run time increases dramatically with the number of hidden states). Second, extensions to high-order models can be very complicated. Third, the ability to do inference on variable length input data requires a time-invariant transition matrix, $A$, which is often less expressive than time-variant ones.

%Third, online inference can be difficult to achieve because of the prerequisite of fixed temporal length during training \cite{}.

\section{Bayesian Filtering}
The problem of temporal \textit{filtering} is an operation that involves the extraction of information about a quantity of interest at time $t$ by using data measured up to and including $t$ \cite{chen2003bayesian}. (Here, we ignore the possibility of noncausal filters). We define a generic form of the filtering problem from the perspective of the dynamic state-space system over a sequence of state variables, $(x_1, \ldots, x_T)$, and time-measured observations, $(y_1, \ldots, y_T)$:
\begin{equation}
\centering    
\begin{aligned}
    &x_{t+1} = f(x_t, q_t) \\
    &y_{t} = h(x_{t}, r_t).
\label{eq:genric_filtering}
\end{aligned}
\end{equation}
In the above formulation, $x_t$ represents the state vector at a given step, while $y_t$ stands for its observation; $q_t$ and $r_t$ represent the process noise and measurement noise at time $t$, respectively; $f$ and $h$ are functions that model physical relationships between adjacent states and measurements, respectively. More specifically, the state function, $f$, is responsible for transitioning state vectors forward in time, which characterises the transition probability, $p(x_{t+1} | x_t)$, and the measurement equation, $h$, for mapping the states to an estimated observation vector, which captures the measurement probability, $p(y_{t} | x_{t})$. 

This formula is widely adopted in modelling many real-world physical systems (\eg estimating airplane locations or robot trajectories) and the quantity of interest that researchers attend to hereby is the state vector $x_t$ (\eg velocity, gravity force or air resistance). In other words, the \textbf{objective} of filtering is to estimate the posterior density $p(x_t | y_{1:t})$ at any given step.

Bayes' theorem builds the fundamental formulation for conditional probability $p(y|x)$ with its inverse conditional probability $p(x|y)$ and the marginal probabilities $p(y)$ and $p(x)$ as follows. This formulation naturally fits the purpose of filtering \cite{ho1964bayesian}, especially when states and observations are treated as random variables subject to certain distributions. The theorem is given as
\begin{equation}
    p(x | y) = \frac{p(y|x) p(x)}{p(y)},
\label{eq:bayes_rule}
\end{equation}
where $p(x)$ represents the \textbf{\textit{prior}} knowledge we have about the states, $p(y|x)$ is the \textbf{\textit{likelihood}} probability, while the denominator, $p(y)$, stands for the probability of observing $y$ happening, which usually gets taken as a constant value due to its independence from the targeted state variables. Therefore, the central idea of Bayesian inference is to use priors and likelihood knowledge, quantitatively and qualitatively, to infer the conditional probability, given tractable observations, which corresponds to the goal of filtering. However, vanilla Bayes theorem is not directly applicable to sequential data, as there is no linkage between data in time.


Formally, Bayesian filtering is defined as a combination of the Markov property and Bayes rule with two major assumptions \cite{chen2003bayesian}: \textbf{1.} The hidden states follow a first-order Markov process $p(x_t | x_{1:t-1}) = p(x_t | x_{t-1})$; \textbf{2.} The real measurements, $y_t$, are independent of the given states. The conditional probability density function of $p(x_t | y_t)$ thus can be described as:
\begin{equation}
\centering    
\begin{aligned}
p(x_t|y_t) &= \frac{p(y_t | x_t) p(x_t)}{p(y_t)} \\
           &= \frac{p(y_t, y_{t-1} | x_t) p(x_t)}{p(y_t, y_{t-1})} \\
           &= \frac{p(y_t|y_{t-1}, x_t)p(y_{t-1} | x_t) p(x_t)}{p(y_t | y_{t-1}) p(y_{t-1})} \\
           &= \frac{p(y_t|y_{t-1}, x_t)p(x_t | y_{t-1}) p(y_{t-1}) p(x_t)}{p(y_t | y_{t-1}) p(y_{t-1}) p(x_t)} \\
           &= \frac{p(y_t | x_t) p(x_t | y_{t-1})}{p(y_t | y_{t-1})}.
\label{eq:bayes_filtering}
\end{aligned}
\end{equation}
Under these assumptions, the prior becomes
\begin{equation}
p(x_t | y_{t-1}) = \itt p(x_t | x_{t-1}) p(x_{t-1} | y_{t-1}) dx_{t-1},
\end{equation}
which represents the newly propagated states only from the very last step posterior, $p(x_{t-1} | y_{t-1})$, and the model dynamic, $p(x_t | x_{t-1})$. The likelihood, $p(y_t | x_t)$, and evidence, $p(y_t | y_{t-1})$, serve the same role as before but are self-contained at given time step $t$, without depending on any remote historical states or observations (\eg $t-2$). 
%The graphical model is depicted as Figure \ref{fig:bayesianFilter}. 
The graphical representation of Bayesian filtering is identical to the one given for HMMs in Figure \ref{fig:hmm}.
\iffalse
\begin{figure}[htp]
    \centering
    \resizebox{.5\linewidth}{!}{\includegraphics[width=4cm]{Figures/bayesian_filtering.pdf}}
    \caption{Bayesian filter in graphical presentation behaves in an analogous manner to a first-order hidden Markov model.}
    \label{fig:bayesianFilter}
\end{figure}
\fi

It is worth noticing that the conditional modelling property of Bayesian filtering makes it easier to perform than the Hidden Markov Model, which aims at modelling the joint probability of the entire sequence data pair (\ie observation $y_{i}$ and hidden states $x_{i}$). For every new incoming state and observation, HMMs need to re-run the whole sequence, while Bayesian filtering can do inference conditioned on only the last state.

To this point, the theoretical formulation of Bayesian filtering has been soundly built, though it is still vague on how to implement it with a tractable realization (\ie how to decide the distribution of likelihood and prior). In the next two sections, we present the celebrated Kalman filter and particle filter as concrete examples that realize Bayesian filtering in practice.

\subsection{Kalman Filtering}
Kalman filtering is one convenient instantiation of Bayesian filtering \cite{chen2003bayesian}. It merges the essence of recursive probability estimation with linear differential systems, through assuming \textbf{Linear–Quadratic} dynamics for state variables and \textbf{Gaussian} uncertainty for both the process and measurement noise. Taken together, these assumptions are known as LQG. Consider the same sequence of state-space data from previous section, $(x_1, ..., x_T)$ and $(y_1, ..., y_T)$, the generic filtering equation \ref{eq:genric_filtering} under the LQG assumptions can be re-expressed in a simpler version as:
\begin{equation}
x_{t+1} = F x_t + q_t
\label{eq:kf_pred_1}
\end{equation}
and
\begin{equation}
y_{t} = H x_t + r_t,
\label{eq:kf_pred_2}
\end{equation}
where $F$ is the transition matrix, $H$ is the measurement matrix, $q_t$ and $r_t$ are white Gaussian noise at time step $t$. These two steps are named the \textbf{prediction} step in Kalman filtering, which jointly operationalize the prior transition step, $p(x_t | y_{t-1})$, in Bayesian filtering.

The second step of Kalman filtering is given according to
\begin{equation}
\centering
\begin{aligned}
    &P_{t|t-1} = FP_{t-1}F^{T} + q_t \\
    &K_t = P_{t|t-1}H^{T} (HP_{t|t-1}H^{T} + r_t)^{-1} \\
    &x_t^{MAP} = \hat{x}_{t|t-1} + K_t (y_t - H\hat{x}_{t|t-1}) \\
    &P_t = P_{t|t-1} - K_tHP_{t|t-1},
\end{aligned}
\label{eq:kalman_update}
\end{equation}
where $K_t$ is called Kalman Gain, $P_t$ is the state error covariance matrix, $\hat{x}_{t|t-1}$ is the prior state estimation given observations till $y_{t-1}$ and $x_t^{MAP}$ is the Maximum A Posteriori (MAP) estimate of $x_t$. 
%The detailed deduction of above equations can be found in appendix \ref{appendix:kalman}.
These equations support the posterior estimation from the priors and the likelihood. In practice, they are named the \textbf{update} step since they assimilate the up-till-now incoming observations and inversely correct the predicted states. A detailed derivation of the Kalman filtering equations, (2.13),  from the point of view of Bayesian filtering is provided in Appendix \ref{appendix:kalman}.
The Kalman Gain,
$K_{t}$ , is derived from the ratio of the state uncertainty, $P$, and the measurement noise, $r_{t}$. It balances the prior state estimation, $\hat{x}_{t|t-1}$, and the measurement error, $y_t - H\hat{x}_{t|t-1}$. An accurate system should reduce the $K_t$ term since the prior prediction should be accurate enough to represent the real states.

Besides the Kalman Gain, another equally critical factor is the error covariance, $P_t$, which in nature reflects the covariance of the state vectors, yet numerically focuses on the state residual errors (here assuming the state-error vector is a random variable). 
%Therefore, in equation \ref{eq:prior}, the deduction of the state covariance yields $Cov(x_t | y_{t-1}) =  Cov(e_t|e_{t-1})$.
The predicted state covariance relies on the physical model matrix, $F$, and the process noise, $q$. One step of Kalman filtering is depicted in Figure \ref{fig:kalmanFilter}.
\iffalse
As indicated by Equation \ref{eq:error_prop}, the prediction of the state covariance relies on the physical model matrix, $F$, and the process noise, $q$. For any transition matrix that has numeric elements that are larger than 1 (\ie $|F| > 1$), the state covariance would be amplified. From equation \ref{eq:error_update}, the error covariance will be udpated by re-assigning the prior prediction $P_{t|t-1}$ with the ratio $(I - K_t H) \in (0, 1)$ that depends on the Kalman Gain $K_t$. One iterating step, $t-1$ to $t$, of Kalman filtering is depicted in Figure \ref{fig:kalmanFilter}.
\fi

The most noticable merit of Kalman filtering is its \textbf{optimality}. Given a linear dynamic system model and known Gaussian distributions for noise, the estimated state is guaranteed to match the real system, since the MAP estimation on a linear function can lead to a global optimum.

The most well-known disadvantage of Kalman filtering is its limitation to only \textbf{uni-modal} modelling. Under LQG assumptions, the implementation of the desired posterior is always a \textbf{single} Gaussian parameterized with its moments (\ie mean and covariance). When the target measurement behaves like a mixture of Gaussian distributions that contains more than one modality, the Kalman filter can only follow one mode. 

Another critical flaw of the Kalman filter is the \textbf{Linear} assumption. Though simple and efficient, many higher level vision tasks are better modeled by nonlinear state transitions, in which case the Kalman filter could only provide sub-optimal solutions.
\begin{figure}[htp]
   \centering
    \resizebox{.7\linewidth}{!}{\includegraphics[width=4cm]{Figures/Kalman.png}}
    \caption{Depicting the Kalman filtering process. A Gaussian shape distribution is propagated by iterating steps at each time frame. However, only one Gaussian blob can be processed at a time. Figure reproduced from \cite{wiki:kalman}.}
    \label{fig:kalmanFilter}
\end{figure}

More generally, not all physical rules can be modeled as linear systems. Thus, the \textbf{Extended} Kalman filter (EKF) and \textbf{Unscented} Kalman filter (UKF) \cite{julier1995new} have been proposed to enable more flexible estimation on nonlinear processes. The former admits nonlinear state transition/measurement functions, $f$ and $h$, to replace the previous matrices, $F$ and $H$, so that the Eq. \ref{eq:kf_pred_1} and \ref{eq:kf_pred_2} become
\begin{equation}
    x_{t+1} = f(x_{t})
\label{eq:nonlinear_k}
\end{equation}
and
\begin{equation}
    y_{t} = h(x_{t}),
\end{equation}
respectively.

The \textbf{update} step is the same as Eq. \ref{eq:kalman_update}, except that the matrices used are derived from the \textbf{Jacobian} matrices of $f$ and $h$, namely $F = \frac{\partial f}{\partial x}$ and $H = \frac{\partial h}{\partial x}$ (first-order Taylor expansion), which represents a linear approximation to nonlinear functions and therefore can not guarantee optimal estimation. The UKF further relieves the \textbf{update} step from the linear constraint by resorting to a sampling approach, but ends up being expensive on computational resources.

\textbf{Applications:} The Kalman filter has been applied widely in fields like computer vision, robotics and navigation systems. Concrete examples include the Global Positioning System (GPS), Unmanned Aerial Vehicles (UAV) and tracking of human trajectories or motions assisted with technologies from signal processing, sensor information and computer vision. Precedents found success when coupling Kalman filtering with physical law based motion models, \eg velocity, acceleration, moving angle, airflow resistance and gravity. In the instance of video-stream vehicle tracking, people found it useful to use the EKF with vehicle's positions, speeds and turning angles as state variables to track the observed coordinates \cite{guerrero2013vehicle}. The main theme is finding an applicable physical model for the state transition.
\iffalse
As a simple example, 
consider tracking objects in a 2D X-Y plane. We can build a simple Kalman filtering system to achieve this goal. First, the state vector $\mathbf{x}$ is explicitly defined as
%exmple from: https://github.com/balzer82/Kalman/blob/master/Kalman-Filter-CA-2.ipynb;
\begin{equation}
\centering
\mathbf{x} =
\begin{bmatrix}
    x\\
    y\\
    v_x\\
    v_y\\
    a_x\\
    a_y\\
\end{bmatrix},
\end{equation}
where $x,y$ are coondinates, $v_x, v_y$ are velocities and $a_x, a_y$ are accelerations. Following the physical motion formula $y = x + \Delta t v + \frac{1}{2} \Delta t^2 a; v = v + \Delta t a$, the transition between states can be defined as (assuming constant acceleration):
\begin{equation*}
\centering
    \mathbf{x}_{t+1} = 
    \begin{bmatrix}
        1& 0& \Delta t & 0 & \frac{1}{2}\Delta t^2& 0 \\
        0& 1& 0& \Delta t& 0& \frac{1}{2} \Delta t^2 \\
        0& 0& 1& 0& \Delta t& 0 \\
        0& 0& 0& 1& 0& \Delta t \\
        0& 0& 0& 0& 1& 0 \\
        0& 0& 0& 0& 0& 1
    \end{bmatrix}
    \mathbf{x}_t
\end{equation*}

The measurement, $\mathbf{y}_t$, namely the observed positions, can be expressed from the measurement matrix as
\begin{equation*}
\centering
    \mathbf{y}_t = 
    \begin{bmatrix}
    1 & 0 & 0 & 0 & 0 & 0 \\
    0 & 1 & 0 & 0 & 0 & 0
    \end{bmatrix}
    \mathbf{x}_t + \mathbf{r}_t
\end{equation*}
where $r_t$ is the measurement noise $r_t \sim\ N(0, R)$. The state error covariance $P_t$ is
\begin{equation*}
\centering
    \mathbf{P}_{t+1} = F\mathbf{P}_{t}F^{T} + \mathbf{q}_t = F
    \begin{bmatrix}
        cov_{x,x}& cov_{x,y}& 0 & 0 & 0 & 0 \\
        cov_{y,x}& cov_{y,y}& 0& 0& 0& 0 \\
        0& 0& 0& 0& 0& 0 \\
        0& 0& 0& 0& 0& 0 \\
        0& 0& 0& 0& 0& 0 \\
        0& 0& 0& 0& 0& 0
    \end{bmatrix}
    F^{T} + \mathbf{q}_t
\end{equation*}
where $\mathbf{q}_t$ is the process noise $\mathbf{q}_t \sim\ N(0, Q)$ and similar for $\mathbf{r}_t$.

The noise parameters, $R$ and $Q$, are manually defined beforehand to mimic the real environment. The very initial error covariance $P_1$ also needs to be specified to reflect the initial uncertainty,
but it will eventually converge to a steady value as the process goes on. Figure \ref{fig:KF_example_ball} plots the development of prediction, update and noise measurement of 2D coordinates along time.
\begin{figure}[htp]
   \centering
    \resizebox{.7\linewidth}{!}{\includegraphics[width=4cm]{Figures/Kalman-Filter-CA-Ball-StateEstimated.png}}
    \caption{Kalman filtering example for tracking 2D plane coordinate measurements which follow linear velocity-acceleration motion function.}
    \label{fig:KF_example_ball}
\end{figure}
\begin{figure}[htp]
   \centering
    \resizebox{.7\linewidth}{!}{\includegraphics[width=4cm]{Figures/Kalman-Filter-CA-Ball-KalmanGain.png}}
    \caption{Kalman Gain, $K_t \in (0, 1)$, changing plot. The lower, the more the measurement fullfill the prediction.}
    \label{fig:KF_example_ball}
\end{figure}
\fi
\iffalse
\begin{figure}[ht]
    \centering
    \begin{minipage}{.45\textwidth}
    \includegraphics[width=1.25\textwidth, height=4cm]{Figures/kalman_vehicle.PNG}
    \end{minipage}
    \begin{minipage}{.45\textwidth}
    \begin{flushright}
    \includegraphics[width=.6\textwidth, height=4cm]{Figures/kalman_motion.png}
    \end{flushright}
    \end{minipage}
\caption{Vehicle tracking on street scenes (Left) with assumed motion states equation that involves velocities $v_{x}, v_{y}$, positions $P_{x}, P_{y}$ and directional angle $\phi$ (Right).}
\label{fig:kalman_vehicle}
\end{figure}
\fi
\iffalse
All abovementioned methods (KF, EKF, UKF) rely on pre-defined motion models as transition functions. No matter how complicated, they are not easily adaptale to out-of-domain data and lack the ability to explore unknown motion relations from the data. How to effectively adapt the transition model to our needs remains an open question.
\fi
Reliance on pre-defined motion models across the Kalman filter and its standard variants (EKF, UKF), makes them not easily adaptable to out of domain data and limits their ability to explore uknown motion relations in the data. How to effectively adapt transition modelling remains an open question.

\textbf{Learning Based Extensions}: In recent progress of machine learning, Kalman filtering is frequently revisited. Researchers try forging its core concepts into a learning structure with two general goals: \textbf{1.} Alleviating the rigid transition model and Gaussian noise assumption; \textbf{2.} Overcoming the dimensionality curse and extending the application landscape to new horizons.

As an example of the first consideration, an early effort proposed to substitute the transition function $f$ as well as the two noise terms with Long-Short Term Memory (LSTM \cite{hochreiter1997long}) units \cite{coskun2017long}. They apply the proposed LSTM-KF to regularize a series of video human body keypoint estimations and demonstrate that the merged method performs better than a Kalman filter under hand-crafted motion models (velocity and acceleration) as well as a pure learning LSTM network. Similar work includes \cite{dynamet2019chen}. Figure \ref{fig:lstm_kf} provides an illustration.

\begin{figure}[ht]
    \centering
    \begin{minipage}{.4\textwidth}
    \centering
    \includegraphics[width=1.\textwidth, height=4cm]{Figures/lstm_kf.PNG}
    \subcaption{(a)}
    \end{minipage}
    \begin{minipage}{.4\textwidth}
    \centering
    \begin{flushright}
    \centering
    \includegraphics[width=.57\textwidth]{Figures/lstm_kf_body.png}
    \end{flushright}
    \subcaption{(b)}
    \end{minipage}
\caption{(a) Realization of Kalman filtering with LSTM units. The state transition, $p(\hat{y}_{t} | \hat{y}_{t-1})$, and noise terms, $\mathsf{Q}$ and  $\mathsf{R}$, now are the outputs of three learnable LSTM networks, rather than manually defined priors.
(b) Body key-point generation outcomes from distinct implementations. Proposed LSTM-KF approach (highlighted with red rectangular) produces the best result.
Both (a) and (b) reproduced from \cite{coskun2017long}.
}
\label{fig:lstm_kf}
\end{figure}

Other work takes this path one step further \cite{haarnoja2016backprop}. In that work, it is argued that the classic transition function is a generative estimator in the probability world, which has limited capacity to handle rich sensory observations, \ie high resolution images and videos. Indeed, existing work resorted to preprocessing raw data input, \eg obtaining 2-D positions of pedestrians through detectors, prior to Kalman filtering.
\iffalse
\begin{figure}[htp]
  \centering
\resizebox{.95\linewidth}{!}{\includegraphics[width=4cm]{Figures/backprop_kf.png}}
\caption{Discriminative state estimation model emboddied through forward neural network from \cite{haarnoja2016backprop}. This model inputs high-dimensional observations, such as raw images denoted as $o_{t}$, and produces an intermediate observation $z_{t}$ to interlace with the underlying dynamic state $\mu$, which will be used to produce final observation $y_t$.
Two noise terms ($\mathsf{Q}$ and $\mathsf{R}$) are also learned instead of pre-defined. 
}
\label{fig:backprop_kf}
\end{figure}
\fi
In response, the authors advocated a discriminative model that maps raw high dimensional observations to a low dimensional vector
%(denoted as $\mathbf{z}$) 
as an intermediate observation state, together with a positive-definite covariance matrix
%, $L$, 
for constructing the noise.
%($\mathsf{Q}$ and $\mathsf{R}$) 
%, as shown in Figure \ref{fig:backprop_kf}. 
The projected vector
%$\mathbf{z}$, 
works as the measurement in the \textbf{update} step to capture the underlying dependency between observations and states. However, arguably such an extension still deviates from directly applying Kalman filtering to complex visual tasks, since its down-steam output is still low dimensional geometry information (\eg groundtruth output is either tracking coordinates in $\mathbb{R}^{2}$ or visual odometry in $\mathbb{R}^{3}$ that determines the position and orientation of a vehicle by analyzing the associated camera images).

As to the second consideration, extensions to wider applications and overcoming associated dimensionality issues, recent breakthroughs have led to the use of Kalman filtering in unpredecented fields, such as video action detection \cite{dave2017predictive}, video artifact reduction \cite{lu2018deep}, temporal feature propagation \cite{zhao2019spatiotemporal} and video pixel prediction \cite{guen2020disentangling}. Theses efforts share two common attributes: \textbf{1.} The \textbf{predict-update} functionality is extended to visual and semantic feature spaces; \textbf{2.} Video frame-wise \textbf{residuals} are found complementary to Kalman filtering mechanisms.

%For example, A. Dave \etal \cite{dave2017predictive} firstly propose to incorporate Kalman structure onto video action semantic detection. 
As an example, it has been proposed to incorporate the Kalman structure into action semantics detection \cite{dave2017predictive}.
In that framework, the noise terms ($q_t, r_t$ of Equations \ref{eq:genric_filtering} and \ref{eq:kalman_update}) are ignored (since the task has marginal relation with state uncertainty) and the semantic action activation layer in a deep ConvNet at every time-step is a linear combination of such features from the previous step and a corrective (residual) term distilled from raw image observations. Notably, such high dimensional representation was prohibitive in earlier eras due to lack of computational resources; see Figure \ref{fig:CNN_KF_Detection} for the predictive-corrective component of \cite{dave2017predictive}.

\begin{figure}[htp]
   \centering
    \resizebox{.85\linewidth}{!}{\includegraphics[width=4cm]{Figures/CNN-KF-Detection.pdf}}
    \caption{Proposed predictive-corrective action detection framework that filters two adjacent observations $t \in (1, 2)$ in \cite{dave2017predictive}. ConvNet (denoted as CNN) is used as the key technique to perform state transit between time steps. Previous prediction at each step will be corrected by the next observation and thus the propagation error is not accumulated. Figure reproduced from \cite{dave2017predictive}.}
    \label{fig:CNN_KF_Detection}
\end{figure}

Various efforts have followed this general idea. One such effort thinks of the predicted video pixel residual as the corrective add-on, which shares the same resolution with original images \cite{lu2018deep}. Others choose to predict the temporal residual of the intermediate ConvNet features \cite{guen2020disentangling, zhao2019spatiotemporal}, since the middle layer preserves rich spatial structure information, and update the recovered feature with real measurements. 
%However, there are some subtle distinctions between them, \ie \cite{zhao2019spatiotemporal} uses deep features with resolution (28x28x192), while \cite{guen2020disentangling} uses (7x7x128).

One possible reason why Deep-Kalman proposals can enhance complex video tasks is that advances from machine learning theory help overcome the long-existing struggle to model high dimensional data. Here, the residual term is essential, since large portions of video data contains redundancy with adjacent frames. By modelling the adjacent residual, models are taught to focus on the dynamic part (\ie on-going action movements or walking pedestrians) rather than static ones (\ie backgrounds).

Beyond the abovementioned uses of Deep Kalman filtering in computer vision tasks, such an idea also has been investigated in the traditional machine learning literature. As examples, a hybrid model that combines physical dynamic rules, learning based transition matrices and latent variables was investigated to estimate the trajectory of a noisy chaotic Lorenz Attractor \cite{satorras2019combining}. Another effort approached Kalman filtering with a variational inference backbone \cite{kingma2013auto} and then modeled the change of a patient’s state over time \cite{krishnan2015deep}. Further similar work includes \cite{karl2016deep, rangapuram2018deep}. Again, these efforts relaxed the LQG assumptions of standard Kalman filtering. Parallel work devoted to supporting high dimensional data modelling in Kalman filtering suggested factorizing latent variables into low dimensional data (even scalars) \cite{becker2019recurrent}.  The authors also relied on recurrent neural networks to enable nonlinear dynamics for the state transition.


%Similarly, G. Lu \etal \cite{lu2018deep}, H. Zhao \etal \cite{zhao2019spatiotemporal} and V. Le Guen \etal \cite{guen2020disentangling} all succeed this idea. Lu thinks of the predicted video pixel residual as the corrective add-on, which shares the same resolution with original images (height:448, width:256). Instead, Zhao and Guen focus on predicting the temporal residual of the intermediate ConvNet features (28x28x192 and 7x7x128 respectively), since the middle layer preserves rich spatial structure information, and update the recovered feature with real measurements.
\iffalse
\begin{figure}[ht]
    \centering
    \includegraphics[width=.6\textwidth, height=4cm]{Figures/pred_cor_kf2.PNG}
\label{fig:deep_kf}
\caption{Generic description of deep Kalman approach for high-dimensional visual observation or semantic feature from \cite{dave2017predictive}.}
\end{figure}
\fi

\subsection{Particle Filtering}
In this section we describe another famous Bayesian filter, the particle filter. In constrast to the Kalman filter, the particle filter is non-linear and non-Gaussian but is still under the Markov property. That is to say, the dynamics behind the state variable and the noise distribution can be of almost any form. These great merits come from the Monte-Carlo Sampling idea that uses a set of particles to represent target distributions in a non-parameteric fashion. Thus, the particle filter is categorized as a Markov Chain Monte-Carlo (MCMC) \cite{del1997nonlinear} method or \textit{Sequential Monte-Carlo} (SMC) \cite{liu1998sequential}.

Instead of directly calculating the desired posterior, $p(x_t |y_t)$, by assuming a Gaussian distribution, its density can be empirically represented by a weighted sum of $N_p$ samples drawn from the posterior distribution
\begin{equation}
    p(x_t| y_t) \approx \frac{1}{N_p} \sum_{t=1}^{N_p} \hat{w}_{t}^{i} \delta(x_t - x_t^{(i)}) = \hat{p}(x_t | y_t),
\label{eq:pf_posterior}
\end{equation}
where $x_t^{(i)}$ are sampled data points from $p(x_t | y_t)$, $\hat{w}_t^{i}$ are weights and $\delta(\cdot)$ is the Dirac delta function. However, it is impossible to draw data from the optimal $p(x_t | y_t)$ prior to owning its estimation. An alternative is to find a \textit{proposal distribution} $q(x_t | y_t)$ and draw samples from it to approximate $p(x_t | y_t)$. Apparently, not all approximated samples are valid and therefore we should weight the alternative samples according to
\begin{equation}
    w^{i}_{t} = \frac{p(x_{t}^{i}| y_{1:t})}{q(x_{t}^{i}| y_{1:t})}.
\label{eq:particle_weight}
\end{equation}

In practice, this step could be done through calculating the absolute value of the deviation of the measurement from its expected value with a certain evaluation metric (\ie using Chi-square distributions on $p(x_{t}^{i}| y_{1:t})$ and $q(x_{t}^{i}| y_{1:t})$).
Therefore, for a batch of samples $N_p$ at time $t$, the normalized weight $\hat{w}^{i}_{t}$ for the $i_{th}$ sample point is
\begin{equation}
        \hat{w}^{i}_{t} = \frac{w^{i}_{t}}{\sum^{N_p}_{i=1}w^{i}_{t}}.
\end{equation}

Recalling that Bayes' rule and the first-order Markov chain assumption contribute greatly to the derivation of the Kalman filter, the particle filter also benefits from these two assumptions. More specifically, 
we follow Equation \ref{eq:bayes_filtering} and further set $q(x_t | x_{t-1}, y_{1:t}) = q(x_t | x_{t-1}, y_{t})$.
Then, Equation \ref{eq:particle_weight} can be rewritten as
\begin{equation}
    \begin{aligned}
       w^{i}_{t} &\sim\ \frac{
           p(y_t | x_t)p(x_t | x_{t-1})
       }{
           q(x_t | x_{t-1}, y_{1:n})
       } \\
       &= \frac{
           p(y_t | x_t)p(x_t | x_{t-1})
       }{
            q(x_t | x_{t-1}, y_{t})
       }.
    \end{aligned}
\end{equation}

The most common choice for the proposal distribution is the prior probability $q(x_t | x_{t-1}, y_{t}) =p(x_t | x_{t-1})$, thus the weights can be simplified as $w^{i}_{t} = p(y_t | x_t^{i})$. Having obtained both the samples and their weights, the posterior can be easily calculated using Equation \ref{eq:pf_posterior}.
In general, the particle filter operates in the following workflow:
\begin{itemize}
    \item Generate data samples from prior probability.
    \item Assign weights to samples that are valued from observations.
    \item Approximate the posterior with weighted samples.
\end{itemize}

\begin{figure}[ht]
    \centering
    \includegraphics[width=.6\textwidth]{Figures/mc.png}
\caption{Illustration of density representation through particles. Purple circles stand for particles. Larger size of circle means denser (larger quantity) particle clustering and therefore higher the density value, $p(x)$. Figure reproduced from \cite{particle}.} 
\label{fig:particle_density}
\end{figure}
            
The particle filter has both pros and cons. On the pro side, the Monte-Carlo based inference empowers the particle filter supporting \textbf{multi-modality}. In the previous literature, each state variable equals to an uni-modal Gaussian distribution and it is unfeasible to expand them to multivariate. On the contrary, the particle filter enables modelling any-form of distribution through particles (as shown in Figure \ref{fig:particle_density}). Problems that demand multiple outcomes, such as robotic localization and multi-target tracking, are then feasible, see Figure \ref{fig:pf_poor}(b).

On the con side, since sampling based methods rely on valid particles to obtain decent distributions, the first evident disadvantage of the particle filter is the possible need to select a large amount of particles, which can be expensive and non-real time in practice. As shown in Figure \ref{fig:pf_poor}(a), the number of particles plays an important role in adequately matching the target distribution.
\begin{figure}[ht]
    \centering     
    \begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/Histogram-Plots-of-Differently-Sized-Monte-Carlo-Samples-from-the-Target-Function.png}
    \subcaption{(a)}
    \end{minipage}
    \begin{minipage}{.425\textwidth}
    \centering
    \begin{flushright}
    \includegraphics[width=1.\textwidth]{Figures/Screen Shot 2020-09-26 at 2.13.55 AM.png}
    \end{flushright}
    \subcaption{(b)}
    \end{minipage}
\caption{(a) Illustration of the sensitivity of Monte Carlo approaches in terms of the number of samples. Insufficient amount of samples can lead to misinformed estimation.
(b) Example of using the particle filter for robot localization from \cite{fox1999monte}. Red dots represent particle samples that can scatter around multiple possible locations on the floor plan; Green dot is the robot agent that can attend to all possible locations covered by particles (blue lines), which differs from the Kalman filter. Subfigure (b) reproduced from \cite{nummiaro2002color}.}
\label{fig:pf_poor}
\end{figure}
However, owning enough particles can not always guarantee optimality. When there are a few particles dominating the probability weights, while the majority of other particles are near-zero weight, the resulting approximation suffers the same issue as above. This issue is referred to as \textbf{sample degeneracy}. The typical remedy is to remove dead particles, perform resampling and assign them uniform weight. This resetting process is dubbed Sequence Importance Resampling (SIR), which sometimes can lead to another serious problem named \textbf{sample impoverishment}. In the impoverishment issue, resampled particles fail to cover multiple modes or different spatial regions because dominant particles can not cover the whole distribution landscape. Resampling from deficient yet dominating particles leads to equally unsatisfying outcomes.

In spite of these disadvantages, the particle filter has benefited a wide range of vision applications. Typical examples includes non-rigid object tracking \cite{nummiaro2002color, okuma2004boosted, zhang2017multi, yang2005fast, smith2005using}, simultaneous localization and mapping (SLAM) \cite{fox1999monte, karkus2018particle} and reinforcement learning (maze wondering) \cite{jonschkowski2018differentiable}. 
%Besides the similar tasks that are shared with Kalman filter, particle filter comes with more handy in terms of dealing with non-rigid vision tasks.  

Recall that the Kalman methods update state variables with the residual between prior and true measurements. In other words, there has to be a direct calculating function that transforms states to measurements for prediction and this function needs to be invertible for updates (\ie meansurement matrix, $H$, and its inverse, $H^{T}$, must exist). Notably, however, strong image features are often abstract and beyond coarse physical system measurements, \eg color histograms and motion cues can not be attained through direct projection from image coordinates and yet they can be crucial for recognizing objects under non-stationary conditions like change of view and illumination.
 \begin{figure}[ht]
    \centering
    \begin{minipage}{.15\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/pf_face.png}
    \subcaption{(a)}
    \end{minipage}
    \begin{minipage}{.25\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/face_bin_pf.png}
    \subcaption{(b)}
    \end{minipage}
    \begin{minipage}{.48\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/adaboost_pf.png}
    \subcaption{(c)}
    \end{minipage}
\caption{(a) Particle filter tracking human face with pre-collected human face color-bin as template (b) from \cite{nummiaro2002color}. (c) Multi-target tracking example in a hockey court from \cite{okuma2004boosted}.
Players, indicated by boxes, are captured by the particle filter based on color information.
Figure reproduced from \cite{nummiaro2002color} and \cite{okuma2004boosted}.}
\label{fig:face_pf_tracking}
\end{figure}
Here, the particle filter excels in working with high-level visual features. In the example of human face tracking, 
an approach has integrated color distribution features into a particle filter \cite{nummiaro2002color}; see Figure \ref{fig:face_pf_tracking} (a) and (b).
%K. Nummiaro \etal \cite{nummiaro2002color} integrate reliable color distribution features into particle filter and compare with target template using Bhattacharyya coefficient in Figure \ref{fig:face_pf_tracking}. 
Their system adopted state vectors from physical image space:
$\mathbf{x} = \{ x, y, \hat{x}, \hat{y}, L_{x}, L_{y}, \hat{L}{x}, \hat{L}_{y} \}$, where $x, y$ are image coordinates, $\hat{x}, \hat{y}$ are coordinate changes, $L_{x}, L_{y}$ are lengths of half-axes of an ellipse encompassing the target and their corresponding changes $\hat{L}_{x}, \hat{L}_{y}$. The observation, however, is the RGB color-bin distribution of the predicted ellipse window organized in 8x8x8 bin size. To update, just re-weighting each particle given the groundtruth color distribution is enough. Other such features include 3D keypoints \cite{choi2012robust}, Sobel-Edges \cite{klein2006full, choi20123d}, a combination of contour, texture and shape \cite{pistori2010mice}, and PCA based appearance features \cite{ross2008incremental}.  

The particle filter is also compatible with machine learning techniques \cite{okuma2004boosted, hess2009discriminatively} and recently has been restructured within deep neural networks. Similar to Deep-Kalman counterparts, a learnable particle filter network aims at resolving physical constraints of transition models and encouraging raw images to interact with state functions \cite{jonschkowski2018differentiable, karkus2018particle}.

\section{Gaussian Process}

A Gaussian process (GP) is a collection of random variables, any finite number of which have (consistent) Gaussian distributions. Here, by consistent, we mean for time-series data, a continuous stochastic process along the time-axis, $x_{1:t}$, can be described as a Gaussian process if and only if for every finite set of indices $1, \ldots, t$ in the index set $1, \ldots, T$, $x_{1:t}$ is a multivariate Gaussian random variable. 

A GP model is specified by its mean function, $m(x)$, and covariance function, $k(x, x^{\prime})$, which generate distributions over function $f$ as follows. Let
\begin{equation}
    m(x)  = \mathbb{E}[f(x)],
\end{equation}
\begin{equation}
    k(x, x^{\prime}) = \mathbb{E}[(f(x) - m(x)) (f(x^{\prime}) - m(x^{\prime}))],
\end{equation}
and
\begin{equation}
    f \sim \mathcal{GP}(m(x), k(x, x^{\prime})),
\end{equation}
with $\sim$ indicating generation of distributions over $f$. In the above, $x^\prime$ is used to indicate a different different point from $x$.

Notably, the mean function, $m(x)$, specifies the central value for each index $x_{t}$ whereas the variance indicates the uncertainty. To obtain a smooth trend among adjacent data points, each data point builds up co-occurance relations with all the others using the covariance function $k$. Due to this regularized inner smoothness attribute, the GP model can demonstrate very good \textbf{interpolation} results for unseen data. (An example for video data is shown in Figure \ref{fig:gauss_3dtrack}). Assuming a sequence comprises $n$ elements, its covariance matrix is then an $n \times n$ matrix.

The choice of the covariance function determines how adjacent points follow each other such that the transition can be coherent and smooth (as distinct from some zig-zag tracking results from the Kalman filter). Therefore, potential functions should assign a relatively high $k(x, x^{\prime})$ value for neighboring data.
Popular candidates are constant $k(x, x^{\prime})= C$, linear $k(x, x^{\prime})= x^{T}x$ and Radius Basis Function (RBF) $k(x, x^{\prime})= exp(-\frac{||x - x^{\prime}||^2}{2l^2})$, with $l$ related to the kernel width. Detailed comparison of various covariance functions can be found elsewhere \cite{duvenaud2014automatic}.

A common way to begin a GP model is specifying a prior mean function and a covariance function $k(x, x^{\prime})$ by experience. Most research selects a \textit{zero} mean function as prior and the covariance values are soley decided by the picked function. Sampling from such an initial choice yields unregularized results. 
%In the exmaple of choosing RBF kernel as covariance function in Figure \ref{eq:gp_fit}(a), sampled functions under the "Prior" title demonstrate a large uncertainty as well as roughly zero mean property.

Typically, one is interested in the posterior probability, $p(x|y)$, with $x$ the underlying variable of interest and $y$ the observable. Correspondingly, to instantiate a GP model it must be fit to observed data.
%However, what researchers are interested is the posterior probability $p(x|y)$, with $x$ as the researched random variable and $y$ as the observed target value. 
\iffalse
Assuming the target value $y$ is governed by $x$ and the weight matrix $w$ specified by a prior as
\fi
\iffalse
\begin{equation}
    \begin{aligned}
    y = x^{T} w + \epsilon    \\
    w \sim N(0, \Sigma_{p})
    \end{aligned}
\end{equation}
where $\epsilon$ is the noise.
\fi
\iffalse
\begin{equation}
    p(w | y, x) = \frac{p(y|x, w)p(w)}{p(y|x)}
\end{equation}
\fi
%$One necessary step prior to using Gaussian process is fitting it with real observation data $Y = \{ y_{1}, ..., y_{t} \}$ since the prior distribution for both mean and covariance functions are too coarse to model anything well. Due to the assumption of isotropic Gaussian on each $x$, one can deduct the marginalized distribution $p(X|Y)$ easily in closed form as following:
%So to instantiate a Gaussian process model, it must be fitted with observed data, $\mathbf{y}={y_1\ldots, y_t}$, from the training set. 
Due to the assumption of an isotropic Gaussiann on each $x$, one can deduce the posterior from the distribution marginalization of the joint probability of two Gaussian random variables $p(x, y)$ as
% ref: https://online.stat.psu.edu/stat505/lesson/6/6.1#:~:text=Conditional%20Distribution%20Properties&text=For%20instance%2C%20gives%20the%20means,variances%20and%20covariances%20for%20vector%20.&text=Any%20distribution%20for%20a%20subset,is%20a%20multivariate%20normal%20distribution.;
% proof of conditional gaussian.pdf: http://users.stat.umn.edu/~helwig/notes/norm-Notes.pdf;
\begin{equation}
    \centering
    \begin{aligned}
    &p(x, y) = \mathcal{N} \left(
        \begin{bmatrix}
            \mu_x \\
            \mu_y
        \end{bmatrix}
        ,
        \begin{bmatrix}
            \Sigma_{x}, \Sigma_{xy} \\
            \Sigma_{yx}, \Sigma_{y} \\
        \end{bmatrix}
        \right)\\    
    \end{aligned}
\label{eq:gp_fit}
\end{equation}
and
\begin{equation}
p(x) = \int p(x, y) dy = \mathcal{N} (\mu_x, \Sigma_x)
\label{eq:gp_fit_2}
\end{equation}
so that
\begin{equation}
    p(x|y) = &\frac{p(x, y)}{p(x)} = \mathcal{N}(\mu_{x} + \Sigma_{xy}\Sigma_{y}^{-1}(y-\mu_{y}), \;\;\; \Sigma_{x} - \Sigma_{xy}\Sigma_{y}^{-1}\Sigma_{xy}^{T}),
\label{eq:gp_fit_3}
\end{equation}
where $\mu_x$ and $\mu_y$ are mean values for prior and observations, respectively, and $\Sigma$ symbolizes the various covariance matrices defined by $k(x,x^\prime)$.
%$\Sigma$ is the covariance matrix defined by the covariance function $k(x, x^{\prime})$.

The middle figure in Figure \ref{fig:gp_demo} demonstrates samples from a trained posterior. In comparison with the ``Prior", the posterior shows fixed target values at trained data points (\ie at position $(x=2, y=1)$), the function looses uncertainty, meaning at this point its variance becomes zero). 
Following a similar idea, the calculation of posterior density of any \textbf{test point} $x_{\ast}$ (also known as the \textbf{predictive posterior} on unseen points) from a pre-trained model is tractable \cite{rasmussen2003gaussian}.
\iffalse
\begin{equation}
    p(f_{\ast} | x_{\ast}, y, x) = \mathcal{N}(\mu_{\ast}, \Sigma_{\ast}) = \mathcal{N}(k_{\ast}k_{-1}\mathbf{y}, k_{\ast\ast} - k_{\ast}k_{-1}k_{T}),
\end{equation}
\begin{equation}
    p(f_{\ast} | x_{\ast}, y, x) = \mathcal{N}(\mu_{\ast}, \Sigma_{\ast}) = \mathcal{N}(k_{\ast}k^{-1}\mathbf{y}, k_{\ast\ast} - k_{\ast}k^{-1}k^{T}),
\end{equation}
where $k_{\ast} = \{k(x_{\ast},x_{1}), k(x_{\ast},x_{2}), ..., k(x_{\ast},x_{t}) \}$, $k_{\ast\ast} = k(x_{\ast}, x_{\ast})$ and $k = \{k(x, x^{\ast}) \}$
\fi

\begin{figure}[ht]
    \centering
    \includegraphics[width=.8\textwidth]{Figures/gp.png}
    \caption{Gaussian process intuition. (Left) Given an initial (prior) GP model with $x$ being a random variable and $x \sim \mathcal{N}(0, \sigma)$, multiple distinct functions can be sampled. After trained with a real value dataset, $\mathbf{y}$, the posterior of a GP model is much confined at trained data positions (middle). (Right) The fit model can be used for performing regression with uncertainty. Seeing the x-axis as temporal stamps would naturally fit time-series data.} 
    \label{fig:gp_demo}
\end{figure} 

The application of the GP to video understanding tasks can be categorized into two main classes: \textbf{1.} static temporal process modelling and \textbf{2.} dynamic state-space modelling. 
%The first one coincides with the origin intention of inventing GP which is serving accurate non-linear regression. It focuses on fitting video data representation into GP model by reckoning the feature at each time-stamp $f_{t}$ as GP random variable. The fitted model is useful in terms of video sequence matching, anomaly detection and classification \cite{cheng2015video, kim2011gaussian, altun2004gaussian, li2015anomaly,cheng2015gaussian}.
The first coincides with the originally intended application of GPs, serving accurate nonlinear regression \cite{rasmussen2003gaussian}. In application to video, the focus is on using the model to represent a visual feature value, $f_t$, at each time, $t$, according to a GP model. Example video applications include video sequence matching, anomaly detection and classification \cite{cheng2015video, kim2011gaussian, altun2004gaussian, li2015anomaly,cheng2015gaussian}.

Another line of research incorporates GPs with state space dynamic models. As mentioned above, a vanilla Gaussian process links neighboring data points using a distance based covariance matrix (\eg an RBF kernel), which does not emphasizes any \textit{causal} relations among data points but accents on the aggregated group effect. In contrast, the Bayesian recursive filter advocates state transition functions to support information propagation to be made about future data. A dynamic function matters particularly for extrapolation tasks, which otherwise would only degrade to the prior mean value of the GP model.

To harvest the advantages of state space domain knowledge, the combination of GPs with Markov dynamic systems has been explored extensively, \eg \cite{ko2009gp, girard2003gaussian, ellis2009modelling, wang2006gaussian, urtasun20063d, wang2007gaussian, lee2016predicting, damianou2011variational}. The core of the compound is assisting GP models with latent state dynamics. 
%Once again, the state transition and observation measurement functions need to be specified. 
In this literature, a research direction formulated the desired dynamical function with GP regressions and the overall framework is referred to as Gaussian process dynamic models (GPDM) \cite{wang2006gaussian, urtasun20063d}.
As a specific example, a linear transition model, $m(x) = wx + b$, was used with a GP model to predict player reactions from American football clips \cite{lee2016predicting}. Input to the system was a sequence of trajectory features extracted from video of players and the GP model was used to regress activity labels, with the values for the parameters, $w$ and $b$, estimated via gradient descent. Other work has incorporated more complicated dynamic models (\eg another GP model that comprises linear and RBF kernels \cite{urtasun20063d}) with application to a wide variety of tasks, including human motion interpolation \cite{wang2006gaussian}, 3D people tracking \cite{urtasun20063d} and pedestrian trajectory prediction \cite{ellis2009modelling}. The latent variable is often initialized as the output from PCA dimension reduction on visual features (\eg body keypoints in \cite{urtasun20063d}) and parameters are learned via a maximum a posteriori solution.
An example applying GPDM to human tracking is shown in Figure \ref{fig:gauss_3dtrack}.

%In response, Lee \etal \cite{lee2016predicting} adopted linear transition model ($m(x) = wx + b$) for their GP model to predict the players' reactions from American football clips. They inputs a sequence of features extracted from target players and model its regression to desired labels with GP. The parameters $\{w, b\}$ is estimated with gradient descent optimization. Other work coins a set of latent states with probabilistic PCA \cite{tipping1999probabilistic, lawrence2004gaussian} from training observations and formulate their dynamic with a separate GP model. The specific dynamic of latent states is characterized through its covariance matrix. An example of such model from \cite{urtasun20063d} is as: $k(x, x^{\prime}) = exp(-\frac{|| x - x^{\prime} ||^{2}}{2l^{2}}) + x^{T}x^{\prime}$, namely a combination of Linear and RBF kernel (For extrapolations beyond training index range (0, t), $x_{t+1}$ will be decided only from early elements using this kernel combination). This technique is  phrased as Gaussian process dynamic model (GPDM), based on which some respectable applications have been built, such as human motion interpolation \cite{wang2007gaussian}, 3D people tracking \cite{urtasun20063d} and long-term pedestrian trajectory prediction \cite{ellis2009modelling}.

One unignorable disadvantage of the GP model is that it can not scale up to large sample size with ease. Since each data point will be modeled as a Gaussian, a series of spatiotemporal features with feature dimension in $\mathbb{R}^d$ and temporal scope $k$ would result in $k \times d$ multivariate Gaussians. Its covariance matrix thus ends up with $k \times k \times d$ elements, which is prohibitive under current parameter estimation literature for large $k$ and $d$.

Moreover, to estimate any involved parameter, \ie the length scale parameter of the RBF kernel for $k(x, x^{\prime})$ or the general fitting process, the space and time complexity is $\mathcal{O}(N^{3})$ (with $N$ the dataset size). Recently, some research has sought remedies for these limitations via machine learning \cite{damianou2013deep, lu2020interpretable, liu2020gaussian}; however, the applications were not to visual tasks.
%researcher seek a remedy in machine learning and deep learning \cite{damianou2013deep, lu2020interpretable,liu2020gaussian} but none has a focus on video visions. 
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.\textwidth]{Figures/gp_3dtrack.png}
    \caption{3D human tracking from GPDM \cite{urtasun20063d} that interpolates the occluded frame. During interpolation, the body part exhibits natural and non-rigid movement trajectory. Figure reproduced from \cite{urtasun20063d}.}
    \label{fig:gauss_3dtrack}
\end{figure}

\section{Auto Regressive Model}
The idea of an Auto-Regressive (AR) model is to capture the auto-correlation of sequential data in a regression type model and use it to improve short-term forecasts. Its key concept is the \textbf{order} of the AR model. 
The auto-regressive model can be formally expressed as
\begin{equation}
    y_{t} = \beta_{0} + \beta_{1}y_{t-1} + \beta_{1}y_{t-2}, ..., + \beta_{t}y_{t-n} + \epsilon_{t},
\label{eq:AR}
\end{equation}
where $\beta_{t}$ is the $n_{th}$ coefficient for the corresponding delay tap version of the series data, $y_{t-n}$, and $\epsilon_{t}$ is the noise signal at the current time-step. One important assumption under the AR model is the \textbf{stationary} property, whereby statistical properties such as mean, variance, auto-correlation, etc., are all constant over time.

In the above formula, lagged data points ranging from $(t-1, t-n)$ are used to infer the data value at point $t$ and therefore it is defined as an AR model of order $n$, or an $AR(n)$ model. The order term corresponds to the same concept from higher-order Markov chains. AR is a sub-class of regression models and can be estimated through various methods such as least-squares, Maximum Likelihood \cite{doretto2003editable}, Yule-Walker equation \cite{doretto2003dynamic} or Maximum Entropy Spectral Analysis (MESA) \cite{burg1974maximum}.

In the field of video sequence analysis, \textbf{dynamic texture} \cite{doretto2003dynamic} data has been argued to have the required stationary property. Running water, flying flags or flickering flame can be viewed as stationary data in the spatiotemporal domain in the sense that they exhibit certain periodic patterns in visual spacetime. Since such patterns are pervasive in real-world videos, models of dynamic texture have been widely investigated for purposes of both analysis and synthesis. Considerable work in this area has relied on AR analytic tools \cite{cliff1975space, doretto2003dynamic,wang2002generative, hyndman2007higher, doretto2003editable, murdock2015building}. Though they differ slightly in processing of the raw image (\eg working on input pixel values \cite{cliff1975space}, PCA features \cite{hyndman2007higher}, Gabor/Laplacian decompositions \cite{wang2002generative}), all have adopted AR of various orders to model state dynamics. Figure \ref{fig:ar_dt} provides an illustrative example.
Of course, the stationary limitation makes the synthesis of video sequences that are parting from dynamic textures sub-optimal. 
Even for dynamic textures, it appears that such models tend to emphasize spatial appearance at the expense of temporal dynamics \cite{woolfe2006shift}.
Likely for these reasons, AR models are less popular than others for video prediction and synthesis.
%In the task of common video prediction or generation, AR appears much less frequently than others (See Section 3.1).  

%A. Cliff \etal \cite{cliff1975space} work on pixels, M. Hyndman \etal \cite{hyndman2007higher} work on low-dimensional PCA features and Y. Wang \etal \cite{wang2002generative} on Gabor/Laplacian decompositions), all have adopted AR for state dynamics, either in lower or higher order.
%Modelling the progression of these dynamic texture attracts attentions and AR has been found applicable for synthesizing texture movements.
\begin{figure}[ht]
    \centering
    \includegraphics[width=.8\textwidth]{Figures/ar_dt.png}
\caption{Dynamic texture example of flicking fire synthesized using higher-order AR model \cite{hyndman2007higher}. To grab a robust as well as sparse representation of frame sequences, an appearance vector of frames is obtained through principle component analysis. 
The feature dynamics are modelled as an AR process.
Figure reproduced from \cite{hyndman2007higher}.}
\label{fig:ar_dt}
\end{figure} 

\section{Recurrent Neural Networks}
In this section, we describe a type of neural network that was invented for processing sequential data, Recurrent Neural Networks (RNNs) \cite{bengio1994learning}. Artificial neurons (\eg perceptrons) are designed with inspiration from biological neurons \cite{hasson2020direct}. In essence, they follow linear combination of their inputs with various nonlinearities (\eg rectifiers, sigmoids and normalizations). Neural networks consisting of multiple layers of such neurons are devised to solve a wide variety of complicated tasks, especially those commonly associated with human intelligence. Regular NNs are feed-forward, namely a collection of directed neurons transforming the input to output without looking back, \ie they can be thought of as directed acyclic computational graphs.

In contrast, RNNs borrow power from recurrently updated hidden states to better capture inner dynamics of sequential data. Their mathematical formulation can be given as:
\begin{equation}
    h_{t} = \sigma ( {W}_{x} x_{t} +  {W}_{h} h_{t-1} + b_{h}),
\label{eq:rnn_1}
\end{equation}
so that
\begin{equation}
    y_{t} = \sigma ({W}_{y} h_{t} + b_{y}),
\label{eq:rnn_2}
\end{equation}
where ${W}_{x}, {W}_{y}, {W}_{h}$ are mapping matrices for the input, $x_{t}$, 
%output $y_{t}$ and hidden state $h_{t}$. $\sigma$ is nonlinear activation function, \ie Sigmoid, Tanh or ReLU, which allows more complicated transition for output and hidden states.
$y_t$ is the output, $h_t$ is the hidden state, $b_y$ and $b_h$ are additive biases and $\sigma$ is a nonlinear activation function (e.g., sigmoid, Tanh or ReLU) allowing for complicated transitions between output and hidden states. Figure \ref{fig:fn_rnn} provides an illustration and comparison to purely feed-forward networks.

\begin{figure}[ht]
    \centering
    \begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/fn_rnn.png}
    \subcaption{(a)}
    \end{minipage}
    \hfill
    \begin{minipage}{.5\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/rnn.pdf}
    \subcaption{(b)}
    \end{minipage}
\caption{(a) Depiction of the difference between feed-forward and recurrent neural networks; (b) Unrolled computational procedure of RNNs.}
\label{fig:fn_rnn}
\end{figure}

Given a sequence of input data $x_{1:T}$, the hidden state $h_{t}$ is consistently refreshed with new incoming input and the inference for output depends on the up-till-now hidden state. This particular module is referred to as a \textbf{memory} unit since it stores historical information in hidden states. In comparison, Bayesian filters and HMMs also belong to memory type models, whereas auto-regressive models and Markov Chain models are categorized as \textbf{memoryless}, since their inference relies on limited past input without updating states.

Furthermore, RNNs differ from Bayesian filters and HMMs in that their states are deterministic rather than stochastic. Some would argue that the deterministic property relaxes the trouble of inferring the hidden state and is more efficient \cite{hochreiter1997long}. The cost is that we would never know the exact state. From the perspective of recursive inference, the RNN is akin much more to the Bayesian filter in allowing for variable input and output length.

With the back-propagation algorithm being a powerful optimization tool for feed-forward NNs \cite{goodfellow2016deep}, RNNs rely on its temporal version, Back-Propagation Through Time (BPTT) to estimate the parameters. However, training RNNs is not always simple. Since the transition matrices ${W}_{x}, {W}_{y}$ and ${W}_{h}$ are shared among all time stamps, RNNs would multiply the same matrices $N$ times ($N$ is the data length) so that the output $y_{t} \propto {W}_{h}^{(N)}$, meaning that the output is proportional to the power $N$ of matrix ${W}_{h}$. During back-propagation, \textbf{gradient vanishing} or \textbf{gradient explosion} thereby happens for small values or large values in the matrix, ${W}_{h}$, respectively.

To counter the difficulity in the training, the Long-Short Term Memory \cite{hochreiter1997long} (LSTM) unit is introduced. The LSTM architecture consists of a set of recurrently connected subnets, known as memory blocks. These blocks can be thought of as a differentiable version of the memory chips in a digital computer. Each block contains one or more self-connected memory cells and three multiplicative units (forget gate $\mathbf{f}_{t}$, output gate $\mathbf{o}_{t}$ and input gate $\mathbf{i}_{t}$) that provide continuous analogues of reset, write and read operations for the cells $\mathbf{c}_{t}$ and output state $\mathbf{h}_{t}$. Figure \ref{fig:lstm} provides an architectural diagram and supporting formulae.
Note that the LSTM equations here match the vanilla RNN equations (\eg Eq. \ref{eq:rnn_1} and \ref{eq:rnn_2}) since
\begin{equation}
\begin{aligned}
     h_t &= o_{t} \circ \sigma_h (c_{t}) \\
         &= f_{t} \circ c_{t-1} + \sigma_g ({W}_{i} x_{t} + {U}_{i} h_{t-1} + b_{i}) \circ \sigma_c ({W}_{c} x_{t} + {U}_{c} h_{t-1} + b_{c}),
\end{aligned}
\end{equation}
which represents a compound mapping function: $(x_t, h_{t-1}) \rightarrow h_t$. Moreover, the mapping from hidden states to desired outputs, $h_t \rightarrow y_t$ in RNN equation \ref{eq:rnn_2}, is often neglected in the LSTM.
\begin{figure}
\begin{minipage}{.5\textwidth}
    \centering
    \includegraphics[width=.85\textwidth]{Figures/lstm.jpg}
\end{minipage}
\begin{minipage}{.45\textwidth}
\begin{flushright}
\begin{math}
\begin{aligned}
  f_{t} &= \sigma_g ({W}_{f} x_{t} + {U}_{f} h_{t-1} + b_{f}) \\
  i_{t} &= \sigma_g ({W}_{i} x_{t} + {U}_{i} h_{t-1} + b_{i}) \\
  o_{t} &= \sigma_g ({W}_{o} x_{t} + {U}_{o} h_{t-1} + b_{o}) \\
  \Tilde{c}_{t} &= \sigma_c ({W}_{c} x_{t} + {U}_{c} h_{t-1} + b_{c}) \\
  c_{t} &= f_{t} \circ c_{t-1} + i_{t} \circ \Tilde{c}_{t} \\
  h_{t} &= o_{t} \circ \sigma_h (c_{t})
\end{aligned}
\end{math}
\end{flushright}
\end{minipage}
\caption{Diagram of Long-Short Term Memory unit and its operating equations. Figure reproduced from \cite{45500}.}
\label{fig:lstm}
\end{figure}
%y_{t} &= \sigma ({W_y} h_{t} + b_y)

At every time step in LSTM processing, memory cell, $\mathbf{c}_{t}$, is decided by: \textbf{1.} the Hadamard product, $\circ$, between forget gate, $\mathbf{o}_{t}$, and previous cell memory, $\mathbf{c}_{t-1}$; \textbf{2.} the same product between the input gate, $i_{t}$, and cell activation vector, $\Tilde{\mathbf{c}}_{t}$. The reason why LSTMs can mitigate gradient problems is that the switching induced by the activation of gating functions turns the multiplicative chain into an addition chain. For example, when the input gate is closed for most elements, the update memory, $\mathbf{c}_{t}$, would be largely dependent on the previous cell state; on the other hand, when the input gate is mostly open, $\mathbf{c}_{t}$ would be the addition of previous cell values and the incoming input. In both cases, the matrix multiplication is largely avoided. A Gated Recurrent Unit network (GRU) \cite{cho2014learning} shares a similar intuition, but merges the memory cell with the state vector.

%\textbf{Application:} Present days, video vision research have been greatly relying on RNN and its variants. For unsupersively learning a strong video representation, N. Srivastava \etal \cite{srivastava2015unsupervised} adopted LSTM on sports videos (UCF-101 \cite{soomro2012ucf101}) to extrapolate unseen feature sequences and use the predictive representation to obtain comparable results. X. Shi \etal \cite{xingjian2015convolutional} incorporate convolutional layers with LSTM that allows patch-wise memory information propagation. Pedestrian trajectory predictions mainly utilizes RNNs to extrapolate potential future 2D coordinate from partial observations \cite{alahi2016social, gupta2018social}. Semantic activity anticipation \cite{abu2018will, ke2019time, zhaodiverse}. Video caption generation \cite{pei2019memory}. 

Recent research in video understanding has relied greatly on RNNs and its variants. As examples: An LSTM has been applied to sports videos (UCF-101 \cite{soomro2012ucf101}) to extrapolate unseen feature sequences \cite{srivastava2015unsupervised}; LSTMs have been agumented with convolutional layers for patch-wise memory information propagation \cite{xingjian2015convolutional}; RNNs have been used for pedestrian trajectory predictions as extrapolations from partial observations \cite{alahi2016social, gupta2018social}. Additional work leveraging RNNs for video understanding includes applications to semantic activity anticipation \cite{abu2018will, ke2019time, zhaodiverse} and caption generation \cite{pei2019memory}. Thus, applications of RNNs to video understanding have spanned relatively early vision numerical extrapolation tasks to high level semantic tasks.

\section{Summary}
All of the techniques overviewed in this chapter have seen some degree of use in video predictive understanding. Following trends elsewhere in computer vision, recent work has especially made use of neural network based approaches, with a particular emphasis on RNNs, as well as combined more classical techniques with such networks. In the next chapter, we shall see how these techniques have been applied to early action recognition and future action prediction.

==> BODY/Backup/chapter2.tex <==
\section{Overview}\label{Sec:early_actio}
One extensively investigated sub-area of video predictive understanding is early action recognition. Its core mission is to recognizing actions while they are still evolving and predicting the correct action labels as early as possible, as illustrated in Figure \ref{fig:action_prediction}.
\begin{figure}[htb]
    \centering
    %\resizebox{.5\linewidth}{!}{\includegraphics[width=4cm]{Figures/action_prediction2.PNG}}
    \resizebox{.75\linewidth}{!}{\includegraphics{Figures/problem_fig.pdf}}
    \caption[The definition of early action recognition.]{(Left) The definition of early action recognition from \cite{ryoo2011human}. Preliminary observations of a particular ongoing action clip are used as input to generate the corresponding class label. Figure modified with permission from \cite{ryoo2011human}. (Right) Illustration of three major perspectives in current literature to tackle early action recognition: One-shot mapping, knowledge distillation and propagation.}
    \label{fig:action_prediction}
\end{figure}

Formally, the problem can be defined as: Given a sequence of action video frame observations $y_{1:T}$ and its semantic label $\mathcal{X}$, where $1$ and $T$ represent the starting and ending indices of action frames, define a function $f : y_{1:t} \rightarrow \mathcal{X}$, which maps various partial segments $y_{1:t}$ to the groundtruth label domain. In particular, it is favorable to have high recognition performance on relatively small frame index (\ie $t \rightarrow 0$), meaning that the algorithm is able to recognize actions correctly with very limited initial observations.

Apparently, there is a fundamental assumption behind this problem setting: The full action sequence supports superior recognition compared to observation of only an initial segment, otherwise the problem is unnecessary. To validate this assumption, the original advocate of this research direction, M. S. Ryoo, conducted a series of experiments that operated existing action recognition algorithms on various partial action clip segments (\ie $y_{1:t}, t \in (1, \ldots, T)$) and demonstrated that insufficient observations in action temporal scope resulted in much inferior recognition accuracy \cite{ryoo2011human}. Also, as a visual example, the partial observation in Figure \ref{fig:action_prediction} (bottom row) can be sensibly categorized into \textbf{pushing} or \textbf{hugging} with equal chance, whereas the full action sequence (top row) reveals high likelihood for \textbf{pushing}.

Follow on work defined a systematic evaluation procedure for early action recognition \cite{kong2014discriminative}: Uniformly divide a full video $y_{1:T}$ into $K$ segments $y[\frac{T}{K}(k-1) +1, \frac{T}{K}(k)]$ where $k = 1, ..., K$ is the index of the segment. The length of each segment is $\frac{T}{K}$ and different videos usually have separate segment lengths. Thus, a partial observed video sequence can be described as $y[1, \frac{T}{K}(k)]$ and recognition accuracy at all possible $k$ should be reported (\eg they pre-define $K=10$ and report 10 sets of accuracies). The majority of successive work follows this paradigm.

In the last decade, researchers approach this task from various perspectives and hereby we group them into three major divisions: \textbf{1.} formulating one-shot mappings from partial observations to groundtruth labels of full observations; \textbf{2.} distilling the information from the full action clip observations into partial observations; \textbf{3.} propagating the limited partial information into the future in a temporal extrapolation fashion. In the following sections, we review all recent research according to these divisions.

\section{One-Shot Mapping Based}
The basic assumption underlying one-shot mapping based approaches is that a partial observation of an action video provides sufficient information in and of itself to define the appropriate overall action class regardless of the unobserved clip portions. What appears to be the first work along these lines \cite{ryoo2011human} made use of sequential feature matching with an Integral Bag-of-Word (IBoW) representation \cite{sivic2008efficient}. The intuition being that the feature distributions of partial and complete action clips should be similar, if they derive from the same action. To avoid inefficiencies that would result from training classifiers for each temporal segment, they initially extract Spatio-Temporal Interest Point features (STIP \cite{laptev2005space}) from raw videos and re-organize them into visual word histograms (IBoW) according to color distributions. Then, a Gaussian kernel matching function is used to generate a probability score representing the likelihood between partial and whole observations. Finally, the selected class label is that of the full action that produces the largest likelihood. As illustrated in Figure \ref{fig:stip_bow_hist}, for each action segment, a color histogram is calculated. Similar work improved the feature representation as well as selection with sparse coding but shared the overall structure \cite{cao2013recognize}. 

\begin{figure}[ht]
    \centering
    \begin{minipage}{.52\textwidth}
        \centering
        \includegraphics[width=1.\textwidth]{Figures/ryoo_2.png}
        %\subcaption{(a)}
        \caption*{(a)}
    \end{minipage}
    \begin{minipage}{.38\textwidth}
        \centering
        \includegraphics[width=1.\textwidth]{Figures/stip_bow_histogram.png}
    %\subcaption{(b)}
        \caption*{(b)}
    \end{minipage}
\caption[STIP features from videos and clustered results by color for each frame]{(a) STIP features from videos and clustered results by color for each frame. (b) Demonstration of Integral Bag-of-Word (IBOW) used in \cite{ryoo2011human}. For each time step, its feature histogram amasses all previous observations. Figure reproduced with permission from \cite{ryoo2011human}.}
\label{fig:stip_bow_hist}
\end{figure}

While the IBoW approach supports fast inference and is learning free, it operates under two restrictive assumptions. First, the feature extractor, STIP, yields an appearance based feature descriptor (indeed STIP comes from spacetime Harris-corner detection \cite{harris1988combined}), which is sensitive to view changes, illumination and other nuisance details of image acquisition. Thus, targets from the same action category are assumed to be similar in appearance. Second, the scheme to matching feature histograms between partial and full actions is not always practical since actions can evolve dramatically, to the extent that the beginning appears totally unlike the ending.

Subsequent work following essentially the same framework improved on the original by employing stronger features as well as more sophisticated machine learning-based classifiers \cite{lan2014hierarchical}. More specifically, the feature representation was enhanced by merging motion descriptors (iDT \cite{wang2013action}) with appearance descriptors (HOG \cite{dalal2005histograms}). Furthermore, to capture the human movements at all levels, they proposed an approach to capture features at three hierarchical temporal scales: a coarse level feature that processes generic videos by taking frames as a whole; a mid-level feature that captures viewpoint specific information by extracting features only belonging to certain specific actors (\eg \textit{level2}, focuses on regions that are pre-clustered by different human actor appearances); a fine-grained movement level that captures pose specific information (\eg \textit{level3} extracts features only from regions that share the same actor appearance \textit{and} pose type, which is again obtained by clustering). To finally assign class labels to given video clips, the authors adopted Support Vector Machines (SVMs) \cite{cortes1995support} that were trained on features from all three levels to jointly make the decision.

Though this relatively new and detailed approach advanced its predecessors through adopting stronger features, hierarchical extractions and learning-based classifiers, it still relied on the assumption that fine grained analysis of an initial partial observation can bridge the past and future. A notable downside to this particular extension is that it relied on clustering algorithms for grouping actors and poses \cite{lan2014hierarchical}, which can be noisy (\eg it is sensitive to the color of clothing).

\iffalse
\begin{figure}[ht]
    \begin{minipage}{.375\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/herichical_repre_future_action_pred.PNG}
    \subcaption{(a)}
    \end{minipage}
    \begin{minipage}{.625\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/action_tube.png}
    \subcaption{(b)}
    \end{minipage}
\caption[Two examples of exploring fine-grained action evolution for early action prediction.]{Two examples of exploring fine-grained action evolution for early action prediction. Subfigure (a) depicts the hierarchical representation of human actors in \cite{lan2014hierarchical} and subfigure (b) showcases the actor detector integrated framework from \cite{singh2017online}. Subfigures reproduced with permission from \cite{lan2014hierarchical} and \cite{singh2017online}, respectively.}
\label{fig:fine-grained}
\end{figure}
\fi

\iffalse
\begin{figure}[htp]
\centering
\subfloat{%
  \centering
  \includegraphics[clip,width=.7\columnwidth]{Figures/herichical_repre_future_action_pred.PNG}%
}
\subcaption{(a)}

\subfloat{%
  \centering
  \includegraphics[clip,width=.7\columnwidth]{Figures/action_tube.png}%
}
\subcaption{(b)}
\caption{Two examples of exploring fine-grained action evolution for early action prediction. Subfigure (a) depicts the hierarchical representation of human actors in \cite{lan2014hierarchical} and subfigure (b) showcases the actor detector integrated framework from \cite{singh2017online}.}
\label{fig:fine-grained}
\end{figure}
\fi

Subsequent work \cite{singh2017online} disposed of unsupervised clustering for detection of actors and their poses by instead making use of object/human detectors pretrained on massive datasets (\eg SSD \cite{liu2016ssd}). Therefore, they proposed to jointly perform action localization as well as action early recognition, based on the assumption that actions only associate with behaviors of human actors, and called the detected actor regions \textbf{action tubes} (\ie bounding box coordinates of detected actors). For given frames, this approach generates bounding box regions together with class labels for all possible regions within each frame 
%(\eg second example in Figure \ref{fig:fine-grained}) 
and rejects negative bounding boxes by matching its Intersection Over Union (IOU) with selected regions from previous frames. Since the approach can consume frames online, early action recognition is naturally decided by the classification result from contemporary observations. 

Arguably, human active regions (\eg \cite{lan2014hierarchical, singh2017online}) are still very coarse if being compared with human skeleton analysis \cite{xia2012view} where each body part (\eg arms, elbows, shoulders etc.) is spatially spotted and used. Correspondingly, other work \cite{chen2018part} has suggested to first use human body key-point extraction tools to locate an actor's body structure information and select the salient body feature parts for early action recognition, with a reinforcement policy learning \cite{mnih2015human} function for performing the selection. 
Along similar lines, research using 3D body skeleton analysis for early action recognition has focused on adaptively selecting the best historical information window for predictions in data-driven fashion \cite{liu2018ssnet}.

Notably, the above reviewed works are mostly actor centric, i.e., they base their inference on analysis of the actor alone, with little regard for other objects and scene context. In contrast, a recent effort has instead considered object centric human actions (e.g., fetching objects or moving something to somewhere) \cite{zhou2018temporal}. This work reckoned that the key to reasoning about complex activities is the pattern of temporal developments between subactions and/or objects at various scales, something that was not modeled explicitly in previous work.
In particular, the authors built a ConvNet to perform feature extractions and 2-layer MLPs to capture frame-wise temporal relations. More specifically, multiple sets of frames sampled from various temporal scales are combined together as the final representation to classify. For example, the collection of frame index groups $(1,9)$, $(2, 5, 9, 12)$ and $(1,4,10)$ represent three sets of temporal relations where states of object or actor (\ie human hand in Figure \ref{fig:temporal_reasoning}) transit differently in both speeds and conditions. 
\begin{figure}[htb]
    \centering
    \resizebox{.8\linewidth}{!}{\includegraphics[width=4cm]{Figures/temporal_reasoning.png}}
    \caption[Example of temporal relation reasoning for early action recognition.]{Example of temporal relation reasoning through sampling frames with multi-scale time intervals \cite{zhou2018temporal}. Frame group $(1,9)$ denotes the relation \textbf{put next to} whereas group $(1, 4, 10)$ denotes the \textbf{take-away} relation. Considering all sub-relations leads to the inference of the action label. Figure reproduced with permission from \cite{zhou2018temporal}.}
    \label{fig:temporal_reasoning}
\end{figure}

While the above approach reasons about temporal relations, it aggregates frame-wise information globally and thereby does not exploit spatial relations of elements within a single frame. More recent work has extended this principle to the spatial dimension \cite{sun2019relational}. Similar to \cite{singh2017online}, it used a learning based detector to generate actor proposals for all characters in one frame. The relation between multiple actors is modeled as nodes and edges as in a graph \cite{santoro2017simple} and a Graph Neural Network (GNN) \cite{hamilton2017representation} is adopted to diffuse information among nodes. Following this direction, a multi-scale spatio-temporal graph based method further explores fine-grained human-to-human and human-to-object interactions for this task \cite{wu2021spatial}.

Finally, some other work considers early action prediction as a special case of action recognition in that only a few action clips that are easily differentiable under full observations become difficult when incomplete. To deal with such difficult cases, they equipped the regular recognition framework with an extra memory module to log hard examples explicitly \cite{kong2018action}. 



\section{Knowledge distillation Based}
Methods in the previous section mainly focus on reasoning about the future directly from the past. The future unobserved information provides negligible contribution to the partially observed information, except the overall action label being used for training. Here, it is worth remembering that previous work has shown that full observation almost always excels over the partial and no one has forbidden the use of unobserved information in training \cite{ryoo2011human}. The more urgent question concerns \textit{how} to use such unobserved information.
Hereby, we discuss research that attempts to lend power from unobserved data in training in order to either enrich the feature representation of partial data or encourage the classifiers to recognize partial data with ease.
%the information entropy between partial and full observations, or in another word, increases their mutual information. 
\begin{figure}[htb]
    \centering
    \resizebox{.7\linewidth}{!}{\includegraphics[width=4cm]{Figures/yukong_2014.pdf}}
    \caption[Temporal action evolution patterns for early action recognition.]{
   Temporal action evolution patterns can be enforced through a score function \cite{kong2014discriminative}, as given in Equation \ref{eq:kong14}. Classifiers may work better with partial videos by considering its ranking score with full videos. Figure modified with permission from \cite{kong2014discriminative}.
   }
    %Illustration of the key idea of \cite{kong2014discriminative}: Temporal action evolution patterns can be enforced through a score function. Classifiers (SSVM) would know better of partial videos through its score ranking relation with full videos.}
    \label{fig:kong2014}
\end{figure}

Initial work that informally considered mutual information in early action recognition trained video segment classifiers that align the temporal order of partial observations to training data \cite{kong2014discriminative,kong2015max}. They achieved this result by using a Structured SVM (SSVM) \cite{tsochantaridis2005large}. More specifically, they evenly divided action videos into equal-length segments, extracted features from each segment, integrated segments into one chunk, such as $y_{1:k}$, and trained SSVM classifiers according to the following constraints (without loss of generality, two progress levels ($k-1, k$) is given):
\begin{equation}
    \alpha^{T}_{k-1}\psi_{1}(y_{1:k-1}, x) \leqslant \alpha^{T}_{k}\psi_{1}(y_{1:k}, x),
\label{eq:kong14}
\end{equation}
where $y_{1:k}$ is the video segment feature accumulated from the very begining till the $k_{th}$ level, $x$ is the groundtruth label, $\alpha^{T}_{k}$ is the score matrix for progress level $k$ and $\psi_{1}(y_{1:k}, x)$ is a joint feature map that represents the spatio-temporal features of action label, $x$, given a partial video $y_{1:k}$. The authors assumed 10 progress levels, such that $k \in (1, 10)$.

The above formulation emphasized temporal label consistency: Besides assigning a correct class label to given input videos, classifiers also need to capture the temporal evolution of actions by monotonically increasing the score for segments across time (first seen in early event detection \cite{hoai2014max}). The intuition coincides with daily human experiences: As we see more, we should know better than before. Some other work follows a similar intuition and built their early activity detection model based on ranking loss \cite{ma2016learning}. It also has been proposed to incorporate global human intentions as a complimentary learning objective to assist partial observation learning, but for action prediction in first-person-view videos \cite{ryoo2015robot}. One particular work further argued for assigning various weights for features from every progress level and suggested using temporal saliency to locate the corresponding weights \cite{lai2017global}. Also, other work adopted the same monotonicity constraints and grounded the feature aggregation on human poses \cite{raptis2013poselet}. Finally, an effort focused on refining the classification confidence score at each time-step in an incremental manner \cite{hou2020confidence}. That work relied on an attention mechanism to provoke high confidence on early observations.
Notably, all these efforts differ from methods in the previous section in that unobserved data gets involved to empower the partial data during training.

Yet another approach to using a scoring function was proposed by the originators of this direction for early action recognition \cite{kong2014discriminative}. In this alternative approach the attempt was made to infer complete future features from partial observations \cite{kong2017deep}, something not previously attempted in early action recognition. Their work supposes that we have features of partial observation, $g(y_{1:t})$, and full observation, $g(y_{1:T})$ ($t \in (1, \ldots, T)$), in the training stage, and proposed to reconstruct the full from partial according to:
\begin{equation}
    \operatorname*{argmin}_{W, \theta} || g(y_{1:T}, \theta)  - W g(y_{1:t}, \theta)||^{2},
\label{eq:deepscn}
\end{equation}
where $W$ is the feature transformation matrix and $g(y, \theta)$ is the feature extraction function with parameter $\theta$. As shown in Figure \ref{fig:deep_scn}, raw partial observations (\eg riding on trails with green grass background) could be mixed with any other actions that share the similar background context (\eg golfing or swimming in pools aside the lawn). Transforming the partial into full observations at the feature level helps differentiate between the possibilities (\ie capturing more details of the bicycle structure as well as human riding motions).

\begin{figure}[htb]
    \centering
    \resizebox{.65\linewidth}{!}{\includegraphics[width=4cm]{Figures/deep_scn2.png}}
    \caption[Illustration of the feature transformation approach.]{Illustration of the feature transformation approach of \cite{kong2017deep}. Raw incomplete features are transformed into features from the fully-observed to gain more discriminative information. Figure reproduced  with permission from \cite{kong2017deep}.}
    \label{fig:deep_scn}
\end{figure} 

In implementation, the state-of-the-art 3D CNN video features (\ie C3D \cite{tran2015learning}) were employed for $g$ and the transformation matrix, $W$, was learned. A downside of this approach is that multiple transformation matrices needed to be learned, i.e., one for each $k$. A more recent upgrade on this work \cite{kong2018adversarial} overcame this concern by converting the deterministic feature transformation process \cite{kong2017deep} to a conditional generative process, with an adversarial learning component \cite{goodfellow2014generative} to promote realism. The progress level, $k$, then plays as a hyper-parameter to inform the regressor (emboddied as a ConvNet) about the input type and correspondingly adjust its weights for the desired output. 
A subsequent development argued for alleviating the heavy burden of high-dimensional feature regression \cite{qin2017binary}. The authors suggested transforming features into a low dimension binary code, as seen in Hashing encoding theory \cite{calonder2010brief}, and then operating the feature reconstruction on the binary encoded counterpart.

Other work approached the same problem by encouraging classifiers to assign correct class labels as early as possible \cite{sadegh2017encouraging}. They noticed that early work also made efforts on regularizing the classifiers \cite{kong2014discriminative}; however, none had explicitly enforced the early recognition of actions. In their framework, a sequence of video frames $(y_0, ..., y_{T-1}, y_{T})$ (denoted as $Fr_{t}$ in Figure \ref{fig:encourage_lstm}) is processed by a ConvNet extractor, LSTM sequential aggregation and MLPs as the final classifier, which would regress a sequence of class probability for certain class index $c$ as: $(\hat{x}_{0}(c), \hat{x}_{1}(c), \ldots, \hat{x}_{T}(c))$ (denoted as $y^{t}(k)$ in Figure \ref{fig:encourage_lstm}).
\begin{figure}[htb]
\centering
\begin{minipage}{.55\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{Figures/encourage_lstm.png}
\end{minipage}
\caption[Algorithmic diagram of Encourging-LSTM.]{Algorithmic diagram of \cite{sadegh2017encouraging}. Sequential frames are processed by deep neural networks step by step and a time-variant cross-entropy loss function encourages early recognition. Figure reproduced with permission from \cite{sadegh2017encouraging}.}
\label{fig:encourage_lstm}
\end{figure}

They designed a novel cross-entropy loss to scale the false-positive loss value based on the incoming time index according to
\begin{equation}
\begin{aligned}
  \mathcal{L}(x, \hat{x}) &= -\frac{1}{C} \sum^{C}_{c=1}\sum^{T}_{t=1} [x^{t}(c)log(\hat{x}^{t}(c) + \\
  &\frac{t(1-x^{t}(c))}{T}log(1-\hat{x}^{t}(c))],
\end{aligned}
\label{eq:time_ce_loss}
\end{equation}
where $C$ denotes the total number of action classes.

Recalling that the false negative term (\eg first term in Equation \ref{eq:time_ce_loss}) aims for correctly assigning labels, whereas the false positive term (second term) for suppressing wrong labels, the authors made the relative weights for the former higher than the latter at the beginning of the sequence. That means high probability score for incorrect class labels is allowed as long as the score for correct ones is high enough. The key intuition behind this choice is tolerance for ambiguity at early stages. Therefore, the overall loss encourages the correct recognition in early time stamps.

Parallel research also exploited the property of loss functions for early action recognition \cite{hu2018early}. Instead of generating hard labels (\eg SVMs only output one fixed label and discard other possibilities), they proposed to produce soft labels in a regression fashion, rather than classification. As a concrete example, they map input videos $y_{1:t}$ using transformation matrix $W$ to a vector $x$ that contains scores for all possible classes $C$ as:
\begin{equation}
    x = s(t) W g(y_{1:t}, \theta), x \in \mathcal{R}^{C},
\label{eq:soft_label_regression}
\end{equation}
where $g(y_{t}, \theta)$ is the feature extraction function, output $x$ has dimension $C$ and $s(t)$ is a scaling factor that monotonically increases along the time index. 
The authors adopted a real value time index, $t$, rather than the evenly allocated progress level, $k$, to enable online inference.
Arguably, extensively adopted softmax classifiers have enabled probability scores for all classes and other related work has revealed its effectiveness \cite{sadegh2017encouraging}. However, no direct comparison of the performance between soft-regression and softmax classification was provided.
\begin{figure}[htb]
    \centering
    \resizebox{.45\linewidth}{!}{\includegraphics{Figures/teacher_student.png}}
    \caption[Illustration of the teacher-student learning approach.]{Illustration of the teacher-student learning approach. The student branch takes partial action clips as input (\eg top row), while the teacher branch (bottom row) takes the full clip. Knowledge distillation implemented through feature distance minimization encourages the student branch to learn from the teacher. Figure reproduced with permission from \cite{wang2019progressive}.}
    \label{fig:teacher_student}
\end{figure} 

Very recently, knowledge distillation \cite{hinton2015distilling} has been applied to squeeze fully-observed information into partial observations \cite{wang2019progressive}.
Two neural networks were employed: One acts as a teacher that gets access to full observations; the second acts as a student with only partial access. The student's representation is driven toward that of the teacher  by minimizing the Mean Square Error (MSE) between the latent features and the Maximum Mean Discrepancy (MMD) between the predicted classification probabilities; see Figure \ref{fig:teacher_student}. Some follow on efforts emphasized both the feature reconstruction consistency and semantic knowledge consistency via integrating multiple loss functions (\eg feature distance loss, adversarial loss and classification loss) for a joint optimization \cite{xu2019prediction, wang2019early}. Indeed, it seems that the distance metric plays a critical role in building the connection between video parts. Further, one recent work has found significant improvements via adopting the \textbf{Jaccard} similarity metric to learn the transition between partial and full observations \cite{fernando2021anticipating}.

\section{Propagation Based}
Another way to exploit future information is by propagating the partial observation into the future. Typically, this type of approach extrapolates the visual representations into the future and then applies an existing classifer. 
The key difference between propagation and mutual information is whether or not the system performs \textbf{temporal extrapolations}. Mutual information methods from the previous section emphasize how to enrich partial observations with future information, whereas propagation based methods in this section focus on how to generate an accurate future based on current observations. Mathematically, propagation based approaches start from any incomplete input $y_{1:t}$, assuming $t < T$, and produce the subsequent information $(y_{t+1}, y_{t+2}, ..., y_{T})$; thus, they can be considered as temporal extrapolation. In contrast, during either the testing or training phase, mutual information based approaches do not extrapolate.
Classification is then based on the the concatenation of the observed and extrapolated.

An early exemplar of the propagation approach operated by working with relatively high-level visual representations so that they can be readily processed by extant recognition tools \cite{vondrick2016anticipating}.
\begin{figure}[htb]
    \centering
    \resizebox{.6\linewidth}{!}{\includegraphics{Figures/anticipate_visual_future.PNG}}
    \caption[Deep regression network from with mixtures of output layers for action prediction]{Deep regression network from \cite{vondrick2016anticipating} with mixtures of output layers. Blue boxes are convolutional and fully connected layers for unified processing on each frame, while green boxes represent the mixture of output layers. To push the predicted visual representation close to the real future, MSE loss (\ie yellow box) is calculated with the groundtruth extracted from future frames in a self-supervised way. Figure reproduced with permission from \cite{vondrick2016anticipating}.}
    \label{fig:anticipation}
\end{figure}
In practice, they formulated a deep regression network, consisting of multiple convolutional and fully connected layers, to temporally regress the future high-level deep feature (\ie fc7 activation output from AlexNet \cite{krizhevsky2012imagenet}). To generate the label for future representations without supervision, they collected a small group of labeled video representations, calculated the similarity score and chose the best one. In order to model multi-modality, they extended the original single output structure to $K$ mixtures (\eg denoted as green boxes in Figure \ref{fig:anticipation}). 

This approach has two positive attributes. First, to the extent that the deep features capture semantically meaningful representations, they should be well suited to support recognition. Second, the mixture output helps to model the possibly multimodality of future outcomes. A notable downside is the potentially prohibitive dimensionality of the representation. Nevertheless, it unveiled a novel approach and inspired several follow-on efforts. A subsequent work used Recurrent Neural Networks (RNNs) with learnable Radial Basis Function (RBF) kernels to improve the nonlinearity of predictions \cite{shi2018action}. 
Yet other work upgraded the deep regression component with a Markov Decision Process (MDP) as well as an RNNs \cite{zeng2017visual}, but shared the same intuition.
%Yet other work upgraded the deep regression component with a Markov Decision Process (MDP) implemented as recurrent neural networks to improve the performance \cite{zeng2017visual}. 

While the initial studies on propagation-based early action recognition achieved promising results, critical questions were left unanswered: What type of feature works best for propagation? How can video redundancy be dealt with? How can remote predictions avoid degeneracy? Further, design decisions appeared to be made heuristically without support from ablation studies. These concerns were addressed in an approach that made use of classic recursive filtering coupled with more careful design \cite{zhao2019spatiotemporal}; see Figure \ref{fig:iccv19_he}.
\begin{figure}[ht]
    \centering
    \begin{minipage}{.48\textwidth}
    \includegraphics[width=1.\textwidth]{Figures/iccv19_he_2.png}
    \end{minipage}
    \begin{minipage}{.48\textwidth}
    \includegraphics[width=1.\textwidth]{Figures/iccv19_he_1.png}
    \end{minipage}
\caption[Deep Kalman filtering.]{ The left sub-figure depicts the overall workflow from \cite{zhao2019spatiotemporal} that revisited Kalman filtering under deep network structure: Partial observations (\ie blue boxes) and their pair-wise residuals (\ie green boxes) are used to propagate information into the future. Kalman filtering update is performed at each time step to combat error accumulation; The right sub-figure shows an ablation study that examines different feature stages through visualization. The intermediate feature stage (\eg $3^{rd}$ column from left) performs the best since it keeps critical information of actors while suppresses noisy background present
in the shallow layer. In comparison the vectorized features deeper in the network are too coarse and suppress important details. Numerical studies backed-up the visualizations. Figure reproduced with permission from \cite{zhao2019spatiotemporal}.}
\label{fig:iccv19_he}
\end{figure}

They proposed to propagate the frame-wise feature residuals to lessen the temporal redundancy and thereby forced the model to focus on the underlying dynamics, rather than static background. Moreover, to combat error accumulation, Kalman filtering is incorporated into a deep network, which iterated the \textbf{prediction} and \textbf{update} steps to stablize long-term predictions. Further, they provided an answer to the above question regarding proper features by examining various feature layers in a deep network in propagation and determined that the intermediate layer features, rather than vectorized last layer feature typically used in earlier work, is more suitable for propagation. Presumably, this intermediate level of representation provides the right level of abstraction from the raw video without loosing too much detail.

Other work combined the idea of feature propagation with a reinforcement reward function to encourage early recognition \cite{gao2017red}; Yet other work propagated both the RGB and motion (\ie optical flow) features from deep networks and adopted adversarial learning to boost the realism of their outputs \cite{gammulle2019predicting}. 
In contrast to most recent work that heavily used deep features, an effort has employed hand-crafted Dynamic Image (DI) \cite{bilen2017action} features for propagation, but still depends on deep recognition models for the label assignment \cite{rezazadegan2017encoding}. Finally, an approach that propagated both graph node features (\eg 2D coordinates) and structures (\eg adjacency matrices) has been proposed to tackle a recently appeared task, namely group-player early action recognition \cite{chen2020group}.

\section{Datasets and Performance}
In this section, we describe datasets, evaluation metrics and performance for the majority of early action recognition approaches discussed in this section. As all datasets are used for both action recognition and early recognition, comprehensive comparisons of them can be found elsewhere \cite{kong2018human, kang2016review}.

\textbf{Evaluation} on early action recognition is based on the same recognition accuracy metric as in action recognition, but with a focus on the \textbf{observation ratio} $K$ ranging from $10\%$ to $100\%$, as discussed in the beginning of this chapter. Since each video only owns a single label, the video level mean average precision is reported against each $K$ value. 

\textbf{UCF-101} \cite{soomro2012ucf101} is a dataset collected from a real-life video platform (Youtube) and trimmed for action recognition (each video contains exactly one action). It includes 101 distinct action classes and 13,320 overall video clips with at least 100 videos for each category. UCF-11 and UCF-50 are two earlier versions of the same dataset that contain 11 and 50 action categories respectively. One critical issue of UCF-101 is that videos from YouTube could be very biased by low-level features, meaning low-level features (\ie color and gist) are more discriminative than mid-level features (\ie motion and shape). Researchers have been progressively evaluating both action recognition and early action recognition on UCF-101.

\textbf{HMDB-51} \cite{kuehne2011hmdb} is a large scale human action recognition dataset that comprises 51 daily action categories. It is worth noticing that it contains some fine-grained human facial motions, such as smiling, laughing, chewing etc, in static background windows, which are not seen in other comparable datasets. This dataset also encompasses a wider range of camera motions and viewpoint changes compared to UCF-101. In total, there are a total of 6,766 video clips with at least 102 videos for each class. There are three official data splits and the averaged evaluation score is often reported as final results.

\textbf{JHMDB-21} \cite{jhuang2013towards} is a subset of HMDB-51 with a special focus on 21 human body joint action categories where additional annotations on joints (13 2D-coordinates body joints) are provided. Compared with HMDB-51, categories that mainly contain facial expressions (e.g. smiling), interaction with others (e.g. shaking hands), and very specific actions (e.g. cartwheels) were excluded. Therefore, there are a total of 928 video clips.

\textbf{BIT} \cite{kong2012learning} consists of 8 classes of human interactions (bow, boxing, handshake, high-five, hug, kick, pat, and push), with 50 videos per class. Videos are captured in realistic scenes with cluttered backgrounds, partially occluded body parts, moving objects, and variations in subject appearance, scale, illumination condition and viewpoint. Even though BIT has a relatively limited number of classes and videos, it is a complex dataset in that: \textbf{1.} The backgrounds as well as actor appearances are highly non-discriminative. Various categories often share the same background and actors; \textbf{2.} The starting and ending phases of the videos are highly similar (\ie actors standing still and facing each other). Thus, researchers often have to resort to motion based features for comparable performance.

\textbf{UT-Interaction} (UTI) \cite{ryoo2015ut} is comprised of 2 sets with different environments. Each set consists of 6 types of human interactions: \textit{handshake, hug, kick, point, punch and push}. Each type of interaction contains 10 videos, to provide 60 videos in total. Videos are captured at different scales and illumination conditions. Moreover, some irrelevant pedestrians are present in the videos.


\textbf{TV Human Interaction} \cite{patron2010high} consists of 300 video clips collected from over 20 different TV shows. It contains five action classes: \textit{handshake, high five, hug, kiss and none}. The class “none” represents all other more general actions such as walking and standing. Annotations are provided for every frame of the videos, including the upper body bounding boxes, discrete head orientations and action labels for each person. 

\textbf{Something2something} \cite{goyal2017something} is a dataset that shows human interaction with everyday objects. In the dataset, humans perform a pre-defined action with a daily object. It contains 108, 499 video clips across 174 classes. The dataset enables the learning of visual representations for physical properties of the objects and the world. Compared with others, the dataset shows primarily human related motions (mostly only hand motions are visible). 

\textbf{SYSU-3DHOI} \cite{hu2015jointly} (3D Human-Object Interaction) includes 480 RGBD sequences from 12 action categories, including “playing phone”, “calling phone”, “pouring”, “drinking”, etc. For building this set, 40 participants were asked to perform 12 different activities freely. For each activity, each participant manipulates one of the six different objects: phone, chair, bag, wallet, mop and besom. Therefore, there are in total 480 video clips collected in this set. The contained activity samples have different durations, ranging from 1.9s to 21s. For each video clip, the corresponding RGB frames, depth sequence and skeleton data were captured by a Kinect camera \cite{zhang2012microsoft}.

\textbf{NTU-RGBD} \cite{shahroudy2016ntu} is by far the largest public set for 3D action recognition and prediction. It contains more than 56,000 video samples with about 4 million frames from 60 action categories. All of these action samples were recorded by a Kinect camera \cite{zhang2012microsoft} from three different views. For collecting this set, 40 subjects were asked to perform certain actions several times. This set is very challenging for early action prediction mainly due to its larger scales of quantity, greater diversity in action categories and more complexity in human-human interaction and human-object interaction.

\textbf{ORGBD} \cite{yu2014discriminative} (Online RGB-D) was collected for online action recognition and early action prediction. There are seven types of actions that people often do in the living room: drinking, eating, using laptop, picking up phone, reading phone (sending SMS), reading book, and using remote. All these actions are human-object interactions. The bounding box of the object in each frame is manually labelled.

\textbf{Sports-1M} \cite{karpathy2014large} contains 1, 133, 158 video URLs, which have been annotated automatically with 487 labels. It is one of the largest video datasets. Very diverse sports videos are included in this dataset, such as shaolin kung fu, wing chun, etc. The dataset is extremely challenging due to very large appearance and pose variations, significant camera motion, noisy background motion, etc. However, since the videos originate from Youtube and authors have not maintained the complete video set, some URLs become invalid or expired. Moreover, the automated labelling is known to have yielded incorrect groundtruth in some cases.

\textbf{Jester} \cite{materzynska2019jester} is a recent video dataset for hand gesture recognition. It is a large collection of densely-labeled video clips that shows humans performing pre-defined hand gestures in front of a laptop camera or webcam with a frame rate of 30 fps. There are in total 148,092 gesture videos under 27 classes performed by a large number of crowd workers. The dataset is divided into three subsets: training set (118,562 videos), validation set (14,787 videos), and test set (14,743 videos).

\textbf{OAD} \cite{li2016online} was captured with a Kinect camera \cite{zhang2012microsoft} in daily-life indoor environments and thus provides RGBD data. It includes 10 actions. The long video sequences in this dataset correspond to about 700 action instances. The starting and ending frames of each action are annotated in this dataset. 30 long sequences are used for training, and 20 long sequences are for testing.

\textbf{PKU-MMD} \cite{liu2017pku} is a large dataset for 3D activity analysis in continuous sequences. The data set contains 1076 long video sequences in 51 action categories, performed
by 66 subjects in three camera views. It contains almost 20,000 action instances and 5.4 million frames in total. This dataset also provides multi-modality data sources, including RGB, depth, Infrared Radiation and Skeleton.

\textbf{OoPS!} \cite{epstein2020oops} is proposed recently to study unintentional human actions. It includes a variety of daily human activities. Instead of focusing on action classification, the paper pays special attention to whether the performer succeeds/fails at achieving the goal. The dataset contains 20,338 videos and only has three class labels: Intentional, Transition and Unintentional. This paper conducted the action-intention prediction task on this dataset: early predicting the failure before it happens (1.5 seconds into future).


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\pagebreak
\begin{landscape}
\vspace*{\fill}
\centering
\begin{longtable}[htbp]{@{}@{} l r r r r r r}
% pairs: absolute number (percentage)
\toprule%
 \centering
 & \multicolumn{1}{c}{{{\bfseries Year}}}
 & \multicolumn{1}{c}{{{\bfseries No. Videos}}}
 & \multicolumn{1}{c}{{{\bfseries No. Actions}}}
 & \multicolumn{1}{c}{{{\bfseries Avg. Len}}}
 & \multicolumn{1}{c}{{{\bfseries Domain}}}
 & \multicolumn{1}{c}{{{\bfseries Data-Modality}}} \\

\cmidrule[0.4pt](l{0.25em}){1-1}%
\cmidrule[0.4pt](r{0.25em}){2-2}%
\cmidrule[0.4pt](r{0.25em}){3-3}%
\cmidrule[0.4pt](r{0.25em}){4-4}%
\cmidrule[0.4pt](r{0.25em}){5-5}%
\cmidrule[0.4pt](r{0.25em}){6-6}%
\cmidrule[0.4pt](r{0.25em}){7-7}%
% \midrule
\endhead

\textbf{OoPS!}  \cite{epstein2020oops} & 2020 &
20,338 & 3 & \highest{9.4s} & \highest{Action-intention} & RGB, Pose, Flow, Naaration \\ 

\myrowcolour
\textbf{Jester}  \cite{materzynska2019jester} & 2019 &
146,092 & 27 & \highest{3s} & \highest{Gesture} & RGB \\ 

\textbf{Something2something} \cite{goyal2017something} & 2017 & 
108,499 & 174 &  \highest{4.03} & \highest{Activity} & RGB \\

\myrowcolour
\textbf{PKU-MMD} \cite{liu2017pku} & 2017 &
1076 & 51 & \highest{-} & \highest{Activity, HOI} & RGB+D, IR, Skeleton\\ 

\textbf{OAD}  \cite{li2016online} & 2016 & 
59 & 10 & \highest{219} & \highest{Activity} & RGB+D, Skeleton\\

\myrowcolour
\textbf{NTU-RGBD} \cite{shahroudy2016ntu} & 2016 &
56,000 & 60 & \highest{-} & \highest{Activity, Interaction} & RGB+D, IR, 3D-Skeleton\\

\textbf{SYSU-3DHOI}  \cite{hu2015jointly} & 2015 &
480 & 12 & \highest{-} & \highest{Activity, HOI} & RGB+D \\

\myrowcolour
\textbf{UT-Interaction} \cite{ryoo2015ut} & 2015 & 
60 & 6 & \highest{3s} & \highest{Human Interaction} & RGB \\

\textbf{Sports-1M} \cite{karpathy2014large} & 2014 &
1,133,158 & 487 & \highest{-} & \highest{Action} & RGB \\

\myrowcolour
\textbf{ORGBD} \cite{yu2014discriminative} & 2014 & 
- & 7 & \highest{12} & \highest{Action, HOI} & RGB+D, Skeleton, BBx\\

\textbf{JHMDB-21}  \cite{jhuang2013towards} & 2013 & 
928 & 21 & \highest{-} & \highest{Action} & RGB, Flow, Skeleton, Contour \\

\myrowcolour
\textbf{UCF-101} \cite{soomro2012ucf101} & 2012 & 13,320 &
101 & \highest{6.39s} & \highest{Action} & RGB \\

\textbf{BIT} \cite{kong2012learning} & 2012 &
50 & 8 & \highest{-} & \highest{Human Interaction} & RGB \\

\myrowcolour
\textbf{HMDB-51} \cite{kuehne2011hmdb} & 2011 & 
6.766 & 51 & \highest{-} & \highest{Action} & RGB \\

\textbf{TV Human-Interaction} \cite{patron2010high} & 2010 &
300 & 20 & \highest{-} & \highest{Human Interaction} & RGB \\
\bottomrule
\caption[Summary of datasets for early action recognition.]{Summary of datasets for early action recognition.} \\
\end{longtable}
\vspace*{\fill}
\end{landscape}

{\bf Performance} evaluation of early action recognition has been focused on consideration of four of the above datasets: UCF-101, J-HMDB, UT-Interaction and BIT. We restrict performance comparisons to that set. For J-HMDB as shown in Table \ref{tab:jhmdb_rst}, we follow the standard procedure to report the recognition accuracy based on the first 20$\%$ frames of videos. Some work also reports results regarding the whole set of observation ratios and we refer readers to \cite{singh2017online, xu2019prediction} for more details. As noticed, recent advances 
based on motion extrapolation and Kalman filtering \cite{zhao2019spatiotemporal} as well as an RNN with RBF kernels \cite{shi2018action} have pushed the early recognition accuracy using only 20$\%$ frames to around $75\%$. Thus, there is still room for further improvements. Very recently, an effort achieved significant improvements (\ie $83\%$) via feature mapping learned through the Jaccard distance \cite{fernando2021anticipating}. 
On the other hand, for the UT-Interaction dataset, recent approaches can achieve over $90 \%$ accuracy with only the first $20\%$ frames and can obtain almost perfect accuracy over the first $50\%$; see Table \ref{tab:uti_rst}. For this dataset, a wide variety of approaches perform very well. These observations somewhat indicate that UT-Interaction is saturated. Similarly, the  UCF-101 dataset has been demonstrated to be easily recognizable using less than $30\%$ frames, as shown in Table \ref{tab:ucf_rst}. Again, a wide variety of aproaches are able to do well on this dataset. In contrast, the BIT dataset, for most approaches, still provides difficulties for early recognition, probably due to its limited size. Although, the most recent approaches can do very well having viewed $50\%$ or more of the data.
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption[Summary of J-HMDB Performance]{Summary of J-HMDB Performance}\label{tab:jhmdb_rst}%
    \begin{tabular}{l|r}
    \toprule
    Methods & Accuracy @ 20\% \\
    \midrule
    \midrule
    Within-class Loss \cite{ma2016learning} & 33\% \\
    DP-SVM \cite{soomro2018online} & 5\% \\
    S-SVM \cite{soomro2018online} & 5\% \\
    Where/What \cite{soomro2016predicting} & 10\% \\
    Context-fusion \cite{jain2016recurrent} & 28\% \\
    ELSTM \cite{sadegh2017encouraging} & 55\% \\
    G. Singh's \cite{singh2017online} & 59\% \\
    TPnet \cite{singh2018predicting} & 60\% \\
    DR2N \cite{sun2019relational} & 66\% \\
    Pred-GAN \cite{xu2019prediction}& 67\% \\
    RBF-RNN \cite{shi2018action} & 73\% \\
    RGN-KF \cite{zhao2019spatiotemporal} & 78\% \\
    JVS+JCC+JFIP \cite{fernando2021anticipating} & 83.5\% \\
    \bottomrule
    \bottomrule
    \end{tabular}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption[Summary of UTI Performance.]{Summary of UTI Performance. Notice that some work reports results for set $1$ and set $2$ of the UTI dataset separately \eg \cite{chen2018part} , while others report the averaged results.}\label{tab:uti_rst}
    \begin{tabular}{l|r|r}
    \toprule
    Methods & Accuracy @ 20\% & Accuracy @ 50\% \\
    \midrule
    \midrule
    S-SVM \cite{soomro2018online} & 11.00 & 13.40 \\
    DP-SVM \cite{soomro2018online} & 13.00 & 14.60 \\
    CuboidBayes \cite{ryoo2011human} & 25.00 & 71.00 \\
    CuboidSVM \cite{ryoo2010overview} & 31.70 & 85.00 \\
    Context-fusion \cite{jain2016recurrent} & 45.00 & 65.00 \\
    Within-class Loss \cite{ma2016learning} & 48.00 & 60.00 \\
    IBoW \cite{ryoo2011human} & 65.00 & 81.70 \\
    DBoW \cite{ryoo2011human} & 70.00 & 85.00 \\
    BP-SVM \cite{laviers2009improving} & 65.00 & 83.30 \\
    ELSTM \cite{sadegh2017encouraging} & 84.00 & 90.00 \\
    Poselet \cite{raptis2013poselet} & - & 73.33 \\
    PA-DRL (set 1) \cite{chen2018part} & 69.00 & 91.70 \\
    PA-DRL (set 2) \cite{chen2018part} & 58.00 & 83.30 \\
    Future-dynamic Image & 89.20 & 91.90 \\
    Early-GAN \cite{wang2019early} & 38.00 & 78.00 \\
    Pred-GAN (set 1) \cite{xu2019prediction} &    -   & 100.00 \\
    Pred-GAN (set 2) \cite{xu2019prediction} &    -   & 85.70 \\
    RBF-RNN \cite{shi2018action} &   -    & 97.00 \\
    Joint-GAN \cite{gammulle2019predicting} & 98.30 & 99.20 \\
    SPR-Net \cite{hou2020confidence} & - & 85.30 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
\end{table}%

\pagebreak
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{landscape}
\vspace*{\fill}
  %\centering
 %\begin{table}
\begin{table}[!ht]
    \caption[Summary of UCF-101 Performance.]{Summary of UCF-101 Performance. Notice that some work only reports accuracy at a few ratios (\ie 50\% and 100\%). The symbol $\approx$ means approximated number from the original plotted graph, rather than actual number, due to the unavailability of some results.}\label{tab:ucf_rst}%
    \setlength{\tabcolsep}{0.5em} % for the horizontal padding
    {\renewcommand{\arraystretch}{1.3}% for the vertical padding
    \begin{tabular*}{\linewidth}{|cc| @{\extracolsep{\fill}} c|c|c|c|c|c|c|c|c|c|}
    \toprule & \multicolumn{1}{r|}{Metrics} & \multicolumn{10}{c|}{Obervation Ratio} \\
    \cmidrule{3-12}    \multicolumn{1}{|l}{Methods} &       & 10\%  & 20\%  & 30\%  & 40\%  & 50\%  & 60\%  & 70\%  & 80\%  & 90\%  & 100\% \\
    \midrule
    \multicolumn{2}{|c|}{IBoW \cite{ryoo2011human}} & 36.29 & 65.69 & 71.69 & 74.25 & 74.39 & 75.23 & 75.36 & 75.57 & 75.79 & 75.79 \\
    \multicolumn{2}{|c|}{DBoW \cite{ryoo2011human}} & 36.29 & 51.57 & 52.71 & 53.13 & 53.16 & 53.24 & 53.24 & 53.24 & 53.45 & 53.53 \\
    \multicolumn{2}{|c|}{MTSSVM \cite{kong2014discriminative}} & 40.05 & 72.83 & 80.02 & 82.18 & 82.39 & 83.21 & 83.37 & 83.51 & 83.69 & 82.82 \\
    \multicolumn{2}{|c|}{MSSC \cite{cao2013recognize}} & 34.05 & 53.31 & 58.55 & 57.94 & 61.79 & 60.86 & 63.17 & 63.64 & 61.63 & 61.63 \\
    \multicolumn{2}{|c|}{DeepSCN \cite{kong2017deep}} & 45.02 & 77.64 & 82.95 & 85.36 & 85.75 & 86.70 & 87.10 & 87.42 & 87.50 & 87.63 \\
    \multicolumn{2}{|c|}{Mem-LSTM \cite{kong2018action}} & 51.02 & 80.97 & 85.73 & 87.76 & 88.37 & 88.58 & 89.09 & 89.38 & 89.67 & 90.49 \\
    \multicolumn{2}{|c|}{MSRNN \cite{lan2014hierarchical}} & 68.00 & 87.39 & 88.16 & 88.79 & 89.24 & 89.67 & 89.85 & 90.28 & 90.43 & 90.70 \\
    \multicolumn{2}{|c|}{PA-DRL \cite{chen2018part}} & -     & -     & -     & -     & 87.30 & -     & -     & -     & -     & 87.70 \\
    \multicolumn{2}{|c|}{AAPNet \cite{kong2018adversarial}} & 59.85 & 80.85 & 86.78 & 86.47 & 86.94 & 88.34 & 88.34 & 89.85 & 90.85 & 91.99 \\
    \multicolumn{2}{|c|}{Student-Teacher \cite{wang2019progressive}} & 83.32 & 87.13 & 88.92 & 90.85 & 91.04 & 91.28 & 91.28 & 91.23 & 91.31 & 91.47 \\
    \multicolumn{2}{|c|}{Joint-GAN \cite{gammulle2019predicting}} & -     & 84.20     & -     & -     & 85.60 & -     & -     & -     & -     & - \\
    \multicolumn{2}{|c|}{RGN-KF \cite{zhao2019spatiotemporal}} & 83.12 & 85.16 & 88.44 & 90.78 & 91.42 & 92.03 & 92.00 & 93.19 & 93.13 & 93.13 \\
    \multicolumn{2}{|c|}{Pred-CGAN \cite{xu2019prediction}} & -     & -     & -     & -     & 91.14 & -     & -     & -     & -     & 93.76 \\
    \multicolumn{2}{|c|}{Eearly-CGAN $\approx$ \cite{wang2019early}} & 78.00 & 84.50 & 86.00 & 88.00 & 89.40 & 89.95 & 90.01 & 90.53 & 90.76 & 91.05 \\
    \multicolumn{2}{|c|}{SPR-Net \cite{hou2020confidence}} & 88.70 & - & - & - & 91.60 & - & - & - & - & 91.40 \\
    \multicolumn{2}{|c|}{STGCN \cite{fernando2021anticipating}} &80.26 &-& 89.86 &-& 92.87 &-& 94.08 &-& 94.43 &- \\
    \multicolumn{2}{|c|}{JVS+JCC+JFIP \cite{fernando2021anticipating}} & - & 91.70 & - & - & - & - & - & - & - & - \\
    \bottomrule
    \end{tabular*}%
}
\end{table}%
\vspace*{\fill}
\end{landscape}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{landscape}
\vspace*{\fill}
\begin{table}[!ht]
    \caption{Summary of BIT-101 Performance}
    \setlength{\tabcolsep}{0.5em} % for the horizontal padding
    {\renewcommand{\arraystretch}{1.3}% for the vertical padding
    \noindent\begin{tabular*}{\linewidth}{|cc| @{\extracolsep{\fill}} c|c|c|c|c|c|c|c|c|c|}
        \toprule
          & \multicolumn{1}{r|}{Metrics} & \multicolumn{10}{c|}{Obervation Ratio} \\
\cmidrule{3-12}    \multicolumn{1}{|l}{Methods} &       & 10\%  & 20\%  & 30\%  & 40\%  & 50\%  & 60\%  & 70\%  & 80\%  & 90\%  & 100\% \\
    \midrule
    \multicolumn{2}{|c|}{IBoW \cite{ryoo2011human}} & 22.66 & 24.22 & 37.50 & 48.44 & 48.44 & 52.34 & 46.09 & 49.22 & 42.97 & 43.75 \\
    \multicolumn{2}{|c|}{DBoW \cite{ryoo2011human}} & 22.66 & 25.78 & 40.63 & 43.75 & 46.88 & 54.69 & 55.47 & 54.69 & 55.47 & 53.13 \\
    \multicolumn{2}{|c|}{MTSSVM \cite{kong2014discriminative}} & 28.12 & 32.81 & 45.31 & 55.47 & 60.00 & 61.72 & 67.19 & 70.31 & 71.09 & 76.56 \\
    \multicolumn{2}{|c|}{MSSC \cite{cao2013recognize}} & 21.09 & 25.00 & 41.41 & 43.75 & 48.44 & 57.03 & 60.16 & 62.50 & 66.40 & 67.97 \\
    \multicolumn{2}{|c|}{DeepSCN \cite{kong2017deep}} & 37.50 & 44.53 & 59.38 & 71.88 & 78.13 & 85.16 & 86.72 & 87.50 & 88.28 & 90.63 \\
    \multicolumn{2}{|c|}{MSDA \cite{chen2012marginalized}} & -     & -     & -     & -     & 70.00 & -     & -     & -     & -     & 81.50 \\
    \multicolumn{2}{|c|}{GLTSD \cite{lai2017global}} & 26.60     & -     & -     & -     & 79.40 & -     & -     & -     & -     & - \\
    \multicolumn{2}{|c|}{PA-DRL \cite{chen2018part}} & -     & -     & -     & -     & 85.90 & -     & -     & -     & -     & 91.40 \\
    \multicolumn{2}{|c|}{AAPNet \cite{kong2018adversarial}} & 38.84 & 45.31 & 64.84 & 73.40 & 80.47 & 88.28 & 88.28 & 89.06 & 89.84 & 91.40 \\
    \multicolumn{2}{|c|}{RGN-KF \cite{zhao2019spatiotemporal}} & 35.16 & 46.09 & 67.97 & 75.78 & 82.03 & 88.28 & 92.19 & 92.28 & 92.16 & 92.16 \\
    \multicolumn{2}{|c|}{Pred-CGAN \cite{xu2019prediction}} & -     & -     & -     & -     & 87.31 & -     & -     & -     & -     & 91.79 \\
    \multicolumn{2}{|c|}{Eearly-CGAN $\approx$ \cite{wang2019early}} & 38.80 & 58.00 & 79.00 & 90.00 & 96.00 & 96.00 & 96.00 & 96.00 & 96.00 & 96.00 \\
    \multicolumn{2}{|c|}{SPR-Net \cite{hou2020confidence}} & 84.10 & - & - & - & 100.00 & - & - & - & - & 99.20 \\
    \multicolumn{2}{|c|}{STGCN \cite{fernando2021anticipating}} & 46.09 & - & 58.59 & - & 81.25 & - & 89.06 & - & 86.72 & - \\
    \bottomrule
    \end{tabular*}%
    }
  \label{tab:bit_result}%
\end{table}%

\vspace*{\fill}
\end{landscape}
\pagebreak



==> BODY/Backup/chapter3.tex <==
\section{Overview}
\begin{figure}[htb]
    \centering
    %\resizebox{.5\linewidth}{!}{\includegraphics{Figures/activity_vs_action.png}}
    \resizebox{.8\linewidth}{!}{\includegraphics{Figures/survey_redrew_1.pdf}}
    \caption[Dissimilarity between future action prediction and early action recognition.]{Illustration of the general dissimilarity between future action prediction and early action recognition. The latter (bottom row) aims to infer a class label for an ongoing action from partial initial observations; the former aims to anticipate (strings of) future actions from initial observations.}
    \label{fig:action_vs_activity}
\end{figure}
Other than recognizing certain \textit{single} actions at its early stage, another emerging topic has caught researchers' attention, that is future action prediction. It differs from the previously discussed problem, early action recognition of Section \ref{Sec:early_actio}, in that its goal is to produce predictions of subsequent future actions. As illustrated in Figure \ref{fig:action_vs_activity}, the input (as solid boxes) and its output (as boundary-dotted boxes) in Early Recognition (bottom row) share the same label, such as \textit{\textbf{making a salad}}, whereas in Action Prediction (top row) input and output are often different yet logically related.

The ability to deduce possible future events from previous and current observations is one of the core functionalities needed by contemporary intelligent systems. In the example of automated traffic systems, \ie artifical integellience guided vehicles, every driver needs to be cautiously aware of surroundings and would benefit from smart prediction systems that can tell the specific next action of in-coming vehicles (\eg turning-right), to better plan its own motion in response (\eg slow-down or keep driving). Early action recognition does not satisfy such a demand, as it simply predicts the completion of an in progress action and thereby lacks sufficient prediction horizon to anticipate future actions. Exploring the plausible future is well studied in other fields, \eg weather forecasting and stock price prediction. In the computer vision community, however, researchers have only recently become heavily active in exploring solutions.

To examine future action prediction in detail, we group existing research into three major divisions: \textbf{1.} activity singleton or sequence prediction; \textbf{2.} joint prediction of activity semantics and times; \textbf{3.} ego-centric oriented action prediction. The first division discusses the most frequent setting for future action prediction: given the raw video frame observations, ${y_{1:t}}$, and/or its action semantics, $x_{1:t}$, produce the semantic label for actions that would happen afterward. The prediction can be either the immediate single following action, \ie $x_{t+1}$, or a sequence of future actions, \ie $x_{t+1: t+n}$.  
Note that the prediction provides only action semantics (\eg labels); time of occurrence and duration are left ambiguous. 
The second division considers not just prediction of sequences of future actions, but also their times. The last division tries to assist action forecastings in ego-centric settings, where observed frames are taken from first-person-view and thus mimic real life carry-on camera settings.

\section{Activity Singleton or Sequence Prediction}\label{Sec:future_action_1}
This section describes the general version of future action prediction, which is mapping the video input, that often contains a sequence of observed actions, into its subsequent sequence of actions, as shown in Figure \ref{fig:action_vs_activity} top row. The length of the predicted sequence can vary from one to many.

Hereby, we formally define the problem according to one of the initial works in future action prediction \cite{chakraborty2014context}. Let a sequence of observed video frames be given as $y^{obs} = (y_{1}, y_{2}, \ldots, y_{t} )$ and its corresponding frame-wise action labels be given as $\hat{x}^{obs} = ( x_{1}, x_{2}, \ldots, x_{t})$. 
Note that the symbol $x^{obs}$ represents the groundtruth video level labels annotated through human labor. However, in most studies, researchers would estimate the action labels with existing methods, rather than directly using the groundtruth video level labels. To clarify this nuance, we denote the estimated action labels as $\hat{x}^{obs}$.
Since actions can take large time spans, the frame-wise action labels can be either repeating or idle (no activity performed). Our task is to produce the future action semantics $x^{unobs} = (x_{t+1}, x_{t+2},...)$ that happen at unobserved time indices, \ie $t+n, n>0$. The set of future time indices of interest, $N=(n, n+1, n+2, \ldots)$, are referred to as the prediction horizon. So in other words, the task is to seek a function $f$ that maps $y^{obs} \rightarrow x^{unobs}$ with specified prediction horizon $n_{i}$. 

Indeed, compared with the standard video action recognition definition $f: y^{obs} \rightarrow x^{obs}$, the above definition seems like a temporal shifted version of the recognition function, \eg shifting $x^{obs}$ to $x^{unobs}$ by a desired time span. However, it is worth noticing that the semantic level information of observed video input, $y^{obs}$, can be inferred beforehand, either with groundtruth annotations or extraction algorithms, and therefore it is possible to operate a high-level semantic mapping $y^{obs} \rightarrow \hat{x}^{obs} \rightarrow x^{unobs}$ as a solution. Actually, most researchers adopted the second approach, especially for long-term predictions that typically cover multiple subsequent actions.

For example, early work along this line \cite{chakraborty2014context} proposed to treat any sequence of actions performed by all actors within a video as connected nodes in a Markov Random Field model (MRF) \cite{geman1986markov}, as shown in Figure \ref{fig:accv2014_mrf}. These nodes are connected with a manually defined edge potential function that reflects a reasonable range of spatiotemporal affinity between any two nodes. Furthermore, a node potential function that denotes how likely a certain observation, $y_{t}$, belongs to certain action label, $x_{t}$, was implemented as SVM classifiers.
\begin{figure}[htb]
    \centering
    \resizebox{.7\linewidth}{!}{\includegraphics{Figures/mrf_activity_prediction.pdf}}
    \caption[MRF based approach for future action inference.]{Workflow diagram of MRF based approach from \cite{chakraborty2014context}. Some nodes are initialized as recognized activity labels from observed video frames (\eg $x_1, x_2, x_3$). Other nodes are initialized with uniform probability for entire action candidate set (\eg $x_4, x_5, x_6$). Loopy belief propagation (LBP) will run $L$ iterations to pass messages between nodes. As noted, the direct mapping from the past to the future is built upon high level action semantic labels $\hat{x}^{obs} \rightarrow x^{unobs}$, instead of raw frame inputs. The labels are extracted from raw frame inputs using a standard action recognition algorithm. Figure modified with permission from \cite{chakraborty2014context}}.
    \label{fig:accv2014_mrf}
\end{figure}
More specifically, the observed action labels, $\hat{x}^{obs}$, come from a pre-trained recognition system that relies on a Bag-of-Word (BoW) approach over Space Time Interest Points (STIP) and Multi-class SVMs. To do the inference of the next action labels $x_{t+n}$, loopy belief propagation (also known as the sum-product algorithm) \cite{murphy2013loopy} is performed to compute the conditional distribution: $p(x^{unobs}| \hat{x}^{obs})$.
The capacity of a Markov model greatly depends on the order of dependency. The adopted MRF model in \cite{chakraborty2014context} specifies the maximum size of the neighboring clique as four nodes (two nodes in the past and two nodes in the future, if any), which leads to faster inference but limited performance. 

Another research effort also adopted this high-level label inference scheme but relies on a more flexible Markov model, namely the Various order Markov dependency Model (VMM) implemented as graph (or tree) structures to model the temporal relation among activity sequences, as shown in Figure \ref{fig:ngram_pst} (a). Work that relies on such structures for future activity parsing include \cite{li2012modeling, pei2011parsing, li2014prediction, hamid2009novel}. These approaches advocate to represent activity sequence information as a sequence of ordered discrete alphabet symbols (grammars) and group them with \textit{n-gram} representations. Again, to obtain action labels from observed inputs, off-the-self action detection as well as recognition algorithms are needed.

As an example, some efforts choose to build a Probabilistic Suffix Tree (PST) for representing complex activity structures \cite{li2014prediction}. The PST structure is learned from training data, with the pretrained tree providing the chained transition probabilty for each suffix. Thus, the inference of future actions can be viewed as finding the most probable suffix leaf node given prefix node inputs, as seen in Figure \ref{fig:ngram_pst} right side.
\begin{figure}[ht]
    \centering
    \begin{minipage}{.32\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/activity_tree.pdf}
    \caption*{(a)}
    \end{minipage}
    \begin{minipage}{.55\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/kang_li.png}
    \caption*{(b)}
    \end{minipage}
\caption[Tree graph action prediction.]{(a) Example of representing an activity sequence as a tree graph from \cite{gupta2009understanding}. The temporal development is structured as tree nodes and leafs in a top-down fashion, where the top stands for the starting and bottom for ending. (b) The prediction of future action ``Grab object close to head" is selected by traversing the PST given prefix input and choosing the most likely suffix. Figure reproduced with permission from \cite{li2014prediction}.}
\label{fig:ngram_pst}
\end{figure}
The obvious drawback of Markov based methods is that the length of prediction is pre-defined in the training set. For example in \cite{li2014prediction}, the height of the PST is decided during training and thus the model can not be easily extended to undefined future lengths. However, the \textit{n-gram} representation of video activity is an over-simplified method, as critical information contained in image space is ignored. To this end, a recent effort researched on video representation learning in Riemannian geometry space, where the learned model can enable hyperbolic space embeddings, which is a continuous version of tree structures as shown in Figure \ref{fig:ngram_pst}. Thus, the predictive model supports building activity hierarchies for both early and future action prediction \cite{suris2021learning}.

Instead of using generative probabilistic models as above, a discriminative instance of Markov Chains, Conditional Random Fields (CRFs) \cite{lafferty2001conditional}, has been suggested to combine with particle filters for anticipating future human-object interactions \cite{koppula2015anticipating}. This combination enables a straightforward temporal extrapolation, as the particle filters are a type of recursive Bayesian filter that can propagate into unlimited time and space. In particular, they jointly modeled the future activity semantics with object affordances as well as movement trajectories. Notably, a recent work has advanced generative adversarial grammar learning for activity forecasting \cite{piergiovanni2020adversarial}.

The aforementioned approaches build models on a high-level semantic space, rather than raw video input or even visual features. The underlying assumption is that activity labels are linked by certain standard rules, \eg actions for making certain salads are dictated by their instructions. Therefore, straightforward modelling on sequences of action labels is sufficient. Yet in real life, scenarios exist where future actions are less well predicted by well defined scripts. For example, pedestrians walking can happen in a wide range of places and times. It can lead to ``road crossing", ``turning", ``stop and watch", etc. So, reasoning the future from an extremely common action is hard. Furthermore, in surveillance camera settings, actors can enter the field of view at times that obscure their previous actions, in which cases observing one's full activity sequence is impossible. To solve such problems, many researchers resort to a direct mapping from $y^{obs}$ to future actions $x^{unobs}$.
\begin{figure}[htb]
    \centering
    \resizebox{1.\linewidth}{!}{\includegraphics{Figures/aio_hmm.PNG}}
    \caption[Multi-sensors next action anticipation.]{The setting of \cite{jain2015car} combing multiple cues. Multiple cues collected from both inside and outside sensors are used to anticipate the next maneuver of drivers. Figure reproduced with permission from \cite{jain2015car}.}
    \label{fig:aio_hmm}
\end{figure}

One early effort that followed this scheme proposed to rely on cues distilled from multiple visual sources to predict the next driver maneuver \cite{jain2015car}. Specifically, it collected information from four information sources: 1. facial motion trajectories and head angles detected from the driver-facing camera and feature tracking techniques; 2. speed logger from the vehicle system; 3. outside context from the road-facing camera; 4. the GPS map. They fused these four types of features with a novel HMM model where the maneuvers of drivers play as the hidden variables, outside sensory as control units and inside sensory as observations. However, since HMMs can not handle very high dimensional data, they converted most sensory cues into binary features, \eg if vehicle speed is larger than 15km/hr, set the feature flag as 1 otherwise 0.

To encourage more expressive features, \eg 3D human head/facial models, the authors made an upgrade on the sequential modelling module \cite{jain2016recurrent}. They replaced the HMMs with a recurrent neural network (an LSTM) and modulated four sensory channels with two individual RNNs. The final fusion was done by MLPs, followed by softmax classifiers. A critical difference between this work and earlier related approaches based on high-level intermediate inferences, e.g., \cite{li2014prediction}, is the encompassed time span. Observations in the high-level based usually cover multiple actions that can takes \textbf{minutes}. In contrast, \cite{jain2016recurrent} only consumes frames that are 0.8 second (about 20 frames) ahead of the event happening, which has the potential to be deployed in real-time systems.

Similar work that focuses on short-term (or singleton) action prediction directly from past raw video inputs appears frequently in many sub-areas. One such effort proposed to leverage environment-agent interactions to anticipate risk actions as well as localize future risk regions \cite{zeng2017agent}. Another worked on anticipating traffic accidents from vehicle cameras through stacking local detected object features and global context \cite{suzuki2018anticipating}. Some other work built a graph Convolutional Network (GCN) to model interactions between multiple agents and contextual objects to forecast future activities along with future trajectories of pedestrians \cite{liang2019peeking}. Pedestrian road-crossing intention prediction is one concrete example of action prediction in traffic scenarios \cite{rasouli2019pie, rasouli2020pedestrian, rasouli2017they}. Again, in these works, past observations contain little or no evidently useful activity semantics, instead researchers found it helpful to mine cues from subtle details.
%as shown in Figure \ref{fig:raw_input_predict}. 
As an example, an effort on anticipating crossing of pedestrians fused human poses, human visual representation extracted from deep networks, scene contextual information and vehicle speed, with a RNN, to make predictions \cite{rasouli2020pedestrian}.

\iffalse
\begin{figure}[ht]
    \centering
    \begin{minipage}{.4\textwidth}
    \includegraphics[width=1.\textwidth]{Figures/amir_ped_intention.png}
    \end{minipage}
    \begin{minipage}{.4\textwidth}
    \includegraphics[width=1.\textwidth]{Figures/peek.png}
    \end{minipage}
\caption{Examples of digging multiple cues for future predictions. (Left) R. Amir \cite{rasouli2020pedestrian} fuses: pedestrian poses, pedestrian/scene visual feature from CNNs and vehicle velocity for intention prediction. (Right) J. W. Liang \cite{liang2019peeking} models persion-object, person-scene and persion-pose altogether for activity prediction.}
\label{fig:raw_input_predict}
\end{figure}
\fi

\section{Joint Prediction of Activity and Occurrence Time}
Joint prediction of future actions and their times has recently become an active research area, as the occurrence time is an important attribute of activities, e.g., \textit{cutting meat} often takes longer than \textit{open lid}.
%for its importance in critical applications like automated navigation, human-computer interaction as well as for the intellectual challenges it presents. 
All video-based action prediction work forecasts upcoming activities, here, the distinction is that both the activities and their times are predicted. An example is provided in Figure \ref{fig:act_time}.
\begin{figure}[htb]
    \centering
    \resizebox{.8\linewidth}{!}{\includegraphics{Figures/alg_redrew_3.pdf}}
    \caption[Predicting future activity labels and time durations.]{Predicting future activity labels and time durations. The left hand side shows initial observed activities, indicated as labelled boxes, with their temporal duration encoded by box length. The right hand side shows possible predictions.}
    \label{fig:act_time}
\end{figure}

An initial effort in this direction \cite{mahmud2016poisson} adopted the Poisson process \cite{kingman2005p} as a key technique for activity inter-arrival time modelling. Notice that inter-arrival time differs from the absolute activity occurrence time in that it stands for the duration between the starting and ending of a certain action. The probability density function for the possible next action interval, $\tau$, under the assumed Poisson distribution is
\begin{equation}
    p(T = \tau) = \frac{\lambda^{\tau}}{\tau\,!} e^{\lambda} 
\label{eq:possion}
\end{equation}
\iffalse
and
\begin{equation}
    p(T > \tau) = e^{-\lambda \tau},
\end{equation}
\fi
where $\lambda$ is the intensity function that controls the shape of the Poisson probability density function and its physical meaning is the average number of events among the whole time span. The Poisson distribution and sampling are plotted at Figure \ref{fig:poisson_intuition} (a) and (b) respectively.

There are three properties of the Poisson distribution that are worth noticing: \textbf{1.} Its samples are always positive integers. Equation \ref{eq:possion} incurs a \textbf{factorial} function on time $\tau$, thus its result must be an integer; additionally, by default researchers assume there is no negative time value, so that $\tau > 0$. To summarize, the Poisson distribution is a positive \textbf{discrete} function as shown in Figure \ref{fig:poisson_intuition} (b). \textbf{2.} Its shape is unimodal. \textbf{3.} It is memoryless in that the sampling of the current step is independent from any previous samples.

To support a stochastic modelling of time, the authors pre-defined a Gaussian Process prior for $\lambda(t)$ and learned its parameters (\ie the mean and variance for certain actions and times) from training data for every action. Then, they performed testing through importance sampling. Unfortunately, they only train and test on a single action input and single action output, without considering recursive temporal predictions.
\begin{figure}
    \centering
    \begin{minipage}{.4\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/poisson_pdf.png}
    \caption*{(a)}
    \end{minipage}
    \begin{minipage}{.4\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/poisson_sample.png}
    \caption*{(b)}
    \end{minipage}
\caption[Poisson distribution.]{(a) Probability density function of Poisson distribution regarding various parameters $\lambda$. (b) Histogram distribution of 1000 sampled inter-arrival times from Poisson process with $\lambda = 5$. Since Poisson is a member of the exponential family, its distribution looks similar to a Gaussian distribution, but its data points are always positive integers.}
\label{fig:poisson_intuition}
\end{figure}

An extension of the initial work \cite{mahmud2016poisson} used the temporal point process for the same task \cite{mehrasa2019variational}, where the intensity parameter $\lambda$ is dynamically calculated from past observations as
\begin{equation}
    p(T = \tau) = \lambda(\tau | x_{1:k}) e^{-\int^{t|x_{1:k}}_{0} \lambda(t) dt},
\label{eq:temporal_possion}
\end{equation}
where $x_{1:k}$ represents past information, such as raw frames, semantic labels or past action times. 
Their model also supports stochastic time and action prediction via sampling the parameter $\lambda$ through a Variational Auto-Encoder (VAE) embodied as LSTMs. This approach is depicted in Figure \ref{fig:vae_app}. Due to the nature of Poisson distribution, this approach can not produce more than one future step (action, time) at each time step. Notably, both efforts \cite{mahmud2016poisson, mehrasa2019variational} resort to a learning fashion for the hyper-parameter $\lambda$.
\begin{figure}[htb]
    \centering
    \resizebox{1.\linewidth}{!}{\includegraphics{Figures/vae_app.png}}
    \caption[VAE-Poisson Process.]{Predicting the next-step action and interval time in \cite{mehrasa2019variational}. Past action and time pairs $(a_{n-1}, \tau_{n-1})$ are used to stochastically produce the future action-time pair from sampled latent variable $z_{n}$ as well as the Action/Time Decoders. Figure reproduced with permission from \cite{mehrasa2019variational}}.
    \label{fig:vae_app}
\end{figure}
\begin{figure}[htb]
    \centering
    \resizebox{.5\linewidth}{!}{\includegraphics{Figures/when_will.png}}
    \caption[Multi-task model for joint prediction of action and time.]{Model introduced in \cite{abu2018will} for action and time prediction via regression. Notice the observed input action is pre-processed into a one-hot encoding and the input time is framed as a real value scalar. Subsequent processing alternates use of fully connected (FC) layers and Gated Recurrent Units (GRUs). The whole scope of the future requires the recursive inference. Figure reproduced with permission from \cite{abu2018will}.}
    \label{fig:when_will}
\end{figure}

Though the Poisson process has been known for modelling time arrival events, not all researchers adopt it. An alternative research direction modeled time as a real-valued output directly from regression models, e.g., using an MLP to generate the output \cite{mahmud2017joint, abu2018will, abu2019uncertainty, ke2019time, gammulle2019forecasting} as shown in Figure \ref{fig:when_will}: For any next-step action, the ``length of future action" and ``remaining length of current action" will be regressed from fully-connected layers. In comparison to previous Poisson methods \cite{mehrasa2019variational, mahmud2016poisson}, these approaches choose deterministic time models rather than the Poisson distribution and therefore their outputs for a given input will be fixed. An exception to this general trend instead assumes a Gaussian prior and approximates the mean and variance via learning \cite{abu2019uncertainty}.
\iffalse
In fact, there exist a third way to model time data: treating time as discrete categorical variables. A parallel work \cite{li2017time} conducted experiments on jointly learning the events happening time and category in recommendation systems, where they found modelling the time as categorical representation and optimizing it with cross-entropy consistently out-performs its real-value counter-part (See Section 4.2 Cross Entropy Loss on Time Prediction of \cite{li2017time}). At this very point, it seems that researchers resort to certain time representation empirically.
\fi

A third way to model temporal data is to treat time in terms of discrete categorical values. Along these lines, research on recommendation systems found that modelling time with a categorical representation and optimizing with cross-entropy consistently outperformed the use of real valued modelling \cite{li2017time}.
It is worth noticing that the range of the discrete categorical variable normally needs to be defined beforehand. For example, in image classifications, the ImageNet dataset defines 1000 categories and thus its models (\ie AlexNet) would output probability score vectors $\in \mathcal{R}^{1000}$. For discrete times, the maximum time index is often chosen as the time range value \cite{neumann2019future}.

To clarify the variability of the design choice for time representation, especially in video understanding tasks, a systematic study of the aforementioned choices was conducted \cite{neumann2019future}. This study grouped time representations into three categories, continuous, discrete and hybrid; see Table \ref{tab:time_representation}.
\begin{table}[htb]
\scriptsize
\centering
\begin{tabular}{|c|l|l|}
\hline
\multicolumn{1}{|c|}{Group} &       \multicolumn{1}{c|}{Method}                     & \multicolumn{1}{c|}{Detail}                                                               \\ \hline
\multirow{3}{*}{Discrete}   & One-in-many Classification & Quantize time in $\Delta{max}$ discrete bins and use classified index as results.                         \\ \cline{2-3} 
                            & Binary Classifiers         & $\Delta{max}$ independent binary classifiers for each time index.                                         \\ \cline{2-3} 
                            & Heuristic Heat-Map         & Generate 1d heat-map and choose the maximum position in heatmap.                            \\ \hline
\multirow{3}{*}{Continuous} & Direct Regression          & Real value regression.                                                                      \\ \cline{2-3} 
                            & Gaussian Distribution      & Estimate time as parameterized Normal $N(t | \mu, \sigma)$ distribution.                    \\ \cline{2-3} 
                            & Weibull Distribution       & Estimate tme as parameterized Weibull $p(t | \alpha, \beta) = 1 - e^{-(t/\alpha)^{\beta}}$. \\ \hline
Hybrid                      & Gaussian Mixture        & Gaussian Mixture of heat-maps. A hybrid model.                                              \\ \hline
\end{tabular}
\caption[Summary of time representations.]{Summary of time representations. $\Delta_{max}$ stands for the maximum time range in datasets.}
\label{tab:time_representation}
\end{table}

\iffalse
\begin{figure}[htb]
    \centering
    \resizebox{.5\linewidth}{!}{\includegraphics{Figures/time_rep_compare.png}}
    \caption{Comparison results of various time methods on BDD100K data. For evaluation metrics, higher Event Prediction Accuracy (EPA) means better performance whereas lower Time-to-Event Error (TTEE) and Model Surprise (MS) mean better performance. Table from \cite{neumann2019future}.}
    \label{fig:time_compare}
\end{figure}
\fi

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
    \begin{tabular}{lccc}
    \toprule
    Model & EPA[\%] & TTEE[s] & MS \\
    \midrule
    \midrule
    One-in-many Classifier & 71.78 & 2.66  & N/A \\
    Binary Classifier & 75.90  & 3.21  & N/A \\
    Direct Regression & 71.11 & 3.81  & N/A \\
    Gaussian Distribution & 66.77 & 5.77  & 10.91 \\
    Weibull Distribution & 55.66 & 8.31  & 3.20 \\
    Heuristic Heatmap & 76.15 & 2.64  & 3.88 \\
    \midrule
    Gaussian Mixture of Heuristic Heatmap & 78.70  & 2.04  & 2.69 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
  \label{tab:bdd_time}%
  \caption[Comparison results of various time modelling methods.]{Comparison results of various time methods on BDD100K dataset. For evaluation metrics, higher Event Prediction Accuracy (EPA) means better performance, whereas lower Time-to-Event Error (TTEE) and Model Surprise (MS) mean better performance. Table reproduced with permission from \cite{neumann2019future}.}
    \label{fig:time_compare}
\end{table}%


In empirical comparison, there were three discrete methods (One-in-many Classifier, Binary Classifier and Heuristic Heatmap), three continuous methods (Direct Regression, Gaussian Distribution and Weibull Distribution) and one hybrid method (Gaussian Mixture of Heuristic Heatmap). These time representations are evaluated on the BDD100K car stop anticipation dataset \cite{yu2020bdd100k} that measures the Event Prediction Accuracy (EPA), Time-To-Event-Error (TTEE) and Model Surprise (MS). In their results (shown in Table \ref{fig:time_compare}), almost all continuous time modelling methods fall short of achieving comparable performance with discrete methods. Moreover, the hybrid model performs the best. This observation on video understanding agrees with the experimental results from other related fields \cite{li2017time}.

One possible explanation to validate the above phenomenon could be the effect of temporal scope prior, $\Delta_{max}$, enforced by discrete models. Continuous methods generate outputs in the real positive number realm, $\mathcal{R}^{+}$, while discrete methods pre-confine the output range to $\mathcal{R}^{\lambda \Delta_{max}}$ ($\lambda$ a scaling factor). This prior implicitly informs the learned prediction model about the reasonable temporal output range, whereas the continuous counterpart tries to cover the whole positive value realm. 
Another potential reason for the observed pattern of results could be the time data format. Most such work (\eg \cite{abu2018will, mehrasa2019variational, ke2019time}) assumes the minimum unit of time is in the unit of seconds, which corresponds to the data formatting common in adopted datasets (\eg Breakfast dataset \cite{kuehne2016end}). Discrete time format matches the original scheme naturally while continuous ones incur unnecessary decimals. Recent work succeeds the discrete time scheme and trains a conditional GAN model based on Gumbel discrete sampling to jointly enhance the accuracy and diversity in both future action semantics and times \cite{zhaodiverse}; see Figure \ref{fig:zhao_eccv2020}. Previous efforts tended to be challenged in producing realistic (accurate) and diverse predictions.

In summary, approaches to joint prediction of actions and their times can be categorized along three dimensions, as follows.

\noindent\textbf{Difference in Inputs:} Similar to the discussion on input data use in Section \ref{Sec:future_action_1}, research in time prediction also can be categorized according to the input data type. Some work aims at learning the mapping from high-level information, extracted from raw observations, to the future. These efforts usually depend on extracted/estimated activity labels and segmented temporal duration as input \cite{abu2018will, abu2019uncertainty, mehrasa2019variational, ke2019time, zhaodiverse}. Other work relies on raw video inputs \cite{neumann2019future, mahmud2017joint}.

\noindent\textbf{Difference in stochastic process:} The majority of work relies on a stochastic process for future actions and times. Various approaches employ a Poisson \cite{mahmud2016poisson,mehrasa2019variational} or Gaussian distributions \cite{abu2019uncertainty} or a generative adversarial network \cite{zhaodiverse}. A few outliers deterministically produce their anticipations \cite{abu2018will, li2017time}.
\begin{figure}[htb]
    \centering
    \resizebox{.9\linewidth}{!}{\includegraphics{Figures/zhao_eccv2020.png}}
    \caption[Diverse action and time prediction.]{Method introduced in \cite{zhaodiverse} that used a sequential modeller (Distance Normalized Gumbel GAN) to produce the whole sequence of subsequent actions and times. Multi-modality is well supported for both action categories and time durations. Figure reproduced with permission from \cite{zhaodiverse}.}
    \label{fig:zhao_eccv2020}
\end{figure}

\noindent\textbf{Difference in prediction horizon:} Some work advocates for one-step future predictions. RNNs have been used to recursively generate next step (action, time) pairs (\eg  \cite{abu2018will}). To obtain the whole scope of the future, results of next-step prediction are reused as input for the next-next. This procedure repeats until it reaches the end of sequence (\eg \cite{mehrasa2019variational, gammulle2019forecasting, mahmud2017joint, neumann2019future}). Alternatively, other approaches generate the rest of the sequence in one shot (\eg \cite{zhaodiverse, abu2019uncertainty}).
Finally, work has made one-shot time independent predictions, so that predictions on remote time indices do not rely on previous ones \cite{ke2019time}. They achieve this goal by making predictions conditioned on the desired prediction index as an extra input. The evident downside of their work is the limited prediction scope.

%\textbf{Differece in output post-processing:} It must be mentioned that efforts that rely on the real-value outputs \cite{furnari2017next} faces limitations. Real-value based approach has found that it is necessary to normalized the time representation to $\in (0, 1)$ for the better learning convergence. Even for the testing phase,  where the overall video length should be assumed as unknown, 


\pagebreak


\section{Ego-Centric Action Prediction}
First person video analysis has attracted increasing attention due to the rich information contained in egocentric visual data and easier access to wearable recording devices. As seen in Figure \ref{fig:ego_centric}, ego-centric filming exhibits much closer viewing angles of objects, environments and interactions of daily activity. However, one critical difference from the third person view dataset (\eg UCF-101 \cite{soomro2012ucf101}) is the lack of notable motion of actors, \ie only the hand motion is typically visible. Moreover, since the camera moves along with its carrier, there usually exists large background motion as well as jittering in video frames.
\begin{figure}[htb]
    \centering
    \resizebox{.9\linewidth}{!}{\includegraphics{Figures/ego_centric.png}}
    \caption{Examples of Ego-centric activity footage.}
    \label{fig:ego_centric}
\end{figure}

Missing actors in activity videos makes classic human action analysis methodologies not naturally applicable and larger view-point changes as well as camera jittering makes motion feature extraction (\eg optical flow) very noisy. These obstacles incentivise researchers to tackle ego-centric data in a slightly different way. 

In the following, we group related research work into two main divisions: \textbf{1.} work that actively explores non-traditional visual cues (\ie hand motion, gaze salience, object trajectory, etc.) that are uniquely salient in ego-view data; \textbf{2.} work that follows regular techniques and treats ego-centric data in a similar way as third-person view data. In this approach, even though videos are filmed under ego-centric view, performed actions can be inferred without direct observation of large portions of the actor.
We first discuss the former division, unique features, from the perspectives of gaze, hand and object.

\noindent\textbf{Gaze Information:} One beneficial information source hidden in first person video is gaze information. Gaze moving on/off of a certain object can closely correspond to the occurrence/ending of a particular action. Much work has enjoyed the incorporation of such information (\eg \cite{su2017predicting, lepetit2009epnp, shen2018egocentric}). 
 
Yet, gaze localization does not come freely. One way to obtain gaze information is the 3D reconstruction of actors and then inferring the gaze direction from head direction and body poses \cite{su2017predicting}. In that work, the authors virtually stabilized input first person video and reconstructed 3D body pose by applying cylindrical projection using existing tools \cite{lepetit2009epnp}. This processing provided labels for the location, orientation, and velocity of actors with pixel level precision, as seen in Figure \ref{fig:gaze} (a). The inferred gaze direction and body pose together indicate the potential social interactions among players and thus contribute to anticipating future behaviors. 
\begin{figure}[ht]
    \centering
    \begin{minipage}{.3\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/cylindrial_geometry.png}
    \caption*{(a)}
    \end{minipage}
    \begin{minipage}{.25\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/egosupervision.png}
    \caption*{(b)}
    \end{minipage}
    \begin{minipage}{.4\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/gaze_event.png}
    \caption*{(c)}
    \end{minipage}
    \caption[Examples of ego-centric methods.]{(a) Examples of 3D reconstruction of stablized basketball players and the recovered gaze direction $\mathbf{z}$ from \cite{su2017predicting}. (b) Example of next player intention groundtruth generated from ego-supervised prior knowledge with high probability score denoted as red, while low score is blue. (c) Gaze-events defined from \cite{shen2018egocentric} where object target detection (white rectangles) \textbf{overlaps} with gaze fixations (white circle). Subfigures (a), (b) and (c) reproduced with permission from \cite{su2017predicting}, \cite{bertasius2017using} and \cite{shen2018egocentric}, respectively.}
\label{fig:gaze}
\end{figure}

Another way to gain gaze information is through manual annotation and/or use of additional instrumentation. Though expensive, it is easily doable through eye-tracking devices. Assuming decent gaze estimation is given, an effort proposed a model to focus on video frames where target objects and gaze estimations coincide \cite{shen2018egocentric} (shown in Figure \ref{fig:gaze} (c)). They paid special attention to gaze-events and distilled attention values from event-fired frames to assist action prediction.  

Some other work that considers gaze as an important visual cue focused efforts on predicting future gaze fixations from observed frames \cite{zhang2017deep}. Their framework proceeded in a similar way to video frame prediction but output binary gaze heat-maps. However, the authors did not show any application of the predicted gaze on other related problems.

\noindent\textbf{Hand Information:} In first person videos, hand movement typically is the major human visible action. Human-object interactions often consist of a movement part and one or more object parts, with “take bowl” as an example. First person videos capture complex hand movements during a rich set of interactions, thus providing a powerful workhorse for studying the connection between hand actions and future representation.

In imitation of the acquisition of gaze information, hand motion can be either annotated or online estimated. For example, an extant hand shape detector \cite{zhu2014pixel} can be applied to obtain a hand mask across frames \cite{shen2018egocentric}. The use of the estimated hand mask is straightforward: Overlaying the hand mask on RGB input frames.
In other recent work, it is proposed to use the hand movement trajectory as an output regularizer \cite{liu2019forecasting}. The authors enforced the learned network model to jointly predict future actions, future hand trajectories and interactive hotspots (regions where interaction would happen with high likelihood). In an ablation study, it was shown that the three related tasks were complementary to each other.
%This multi-task learning on three related tasks are proven to be complementary to each other in their ablation studies.

\noindent\textbf{Object Information:} 
Objects that are interacted with are another potentially important source of information for predicting future actions. While such information can be generally useful for action prediction, it can be of particular importance in first-person video where the movements of the actor may be obscured. 
%Since human activities often can be decomposed in terms of atomic actions and interactions with objects, intelligent wearable systems would benefit from the ability to anticipate user-object interactions.

An early work along these lines investigated the relevance of egocentric object trajectories in the task of next-active-object prediction \cite{furnari2017next}. Provided that an object detector/tracker is available, they proposed to analyze object trajectories observed in a small temporal window to detect next-active-objects before the object-interaction is actually started. 
%\textcolor{red}{\sout{Objects being held by the action performer are dubbed as active objects and other non-manipulated objects in the same scene as passive objects.}}

A more recent work incorporated information on the spatial location of objects into ego-centric action prediction \cite{furnari2019would}. The authors adopted a pretrained deep object detector to localize objects and merged their deep features with another two feature modalities (\ie RGB and optical flow) captured globally from the entire frame. However, their major inference engine is a novel Rolling-Unrolling (RU) LSTM system and object features are simply used as input. In an ablation study, they found that inclusion of the object information helped achieve much better results compared to neglecting that information.

As mentioned above, there are other efforts that treat ego-data no differently from regular third person data.
\iffalse
Examples includes \cite{furnari2018leveraging} which leverages uncertainty nature in future actions and proposes Top-K loss to enhance the accuracy. They process ego-centric with well-known action deep network model pre-trained on third person videos datasets. Another unique line of research is from the group of Kris. M. Kitani \cite{rhinehart2017first,bokhari2016long}. They ask an interesting question: what if the next ego viewpoint action will happen in scenes or places that does appear in current views (\eg current action happens in living room while next activity will take place in kitchen room)? 
\fi
One such approach processed ego-centric video with a standard deep neural network action recognition model pretrained on third person video datasets \cite{damen2018scaling,wang2015towards}, but now fine-tuned for ego-action future prediction assisted by top-loss \cite{furnari2018leveraging}. Other research made use of standard third person analysis tools to anticipate events that might occur in different places than those currently in view \cite{rhinehart2017first, bokhari2016long}. For example, the current view is of the living room, while the future activity will occur in the kitchen.
In response, they proposed to merge 3D point cloud location information obtained from a SLAM system with interactive objects and high-level scene labels to do the predicting 
%(seen in right of Figure \ref{fig:ego}).

\iffalse
\begin{figure}[htb]
    \centering
    \begin{minipage}{.6\textwidth}
    \includegraphics[width=1.\textwidth]{Figures/ego_active_traj.png}
    \end{minipage}
    \begin{minipage}{.35\textwidth}
    \includegraphics[width=1.\textwidth]{Figures/ego_slam.png}
    \end{minipage}
    \caption{(Left) detected object trajectory from \cite{furnari2017next}. (Right) Prediction of future activity and happening place, with the help of 3D point cloud construction \cite{bokhari2016long}.}
\label{fig:ego}
\end{figure}
\fi
Another interesting use of ego-centric data is exploiting the prior knowledge behind the ego-centric data for unsuperivsed learning \cite{bertasius2017using}. The authors researched predicting the next cooperative player with regard to the ego-centric viewer. 
%For example, this approach allows prediction of which teammate the camera carrier will interact with next. 
Instead of manually annotating the groundtruth target, they generated pseudo groundtruth in an unsupervised fashion by using ego-centric assumptions; see Figure \ref{fig:gaze} (b).
%Their work begins by producing human player detections using pretrained networks and then builds its own groundtruth unsupervisedly.
%: \textbf{1}. an ego location prior that captures the locations in a first-person image where the bounding box predictions are usually most dense; \textbf{2.} an ego size prior that focuses on players who are physically closer to the camera carrier; \textbf{3.} an ego pose prior that assumes right parts of the person’s body will have
%smaller coordinate values in a first-person image than the left part, if facing the camera. Finally, they learned a network to map the raw RGB frames input to a player intention heat-map, such as Figure \ref{fig:gaze}(b). In follow-up work \cite{bertasius2016first}, they suggested embedding first person coordinates, to better locate the future interaction object positions.


\section{Datasets and Performance}
In this section, we describe datasets, evaluation metrics and performance in evaluation of the majority of future action prediction approaches discussed above.

\pagebreak
\begin{landscape}
\begin{longtable}{@{}@{} l r r r r r r}
% pairs: absolute number (percentage)
\toprule%
 \centering
 & \multicolumn{1}{c}{{{\bfseries Year}}}
 & \multicolumn{1}{c}{{{\bfseries No. Videos}}}
 & \multicolumn{1}{c}{{{\bfseries No. Actions}}}
 & \multicolumn{1}{c}{{{\bfseries Avg. Len}}}
 & \multicolumn{1}{c}{{{\bfseries Domain}}}
 & \multicolumn{1}{c}{{{\bfseries Data-Modality}}} \\

\cmidrule[0.4pt](l{0.25em}){1-1}%
\cmidrule[0.4pt](r{0.25em}){2-2}%
\cmidrule[0.4pt](r{0.25em}){3-3}%
\cmidrule[0.4pt](r{0.25em}){4-4}%
\cmidrule[0.4pt](r{0.25em}){5-5}%
\cmidrule[0.4pt](r{0.25em}){6-6}%
\cmidrule[0.4pt](r{0.25em}){7-7}%
% \midrule
\endhead

\myrowcolour
\textbf{BDD100K} \cite{yu2020bdd100k} & 2020 &
100,000 & 3 & \highest{40s} & \highest{Car-Stop} & RGB \\ 

\textbf{EGTEA} \cite{fathi2011learning} & 2019 & 
39,596 & 149 & \highest{-} & \highest{Human Interaction} & RGB, HandMask, Gaze \\

\myrowcolour
\textbf{PIE} \cite{rasouli2019pie} & 2019 &
56,000 & 60 & \highest{-} & \highest{Action} & RGB, Skeleton\\

\textbf{Epic-Kitchen} \cite{damen2018scaling} & 2018 &
272 & 125 & \highest{3s} & \highest{Activity, HOI} & RGB \\ 

\myrowcolour
\textbf{MultiTHUMOS} \cite{yeung2018every} & 2017 & 
400 & 65 &  \highest{4.03s} & \highest{Activity} & RGB \\

\textbf{JAAD} \cite{kotseruba2016joint} & 2017 & 346 &
11 & \highest{6.39s} & \highest{Action} & RGB, BB \\

\myrowcolour
\textbf{CAD120} \cite{koppula2013learning} & 2013 & 
120 & 20 & \highest{-} & \highest{Action, HOI} & RGB+D, Skeleton\\

\textbf{50 Salads} \cite{lea2017temporal} & 2012 &
50 & 17 & \highest{-} & \highest{Action-traffic} & RGB, Temporal-Seg \\

\myrowcolour
\textbf{MPII-Cooking}  \cite{rohrbach2012database} & 2012 &
44 & 65 & \highest{600s} & \highest{Activity-cooking} & RGB \\

\textbf{VIRAT} \cite{oh2011large} & 2011 & 
59 & 10 & \highest{219} & \highest{Activity} & RGB+D, Skeleton\\

\myrowcolour
\textbf{UCI-OPPORTUNITY} \cite{roggen2010collecting} & 2010 &
10h & 5 & \highest{-} & \highest{Action, HOI} & RGB, Sensor \\

\textbf{Human-Object-Interaction}  \cite{gupta2009observing} & 2009 & 
10 & 6 & \highest{-} & \highest{Action} & RGB \\
\bottomrule
\caption[Summary of datasets for future action prediction.]{Summary of datasets for future action prediction.} \\
\end{longtable}
\end{landscape}

\textbf{Epic-Kitchen} \cite{damen2018scaling} is a large first-person video dataset, which is captured by 32 subjects in 32 different kitchens. The videos in this dataset contain daily activities of the subjects, i.e., no scripts are provided to instruct the subjects. This makes this dataset very natural and challenging. There are 272 training videos, which are captured by 28 subjects. Each video contains multiple action segments, which are categorized into 125 classes. Since the annotations of the testing videos are not available, the training videos are used to perform cross-validation for evaluation. Specifically, the training videos are randomly split into 7 splits, each containing videos of 4 subjects.

\textbf{50 Salads} \cite{lea2017temporal} contains 50 videos which are performed by 25 subjects. Each subject is preparing two mixed salads. There are 17 fine-grained action classes. Researchers often perform 5-fold cross-validation for evaluation using the splits provided by the authors. There are a total of 50 videos that are filmed over 100 hours.

\textbf{Breakfast} \cite{kuehne2014language} contains 1,712 videos of 52 different actors making breakfast. Overall, there are 48 fine-grained action classes and about 6 action instances for each video. The average duration of the videos is 2.3 minutes and the longest video is 10 minutes.

\textbf{MultiTHUMOS} \cite{yeung2018every} is a challenging dataset for action recognition, containing 400 videos of 65 different actions. On average, there are 10.5 action class labels per video and 1.5 actions per frame and thus it is suitable for long-term activity anticipations.

\textbf{BDD100K} \cite{yu2020bdd100k} consists of 100,000 driving video sequences each 40 seconds of length, accompanied with basic sensory data such as GPS, velocity or acceleration. In total, there are 31k vehicle stopping and 21k not-stopping sequences for training, and 4.6k stopping and 3.1k non-stopping sequences for evaluation.

\textbf{VIRAT} \cite{oh2011large} is a collection of approximately 25 hours of surveillance video taken from various scenes, with an average of 1.6 hours per scene. Multiple HD cameras are used to capture at 1080p or 720p at rates between 25 to 30 Hz. The view angles of cameras towards dominant ground planes ranged between 20 and 50 degrees by stationing cameras mostly at the top of buildings to record a large number of event instances across area, while avoiding occlusion as much as possible.
%\textbf{JAAD} \cite{kotseruba2016joint}

\textbf{PIE} \cite{rasouli2019pie} comprises 1,842 pedestrian tracks captured using an on-board monocular camera, while driving in urban environments with various street structures and crowd densities. Overall, the ratio of pedestrian non-crossing to crossing events is 2.5 to 1. All video sequences are collected during daylight under clear weather conditions. The videos are continuous, allowing us to observe the pedestrians from the moment they appear in the scene until they go out of the field of view of the camera.

\textbf{MPII-Cooking} \cite{rohrbach2012database} contains 44 instances of cooking activity, which are continuously recorded in a realistic setting. Predictable high level activities are about preparing 14 kinds of dishes, including: making a sandwich, making a pizza, and making an omelet, etc. There are overall 65 different actionlets as building blocks shared among various cooking activities, such as cut, pour, shake, and peel.

\textbf{GTEA Gaze} \cite{fathi2011learning} contains 17 sequences of meal preparation activities performed by 14 different subjects, with the spatial resolution of 640 \& $\times$ 480. It contains the subjects’ gaze location in each frame and the corresponding activity labels. Its extension, \textbf{GTEA Gaze++} \cite{fathi2012learning}, contains 37 sequences performed by 6 subjects of preparing 7 types of meals. Their latest collection, EGTEA \cite{li2018eye}, comes with 10, 321 action instances from 19 verb, 53 noun and 106 action classes.

\textbf{UCI-OPPORTUNITY} \cite{roggen2010collecting} was created in a sensor-rich environment for the machine recognition of human activities. They deployed 72 sensors of 10 modalities in 15 wireless and wired networked sensor systems in the environment, on the objects, and on the human body. The data are acquired from 12 subjects performing morning activities, yielding over 25 hours of sensor data. It contains five high level predictable activities (Relaxing, Coffee time, Early Morning, Cleanup, Sandwich time), 13 low level actionlets (e.g., lock, stir, open, release), and 23 interactive objects (e.g., bread, table, glass).

\textbf{CAD120} \cite{koppula2013learning}  has 120 RGB-D videos of four different subjects performing 10 high-level activities. The data is annotated with object affordance and sub-activity labels and includes groundtruth object categories, tracked object bounding boxes and human skeletons. The set of high-level activities are making cereal, taking medicine, stacking objects, unstacking objects, microwaving food, picking objects, cleaning objects, taking food, arranging objects, having a meal. The set of sub-activity labels are reaching, moving, pouring, eating, drinking, opening, placing, closing, scrubbing, null and the set of affordance labels are reachable, movable, pourable, pourto, containable, drinkable, openable, placeable, closable, scrubbable, stationary.

\textbf{HOI} \cite{gupta2009observing} is the Maryland Human-Object Interactions dataset, which consists of six annotated activities: answering a phone call, making a phone call, drinking water, lighting a flash, pouring water into container and spraying. These activities have about three to five action units each. Constituent action units share similar human movements: 1) reaching for an object of interest, 2) grasping the object, 3) manipulating the object, and 4) putting back the object. For each activity, there are 8 to 10 video samples.

\textbf{Evaluations} for future action prediction can be grouped into two division: \textbf{1.} Reporting the mean average precision of future action label classifications at a single pre-planned future time horizon; \textbf{2.} Reporting the mean average precision over a range of time horizons. The former is widely adopted for activity singleton or sequence anticipations, while the latter for joint activity and time duration anticipations.

In this report, we summarize dataset performances that are frequently  and extensively investigated in recent years regarding the above two divisions. Additional results can be found in the original papers. For the first division, we showcase the next activity anticipation results on the Epic-Kitchen dataset \cite{damen2018scaling}. In its standard setting, the prediction horizon is fixed as the future \textbf{1s}. Epic-Kitchen dataset has complete annotations for fine-grained sub-action denoted as \textbf{Verb}, interactive objects as \textbf{Noun} and high-level action category as \textbf{Action}. Accuracies for all three attributes will be reported. Two sets of accuracy, namely top-1 that only accept the best prediction for evaluation and top-5 that would accept 5 best guesses as final results, are listed to shed light on the robustness of their models; see Table \ref{tab:epic_rst}.

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption[Future action prediction accuracy on future 1 second for Epic-Kitchen.]{Future action prediction accuracy on future 1 second for Epic-Kitchen. ``set1'' stands for the test set whose scenes appear in the training set, whereas ``set2'' for the test set that does not share scenes with the training set.}
    \begin{tabular}{c|cccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{}} & \multirow{2}[2]{*}{Method} & \multicolumn{3}{c}{Top/Top5 Accuracy} \\
    \multicolumn{1}{c}{} &       & Verb  & Noun  & Action \\
    \midrule
    \midrule
    \multirow{6}[1]{*}{set1} & 2S-CNN \cite{damen2018scaling} & 29.76/76.03 & 15.15/38.65 & 4.32/15.21 \\
          & TSN \cite{damen2018scaling}  & 31.81/76.56 & 16.22/42.15 & 6.00/18.21 \\
          & TSN+MCE \cite{miech2019leveraging} & 27.92/73.59 & 16.09/38.32 & 10.76/25.28 \\
          & Trans R(2+1)D \cite{miech2019leveraging} & 30.74/76.21 & 16.47/42.72 & 8.74/25.44 \\
          & RULSTM \cite{furnari2019would} & 33.04/79.55 & 22.78/50.95 & 14.39/33.73 \\
          & FHOI \cite{liu2019forecasting} & 36.25/79.15 & 23.83/51.98 & 15.42/34.29 \\
    \midrule
    \midrule
    \multirow{6}[0]{*}{set2} & 2S-CNN \cite{damen2018scaling} & 25.23/68.66 & 9.97/27.38 & 2.29/9.35 \\
          & TSN  \cite{damen2018scaling} & 25.30/68.32 & 10.41/29.50 & 2.39/9.63 \\
          & TSN+MCE \cite{miech2019leveraging} & 21.27/63.66 & 9.90/25.50 & 5.57/25.28 \\
          & Trans R(2+1)D \cite{miech2019leveraging} & 28.37/69.96 & 12.43/32.20 & 7.24/19.29 \\
          & RULSTM \cite{furnari2019would} & 27.01/69.55 & 15.19/34.28 & 8.16/21.20 \\
          & FHOI \cite{liu2019forecasting} & 29.87/71.77 & 16.80/38.96 & 9.94/23.69 \\
    \end{tabular}%
  \label{tab:epic_rst}%
\end{table}%

For the second division, we follow the Mean-over-Class (MoC) evaluation metrics to measure the performance of joint activity category and duration anticipation on two datasets, Breakfast \cite{kuehne2014language} and 50Salads \cite{lea2017temporal}; see Tables \ref{tab:breakfast_rst} and \ref{tab:breakfast_rst_est} for Breakfast and Tables \ref{tab:50salads_rst} and \ref{tab:50salads_rst_est} for 50Salads. The evaluation method, MoC, represents the average accuracy over the entire prediction horizon.

For singleton activity prediction, as seen in Table \ref{tab:epic_rst}, the current performance is far from satisfactory and thus definitely deserves more effort. For the joint anticipation of activity and time duration, the performance produced from methods that take groundtruth (action, time) observations as input achieves decent results even for remote time indices (\eg 75\% accuracy for 50\% future video horizon predictions for the Breakfast dataset \cite{gammulle2019forecasting}, as seen in Table \ref{tab:50salads_rst}). However, given (action, time) inputs from off-the-self algorithms (Table \ref{tab:breakfast_rst_est} and \ref{tab:50salads_rst_est}), which do not guarantee noisy-free estimation, performance on both datasets drops dramatically. This observation reflects the fact that the current bottle-neck is the accuracy of action detection and segmentation methods more so than the prediction algorithms.


\begin{landscape}
\begin{table}[t]
%\resizebox{\linewidth}{!}{
    \centering 
    \setlength{\tabcolsep}{0.7em} % for the horizontal padding
    {\renewcommand{\arraystretch}{1.3}% for the vertical padding
\noindent\begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} c c c c  c c c c} 
\toprule % Top horizontal line
% \multicolumn{3}{|c|}{10}
Observation & \multicolumn{4}{c}{20\% } & \multicolumn{4}{c}{30\%} \\ 
\cmidrule(l){2-5}
\cmidrule(l){6-9}
Prediction & 10\% & 20\% & 30\% & 50\% &  10\% & 20\% & 30\% & 50\% \\ % Column names row
\midrule % In-table horizontal line
RNN \cite{abu2018will} & 0.6035 & 0.5044 & 0.4528 & 0.4042 & 0.6145 & 0.5025 & 0.4490 & 0.4175 \\ % Content row 1
CNN \cite{abu2018will} & 0.5797& 0.4912 & 0.4403 & 0.3926 & 0.6032 & 0.5014 & 0.4518 & 0.4051\\ % Content row 2
TOS-Dense \cite{ke2019time} & 0.6446 & 0.5627 & 0.5015 & 0.4399 & 0.6595 & 0.5594 & 0.4914 & 0.4423 \\ % Content row 3
R-HMM (\textbf{Avg})\cite{abu2019uncertainty} & 0.5039 & 0.4171 & 0.3779 & 0.3278 & 0.5125 & 0.4294 & 0.3833 & 0.3307\\
R-HMM (\textbf{Max})\cite{abu2019uncertainty} & 0.7884 & 0.7284 & 0.6629 & 0.6345 & 0.8200 & 0.7283 & 0.6913 & 0.6239 \\
NDR-GAN (\textbf{Avg})\cite{zhaodiverse} & 0.7222 & 0.6240 & 0.5622 & 0.4595 & 0.7414 & 0.7132 & 0.6530 & 0.5238 \\ % Content row 3
NDR-GAN (\textbf{Max})\cite{zhaodiverse} & 0.8208 & 0.7059 & 0.6851& 0.6406 & 0.8336 & 0.7685 & 0.7213 & 0.6406 \\ % Content row 3
NeualMemory \cite{gammulle2019forecasting} & 0.8720 & 0.8524 & 0.8102 & 0.7547 & 0.8790 & 0.8279 & 0.8210 & 0.7630 \\ % Content row 3
\midrule % In-table horizontal line
\end{tabular*}
}
\caption[Results on Breakfast dataset with groundtruth observations.]{Breakfast Dataset results of dense anticipation mean over classes (MoC) accuracy with groundtruth (action, time) observations as inputs. \text{Avg} stands for averaged results across 16 samplings, while \text{Max} stands for taking the best result among 16 samples.}
\label{tab:breakfast_rst}
\end{table}
\begin{table}[t]
%\resizebox{\linewidth}{!}{
    \centering 
    \setlength{\tabcolsep}{1em} % for the horizontal padding
    {\renewcommand{\arraystretch}{1.3}% for the vertical padding
\noindent\begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} c c c c  c c c c} 
\toprule % Top horizontal line
% \multicolumn{3}{|c|}{10}
Observation & \multicolumn{4}{c}{20\% } & \multicolumn{4}{c}{30\%} \\ 
\cmidrule(l){2-5}
\cmidrule(l){6-9}
Prediction & 10\% & 20\% & 30\% & 50\% &  10\% & 20\% & 30\% & 50\% \\ % Column names row
\midrule % In-table horizontal line
RNN \cite{abu2018will} & 0.1811 & 0.1720 & 0.1594 & 0.1581 & 0.2164 & 0.2002 & 0.1973 & 0.1921 \\ % Content row 1
CNN \cite{abu2018will} & 0.1790 & 0.1635 & 0.1537 & 0.1454 & 0.2244 & 0.2012 & 0.1969 & 0.1876\\ % Content row 2
TOS-Dense \cite{ke2019time} & 0.1841 & 0.1721 & 0.1642 & 0.1584 & 0.2275 & 0.2044 & 0.1964 & 0.1975 \\ % Content row 3
R-HMM (\textbf{mode})\cite{abu2019uncertainty} & 0.1671 & 0.1540 & 0.1447 & 0.1420 & 0.2073 & 0.1827 & 0.1842 & 0.1686\\
TCN-Cycle \cite{farha2020long} & 0.2588 & 0.2342 & 0.2242 & 0.2154 & 0.2966 & 0.2737 & 0.2558 & 0.2520 \\
Attn-GRU \cite{ng2020forecasting} & 0.2303 & 0.2228 & 0.2200 & 0.2085 & 0.2650 & 0.2500 & 0.2408 & 0.2361 \\
\midrule % In-table horizontal line
\end{tabular*}
}
\caption[Results on Breakfast dataset without groundtruth observations.]{Breakfast Dataset results of dense anticipation mean over classes (MoC) accuracy \textbf{without} groundtruth (action, time) observations as inputs.}
\label{tab:breakfast_rst_est}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
\centering 
    \setlength{\tabcolsep}{1em} % for the horizontal padding
    {\renewcommand{\arraystretch}{1.3}% for the vertical padding
\noindent\begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} c c c c  c c c c} 
\toprule % Top horizontal line
% \multicolumn{3}{|c|}{10}
Observation & \multicolumn{4}{c}{20\% } & \multicolumn{4}{c}{30\%} \\ 
\cmidrule(l){2-5}
\cmidrule(l){6-9}
Prediction & 10\% & 20\% & 30\% & 50\% &  10\% & 20\% & 30\% & 50\% \\ % Column names row
\midrule % In-table horizontal line
RNN \cite{abu2018will} & 0.4230 & 0.3119 & 0.2522 & 0.1682 & 0.4419 & 0.2951 & 0.1996 & 0.1038 \\ % Content row 1
CNN \cite{abu2018will} & 0.3608 & 0.2762 & 0.2143 & 0.1548 & 0.3736 & 0.2478 & 0.2078 & 0.1405\\ % Content row 2
TOS-Dense \cite{ke2019time} & 0.4512 & 0.3323 & 0.2759 & 0.1727 & \textbf{0.4640} & 0.3480 & 0.2524 & 0.1384 \\ % Content row 3 
R-HMM (\textbf{Avg}) \cite{abu2019uncertainty} & 0.3495 & 0.2805 & 0.2408 & 0.1541 & 0.3315 & 0.2465 & 0.1884 & 0.1434\\
R-HMM (\textbf{Max}) \cite{abu2019uncertainty} & 0.7489 & 0.5875 & 0.4607 & 0.3571 & 0.6739 & 0.5237 & 0.4673 & 0.3664 \\
NDR-GAN (\textbf{Avg})\cite{zhaodiverse} & 0.4663 & 0.3562 & 0.3191 & 0.2137 & 0.4613 & 0.3637 & 0.3310 & 0.1945\\ % Content row 3
%Proposed (\textbf{Top-1}) & 0.4903 & 0.3998 & 0.3596 & 0.2537& 0.4926 & 0.4582 & 0.3572  &  0.2646 \\
NDR-GAN (\textbf{Max})\cite{zhaodiverse} & 0.5150 & 0.3845 & 0.3606 & 0.2762 & 0.5079 & 0.4754 & 0.3783  &  0.2908  \\
NeualMemory \cite{gammulle2019forecasting} & 0.6996 & 0.6433 & 0.6271 & 0.5216 & 0.6810 & 0.6229 & 0.6118 & 0.5667 \\ % Content row 3
\midrule % In-table horizontal line
\end{tabular*}
}
\caption[Results on 50Salads dataset with groundtruth observations.]{Results for the 50Salads dataset of dense anticipation mean over classes (MoC) accuracy with groundtruth (action, time) observations as inputs.} 
\label{tab:50salads_rst}
\end{table}

\begin{table}
\centering 
    \setlength{\tabcolsep}{1em} % for the horizontal padding
    {\renewcommand{\arraystretch}{1.3}% for the vertical padding
\noindent\begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} c c c c  c c c c} 
\toprule % Top horizontal line
% \multicolumn{3}{|c|}{10}
Observation & \multicolumn{4}{c}{20\% } & \multicolumn{4}{c}{30\%} \\ 
\cmidrule(l){2-5}
\cmidrule(l){6-9}
Prediction & 10\% & 20\% & 30\% & 50\% &  10\% & 20\% & 30\% & 50\% \\ % Column names row
\midrule % In-table horizontal line
RNN \cite{abu2018will} & 0.3006 & 0.2543 & 0.1874 & 0.1349 & 0.2164 & 0.2002 & 0.1973 & 0.1921 \\ % Content row 1
CNN \cite{abu2018will} & 0.2124 & 0.1903 & 0.1598 & 0.0987 & 0.2914 & 0.2014 & 0.1746 & 0.1086\\ % Content row 2
TOS-Dense \cite{ke2019time} & 0.3251 & 0.2761 & 0.2126 & 0.1599 & 0.33512 & 0.2705 & 0.2205 & 0.1559 \\ % Content row 3 
R-HMM (\textbf{mode}) \cite{abu2019uncertainty} & 0.2486 & 0.2237 & 0.1988 & 0.1282 & 0.2910 & 0.2050 & 0.1528 & 0.1231\\
TCN-Cycle \cite{farha2020long} & 0.3476 & 0.2841 & 0.2182 & 0.1525 & 0.3439 & 0.2370 & 0.1895 & 0.1589 \\ %
Attn-GRU \cite{ng2020forecasting} & 0.3932 & 0.3139 & 0.2701 & 0.2388 & 0.4173 & 0.3273 & 0.3144 & 0.2639 \\
ACC-Grammar \cite{piergiovanni2020adversarial} & 0.3950 & 0.3320 & 0.2590 & 0.2120 & 0.3950 & 0.3150 & 0.2640 & 0.1980 \\
%Content row 3
\midrule % In-table horizontal line
\end{tabular*}
}
\caption[Results on 50Salads dataset without groundtruth observations.]{Results for the 50Salads dataset of dense anticipation mean over classes (MoC) accuracy \textbf{without} groundtruth (action, time) observations as inputs.} 
\label{tab:50salads_rst_est}
\end{table}
\end{landscape}



==> BODY/Backup/chapter4.tex <==
% \section{Introduction}
\iffalse
Action/activity associated analysis discussed in the previous chapter is one of the most important fields in video predictive understanding. Yet, there are many other equally interesting video problems that also find non-trivial benefits from researching the predictive property of videos.
In this chapter, we perform a review on some additional video prediction tasks.

Along the same line of our definition of \textbf{Predictive} in chapter \textbf{1}, our discussions here also focus on the \textbf{temporal extrapolation} attribute of targeted tasks.

\section{Video Pixel Predictions}
Foreseeing the future can be achieved by various perspectives, \ie predicting the future semantic information such as action or activity labels. However, some researchers find it more interesting to predict the visual future, \eg future pixel-wise appearance, not just the semantic one. The basic assumption is that visual future is very informative and a vivid pixel prediction would naturally provide strong support to many other down-stream tasks simultaneously. For example, with an accurate prediction of future traffic camera frames, any off-the-self recognition \& detection \& segmentation algorithms can be applied to operates differing duties, without designing any novel algorithms.
  

    \subsection{Frame Prediction}
    \subsection{Semantic Prediction}
\section{Trajectory Prediction}

Bla bla..

\section{Human Motion Forecasting}

Bla bla..

% \subsection{Theory and Procedures}

Bla bla..

% \subsection{Simulated and Measured Results}

Bla bla..

\section{Predictive Coding for Unsupervised Representation Learning}

\section{Datasets}

And the conclusion is, same old same!
\fi

\section{Motivation}
In the computer vision community, video predictive understanding refers to the inference of the unobserved future from the current as well as historical information. 
From a theoretical perspective, video predictive understanding is of importance as it addresses the basic scientific question of how to extrapolate future events from previous observations. From a practical perspective, the ability to predict future events from videos has potential to provide positive impact for wide range of artificial intelligence applications, including autonomous vehicle guidance, effective time response to surveillance data and improved human computer interaction.

In video understanding, researchers are generally pursuing answers for two fundamental focal points: \textbf{what to predict} and \textbf{how to predict}. The intuition behind the first focus is that the future can be of several forms (\ie future semantic, physical trajectories, poses or pixel distributions) and it is non-trivial to explore its most feasible format to better assist real-life applications. To this end, diverse sub-areas have appeared that work on predicting the future in various knowledge domains. The second focus explores various mathematical techniques, information sources and data modalities to enhance the prediction accuracy.

\section{Overview of video predictive understanding}
The major sub-areas of video predictive understanding are pixel prediction, semantic segmentation prediction,  trajectory prediction, human motion prediction, predictive coding as well as early action prediction and future action prediction. While the focus of this review is early action prediction and future action prediction, in the next several paragraphs, each of these sub-areas will be briefly presented to provide context.

\textbf{Video pixel prediction} is concerned with generating pixelwise values for potential future images extrapolated temporally from previous observations. Early approaches to this problem attempted generation through learning procedures without adequate attention to basic elements of image structure (e.g., spatial gradients and optical flow) and yielded results that had undesirable artifacts (e.g., blurry images) as well as short prediction horizons \cite{ranzato2014video, srivastava2015unsupervised, oh2015action}. Subsequent work that explicitly considered such basic image structure yielded improved results \cite{mathieu2015deep, liu2017video}; however, prediction horizons were little extended. To support longer term predictions, work has relied on higher-level image analysis (e.g., body keypoint and motion analysis \cite{villegas2017decomposing, oliu2018folded, villegas2017learning}). Other work has made use of stochastic generative models to capture uncertainty \cite{lee2018stochastic, babaeizadeh2017stochastic, villegas2019high}. Yet other work has decomposed motion and appearance for separate processing via latent variables to better control outcomes \cite{tulyakov2018mocogan, hsieh2018learning, rybkin2018learning, jaegle2018predicting} as well as emphasized object centric motions \cite{ye2020object, wu2020future, ye2019compositional}. Generation of naturalistic future images beyond short time horizons remains challenging. Also, it is worth noting that such predictions may lend little insight into higher-level (e.g., semantic) understanding of future events.

\iffalse
\textbf{Video pixel prediction} is one popular such direction with an attention on hallucinating the future imagery pixel intensity. The idea is intuitive in that a pixel-wise future mimics the real visual future that could be captured by human vision systems. 
%That is to say, by foreseeing an authentic visual future, any premade detection or recognition algorithms should be deployed straightforwardly to obtain the craved future information. Thus, the key is to recover the future pixels as realistic as possible. 
Some early work has encountered difficulties, \ie blurred effects, in producing recognizable future nature images \cite{ranzato2014video, srivastava2015unsupervised, oh2015action}. It has been proposed to count on image gradient difference or flow constraints to motivate sharper predictions \cite{mathieu2015deep, liu2017video}. However, these work endures a critical issue with regard to the short prediction horizon. 
%Most of them could not make sensible predictions on remote futures (\ie 10 seconds and onward). 

Later on, some work has been done to elongate valid predictions via supplementary assistance from motion or low-level body key-points \cite{villegas2017decomposing, oliu2018folded, villegas2017learning}. Some others advocate stochastic generative models for future predictions as the future could probably contain uncertainty \cite{lee2018stochastic, babaeizadeh2017stochastic, villegas2019high}. Another fashion of video prediction rather focuses on manipulations. It has been suggested to decompose motion and content in predictions to the extent that manipulating on the latent variables can lead to controlled outcomes \cite{tulyakov2018mocogan,hsieh2018learning}. Recently, some efforts have been done to emphasize the beneficial effect of attending to object-centric motions in video predictions \cite{ye2020object, wu2020future, ye2019compositional}. 
\fi

\begin{figure}[htp]
    \centering
    \resizebox{.65\linewidth}{!}{\includegraphics[width=4cm]{Figures/pixel_semantic.pdf}}
    \caption[Video pixel prediction in upper row and semantic segmentation prediction in lower row.]{Video pixel prediction in upper row and semantic segmentation prediction in lower row. A desired future scene parsing (semantic segmentation of a future frame) can be obtained via either: \textbf{1.} pixel prediction and then semantic segmentation; \textbf{2.} direct semantic prediction.}
    \label{fig:pixel_semantic}
\end{figure}

\textbf{Video segmentation prediction} bears high similarity with pixel prediction, yet it differs in that its outputs come in terms of pixelwise semantic labels (\eg road, tree, etc.). 
\iffalse
For example, predicting the future road condition can be approached in either one of the following mindsets: \textbf{1.} Do prediction on future frames and then operate segmentation algorithms; \textbf{2.} Directly predict the future segmentation. Video semantic prediction adopts the second philosophy and related work mostly focuses on pixel-wise segmentation \cite{luc2017predicting, luc2018predicting, jin2017predicting}, with few on detections (\eg \cite{singh2018predicting, yagi2018future}). As noted in Figure \ref{fig:pixel_semantic}, future semantic is less complex in terms of pixel intensity distributions (\eg each pixel at most possesses a single class label), compared with raw future images (\eg each pixel ranges in $(0, 255)$ for each channel of RGB) and thus it has been favored. 
In terms of methodology, approaches in this field are alike to those in pixel predictions, nonetheless with the objective function substituted with the desired downstream task (\ie instance segmentation). 
\fi
To achieve future semantic segmentations, one might either perform pixel prediction followed by standard semantic segmentation operations or directly infer future semantic segmentations. The latter approach is the focus of video semantic segmentation prediction. Figure \ref{fig:pixel_semantic} provides a visual illustration of the differences between pixel and semantic segmentation prediction. While different in output (i.e., single valued pixel labels vs. RGB values), semantic segmentation work has largely leveraged similar techniques as used for pixel predictions, with various levels of emphasis on purely appearance vs. dynamics semantics \cite{luc2017predicting, luc2018predicting, jin2017predicting, singh2018predicting, yagi2018future}. An important distinction is that the objective functions for semantic segmentation approaches typically rely on the downstream task (e.g., instance segmentation) compared to pixel predictions. 

\textbf{Video trajectory prediction} is another intensively investigated sub-area of video predictive understanding.
In this case, observed video is preprocessed into sequences of 2D coordinates that capture the trajectories of objects of interest (e.g., humans, vehicles). The goal is to predict a future sequence in the same format.
Early work focused on the forecasting of a single trajectory \cite{kitani2012activity}, whereas more recent research has expanded to the prediction of crowd trajectories \cite{alahi2016social, gupta2018social, sadeghian2019sophie, liang2019peeking, sadeghian2019sophie, ivanovic2019trajectron, salzmann2020trajectron++}. Among these efforts, some implicitly fused crowd information, by passing messages between targets, to better infer every single future trajectory \cite{alahi2016social, gupta2018social}. Other work actively embraced rich scene context to assist their predictions \cite{liang2019peeking, sadeghian2019sophie}. Yet other work explicitly used physical social distance to encode the crowd effect for their trajectory forecasting \cite{ivanovic2019trajectron, salzmann2020trajectron++}. Recently, a spatio-temporal version of a graph neural network has been found useful for this task \cite{mohamed2020social}. As with other areas of video prediction, long term prediction remains an outstanding challenge and while some work has made use of scene context, it is likely that much more can be explored in that direction. 

\textbf{Human motion prediction} focuses on foreseeing future human motion in the form of body key-points (\eg 24 body part coordinates \cite{martinez2017human}). This task is very akin to trajectory prediction, since its data is abstract key-points rather than raw pixels. The majority of work in this sub-area used recurrent neural networks in a Encoder-Decoder fashion to produce future pose sequences \cite{martinez2017human, fragkiadaki2015recurrent}. 
On top of that, a wide range of machine learning techniques have been applied to this sub-area, including attention \cite{tang2018long}, contrastive learning \cite{coskun2018human} and imitation learning \cite{wang2019imitation}. An important (and remaining) challenge in this area is to restrict generated motions to be realistic, even while varied. Advances along this direction have exploited geometric constraints \cite{gui2018adversarial} as well as generative modeling \cite{aliakbarian2020stochastic, wang2019imitation}.
\iffalse
Some work exploited geometric cues \cite{gui2018adversarial} and some others focused on producing diverse yet realistic future human motions with generative modelling \cite{aliakbarian2020stochastic, wang2019imitation}. A special study explored the prediction of human motion from video audios \cite{shlizerman2018audio}. Many learning philosophy, such as metric learning and imitation leaning, are found useful for this task \cite{coskun2018human}. 
\fi

\textbf{Video predictive coding} is rather different from the above sub-areas. It is concerned with coding raw video data into a high dimensional representation in such a way that it can be easily decoded into the future of input video. The learned representations are used as video features for various tasks. For example, early work along this line conducted video prediction learning with an objective to extrapolate frame-wise deep features that ultimately were applied to unsupervised action recognition \cite{srivastava2015unsupervised}. Follow on work enriched this idea with contrastive learning \cite{han2019video}. A recent effort that tried a similar idea on unsupervised video skeleton action recognition also observed success \cite{su2020predict}. Another effort found predictive coding meaningful for video retrievals \cite{yu2020encode}. 
A particularly interesting aspect of this line of work is that it requires no annotation, as the learning and feature distillation simply makes use of already available video data.
Researchers find this valuable since predictive coding is self-contained and requires zero annotations, thus it alleviates the heavy burden of human labeling.

\textbf{Action prediction} is principally concerned with the prediction of human actions. Among many important research topics in video understanding, action recognition arguably has received the most interest and efforts in the last decade \cite{kang2016review, kong2018human}. With tremendous advances achieved and various experiments explored in recent years, some researchers have refocused on the ability to \textit{foresee} the happening of certain actions rather than recognize the completed ones. The reason can be easily seen from the practical application point of view: Full action executions often take elongated time spans and thus performing the recognition algorithm after the action is completed would naturally lose the capability to react in real-time, which, however, in many conditions is essential.

\begin{figure}[h]
    \centering
    %\resizebox{.5\linewidth}{!}{\includegraphics[width=4cm]{Figures/action_prediction2.PNG}}
    \resizebox{1.\linewidth}{!}{\includegraphics{Figures/examples_fig.pdf}}
    \label{fig:examples}
    \caption[Representative applications of early action recognition and future action prediction.]{Representative applications of early action recognition and future action prediction. Sub-figure (a)-(b) depict the use of early action recognition on reducing the computational budget of portable devices (\eg mobile phones typically lack GPU and memory space to process elongated videos) and on diminishing the response gap for fast feedback systems (\eg human-robot interactions and self-driving vehicles). Sub-figure (c) plots the application for future action prediction: Anticipating pedestrian behaviors at traffic intersections.}
\end{figure}

As examples: In the video anomaly detection task, people expect a vision system that automatically spots any potentially disruptive events as early as possible and then sends out an alarm before any damage is done. Obviously, such a system is required to either recognize harmful actions in effective time or anticipate their happening in advance in space and time. Similarly, in the automonous driving setting, desirable unmanned vehicles need to be highly sensitive to pedestrian walking intentions, in particular at traffic crossings, to avoid accidents. To achieve that goal, the vehicle system needs to leverage contextual information from the scene (\eg traffic lights and crossings) together with pedestrian ego-motion, standing pose, heading angle, etc., to judge their most likely next action and respond in kind.

In general, based on application scenarios, researchers mainly explore two finer divisions: early action recognition and future action prediction. The former refers to recognizing the on-going actions as early as possible, while the latter to making plausible predictions on future actions that would happen after the execution of the current one. The focus of this review is on early action recognition and future action prediction. Figure \ref{fig:examples} provides illustrative examples of both early action recognition and future action prediction.

\iffalse
Largely, there are two subdivisions to this sub-area. The first, early action recognition, addresses the inference of a single action before it is complete. The second, future action prediction, addresses longer term inference of future, follow-on actions. Both of these areas have received extensive attention in the past decade, \eg \cite{kong2014discriminative, chakraborty2014context, abu2018will, zhao2019spatiotemporal, li2014prediction} and will be reviewed in detailed in Chapter \ref{CH2}.
\fi


\iffalse
The last division of video predictive understanding is the prediction of action/activity. Some researchers argued that recognition of actions should be advanced in time and thus proposed to investigate how early can computer vision system recognize actions well. On the other hand, some others are more into foreseeing the future activities. Both of them have received tremendous attentions in the last decade \cite{kong2014discriminative, chakraborty2014context, abu2018will, zhao2019spatiotemporal, li2014prediction}.
\fi

\iffalse
In the following chapter, our discussion will focus on two main topics: \textbf{1.} Fundamental mathematical tools for video sequence analysis; \textbf{2.} Early action recognition and future activity anticipation. The first topic lays out necessary knowledge towards how to model visual sequences, which will be reflected in cases studies in the second topic.
We choose to meticulously survey on action/activity since they receive the most efforts in terms of the scope of mathematical models, the variousness and modality of datasets and the richness of sub-divisions.
\fi

\section{Outline}
This chapter has served to motivate and provide a broad overview of video predictive understanding. Chapter \ref{CH2} will provide a detailed review of early action recognition. Chapter \ref{CH3} will provide a detailed review of future action prediction. Finally, Chapter \ref{CH4} will provide conclusions, including suggestions for future research directions.

==> BODY/Backup/chapter5.tex <==
% \section{Datasets \& BenchMark}
\section{Current trends}
Throughout this survey, various video predictive tasks have been discussed, among which early action recognition and future action prediction have been studied in a detailed manner. Even though recent efforts have advanced the performance of both tasks greatly, in this section we summarize current status and discuss the potential urgent challenges awaiting to be solved.

\subsection{Early action recognition}
Current trending approaches on early action recognition greatly rely on success from the video action recognition area, where large scale datasets and powerful video discriminative feature representation are frequently advanced via deep learning. As examples: Recent progress comes from use of enhanced video features (\eg \cite{zhao2019spatiotemporal,kong2018adversarial} Temporal segment network \cite{wang2015towards}, \cite{wang2019progressive} ResNet \cite{he2016deep} and \cite{shi2018action} Inception network \cite{szegedy2015going}). Among this progress, the mutual information based (Section 3.2.2) and the propagation based (Section 3.2.3) are the front runners in terms of performance on recent benchmark datasets. These two approaches share the intuition that partial information needs to be augmented, yet they follow different methodologies to achieve that end.

Mutual information based approaches focus on reconstructing a complete video representation through feature matching or knowledge distillation. In these approaches, partial features are mapped to global features, mostly with feature-wise Euclidean distance measuring the feature similarity, with little or no explicit temporal modeling.
In contrast, propagation based approaches focus on the temporal evolution of videos and endeavor to recover useful features at each time step. Some classic temporal sequential models (\eg Kalman filtering and Markov Decision process) are frequently revisited in these approaches; see \cite{zhao2019spatiotemporal, zeng2017visual}.

For early action recognition, a remaining demand is extending study to un-constrained environments. Popular datasets (\eg UCF-101 \cite{soomro2012ucf101}) in existing research are known to be carefully trimmed and controlled.  Though they are collected from real-life video sources and called ``in the wild'', the contained motion is almost always clean, visible and smooth. Such quality is not always guaranteed in many real-life environments. Moreover, the fact that early action recognition still performs poorly in the BIT dataset indicates that most current methods are sensitive to the dataset, \eg between class variation is much greater in UCF-101 compared to BIT.
%\ie UCF-101 has large intra-class variants since its classes are quite dissimilar, while BIT owns near actions (\eg \textit{pushing} and \textit{patting}). 

Even though some research has revealed that certain action categories are relatively easy to recognize early \cite{kong2018adversarial}, it would be favorable to understand the reason behind the observed patterns. For datasets that can be readily recognized early on (\eg UT-Interaction), the decisive factor for the success is still unknown. Also as noted by \cite{zhou2018temporal}, for more complex daily actions that would include compound reasoning structure, \ie ``trying to pour water into a glass, but missing so it spills next to it" from the Something2something dataset, the accuracy is extremely unsatisfactory (around $10\%$ accuracy), indicating that current high accuracy on most examined datasets does not equal to the desired reasoning ability in computational intelligence. 

Another critical issue is the current evaluation procedure for early action recognition. As mentioned in Section 3.1, action videos are often being divided into $k \in (10\%, 100\%)$ progress levels and the recognition accuracy with regard to each level will be reported. However, such a split design may be too coarse to allow for understanding of real actions that unfold more incrementally. For some actions that can be completely executed within 10\% of frames, a high recognition accuracy is misleading. 
Furthermore, little has been done to consider the relative importance of early recognition as a function of action (e.g., elder people falling requires earlier recognition to be useful compared to many other actions).
%Furthermore, as to the question \textit{how early is enough}, different actions should be evaluated with more cautions. Since some dangerous action (\eg elder people falling down) would require a earlier recognition than others, to be practical efficient.

\subsection{Future Action Prediction}
Mainstream approaches for future action prediction either use temporal sequential tools for building the causal relation between past and long-term future at a high-level (\eg semantics and/or time durations), or make use of visual features (\eg objects, eye gazes, hand motions, poses, etc.) extracted from recently observed frames for anticipating the immediate next action label. In the first research line, the Recurrent Neural Network (RNN) as well as its hybrids with certain traditional sequence models (\eg RNN-HMM \cite{abu2019uncertainty} or Poission-LSTM \cite{mehrasa2019variational}) are the major workhorse, as seen in recent efforts. The high level semantics are often preprocessed with off-the-shelf algorithms and these approaches, in most cases, resorted to a data-driven methodology to learn parameters for both RNNs and classic models. 

In the second direction (\ie more direct use of visual features), the focus is employing multi-modal data with the most effectiveness. Typically, the fusion of distinct information is achieved through one of the following strategies: stacking them together as a single input (\eg \cite{furnari2019would}); designing a multi-task learning framework with extra data modality as regularizers (\eg \cite{liu2019forecasting}); fusing them using a hierarchical structure (\eg \cite{jain2016recurrent, rasouli2020pedestrian}). As means to produce the future action label, researchers often resorted to the recently advanced deep ConvNet features (\eg I3D features \cite{carreira2017quo}) and learned a classifier from the training data.

For joint activity and time duration prediction, it is still an open question as to how to represent times most effectively. Modelling time as a discrete variable seems to perform well, yet it fails when any future time duration exceeds its pre-defined scope. In contrast, the continuous representation would either be too coarse (\eg real value regression) or constrained into a uni-modal distribution (\eg Gaussian), which naturally lacks the ability to model multi-modality of times (\eg \textit{boiling\_egg} can take longer time for a hard boiled egg as well as shorter time for a soft boiled one).

Currently, the prediction of activities often happens in a narrow spatial scope, such as kitchen areas or cooking stations. Yet, daily activities often take place with a transition of locations, \ie fetching objects in another room can incur a scene change.
Even for the ambitious Epic-Kitchen dataset \cite{damen2018scaling}, the default assumption is that all objects relevant for prediction are visible in the current frame. Indeed, there seems to be only one effort that considers prediction across multiple locations \cite{rhinehart2017first} and the dataset has yet to be shared.
%There is few work that jointly modeled future activity category and locations with the help of 3D point cloud and SLAM systems (\eg \cite{rhinehart2017first}), which allows for anticipations beyond the current view space. However, such a work and its data set does not maintain a public accessible portal. Even for a more recent and relative large scale dataset, Epic-Kitchen \cite{damen2018scaling}, the default setup for anticipation assumes the future interactive object to be visible in the current frame, which is less sensible.

As discussed in Section 3.2, in long-term future action predictions, researchers typically resort to the mapping between the high-level semantics \cite{li2014prediction} (\eg model a mapping from a sequence of observed activities to a sequence of future activity labels).
Indeed, in some cases researchers have gone to the extreme of taking groundtruth labels for the observed portion of the video as input.
This setting is reasonable in that an extended video clip contains many frames, which prohibit online low-level feature computation as well as storage, and high-level semantics summarize long videos in a manageable and meaningful way.
Nonetheless, this scheme ignores the rich visual elements that have been demonstrated to be worth exploiting in other areas and which are worth further consideration in long-term predictions.
Moreover, approaches that employ groundtruth labels as input avoid the critical issue of how to extract the labels video in the first place.


\section{Future Work}
In this final section, several directions for future work are suggested.

\textbf{Improved interpretability} of algorithms and representations is necessary to truly understand the early action recognition and future action prediction tasks and their enabling mechanisms. 
From the perspective of understanding the learning methods, there is a demand to further research \textit{what has been learned} by proposed solutions. As an example: In student-teacher learning \cite{wang2019progressive}, it would be beneficial to monitor and understand the teaching process. In the example of deep Kalman feature propagation \cite{zhao2019spatiotemporal}, answers are needed for questions such as how does learning based Kalman filtering affect the error accumulation and what are the motion kernels learned for feature propagation (\eg are they mimicking a warping function)? Both analytic (e.g., \cite{hadji2017spatiotemporal}) and visualization methodologies (e.g., \cite{feichtenhofer2020deep}) have potential for shedding light on these questions.

\textbf{Integrating feature extraction with prediction} is an urgent concern for most high-level based approaches. It has been seen that a decent semantic estimation of input partial observations plays a critical role in making satisfactory long-term prediction (\eg see Table \ref{tab:breakfast_rst} and Table \ref{tab:50salads_rst}), while a noisy estimation deteriorates the performance remarkably (\eg see Table \ref{tab:breakfast_rst_est} and Table \ref{tab:50salads_rst_est}). To tackle this discrepancy, it might be worth integrating the future prediction into the semantic extraction, with an objective to improve the robustness of future prediction with noisy inputs.

\textbf{Better modelling of long-term correlation} is necessary to achieve scalable prediction of activities. The cue that can precisely indicate the future could possibly hide in details that are far away from current observations, and thus it is essential to keep logging historical information and effectively spot the correlations between minor details and future events. Though some efforts have been made for action recognition (\eg the authors in \cite{wu2019long} designed a long-term filter bank to keep a track of remote historical features), its effects on other areas stays unknown and it is likely beneficial to revisit such an ability for future action predictions.


\textbf{Stronger temporal sequence modelling tools} are always favorable to video understanding. The majority of mathematical tools mentioned in Chapter 2 are theoretically grounded and widely adopted. Recently, however, it has been proposed to explore other advances, such as temporal convolution \cite{lea2017temporal}, which challenges the use of memory hidden states, or transformers \cite{girdhar2019video}, which get rid of the recurrent structure and yet demonstrates superior results, as alternatives to classic sequence modelling tools. These innovate findings break the traditional design where the temporal modelling has to be sequential and mostly Markovian. Such directions are worth further investigation. 
%So, it is worth rethinking about the efficiency of current methods and exploring any potential stronger models.

\textbf{Learning efficiency} is another concern that closely associates with most recent learning approaches, since these methods prerequisite sufficient size of datasets and expensive annotations, which incurs huge amounts of human labeling efforts, data cleaning and unavoidable data biases. So, how to learn meaningful information without strong supervision or with noisy labels awaits to be answered. Besides, there is also a need for an adaptive learning framework that can assimilate unseen data and new action categories, since people's daily activities would evolve along with their own development. An active and continuous learning framework would be of great benefit.
Unsupervised approaches to representational learning, e.g., as introduced under the topic of predictive video coding in Chapter 1, provide a potentially useful avenue to explore to address these concerns.


\textbf{Creation of better datasets and experimental protocols} is necessary to better validate prediction algorithms. From the perspective of datasets and evaluation metrics, it is worth understanding the specific observation ratios that are practically valuable in real-life conditions with regard to actions, and therefore re-evaluating existing approaches using this new criterion. It is also worth investigating the correlation between the video observation ratio and action evolution ratio of popular datasets, in order to examine the validation of current early recognition evaluation metrics. 

\section*{Acknowledgements}
The authors thank Michael S. Brown and Kosta G. Derpanis for the insightful comments they provided on this review.




==> BODY/Backup/chapter6.tex <==
\section{Conclusion}

In conclusion, as Brad Pitt and his chio wife said in \cite{BibtexKey}, NTU researchers have no life. So, go get a life!

\section{Future Work}

A few suggestions are provided for related future works:

\begin{enumerate}

\item Bla.. 

\item Bla..

\item Bla..

\end{enumerate}

==> BODY/ch01_intor_back.tex <==
% \textcolour{red}{We need to discuss on the organization of the sections in this chapter.}

\section{Motivation}
Over the past several years, computer vision research has shifted from concentrating on ConvNet-based to transformer-based models. This transition is evident from the proposal of numerous transformer models for video classification (\eg~\cite{arnab2021vivit,liu2021swin,fan2021multiscale,liu2022video,li2022mvitv2}) and segmentation (\eg~\cite{mei2021transvos,duke2021sstvos,cheng2021mask2formervid}). In parallel, video segmentation continues to be a subject of great interest due to its theoretical as well as practical importance. From a theoretical perspective, video segmentation addresses the fundamental problem of assigning category membership to video on a pixel-wise basis. From a practical standpoint, applications to downstream video understanding tasks, e.g., autonomous driving and video editing, also contribute to continuing growth in interest from the research community.
%Over the past several years, computer vision research has shifted from an emphasis on ConvNet-based models to transformer-based models. This transition is evident from the proposal of numerous transformer models for video classification~\cite{arnab2021vivit,liu2021swin,fan2021multiscale,liu2022video,li2022mvitv2} and segmentation~\cite{mei2021transvos,duke2021sstvos,cheng2021mask2formervid}. More specifically, video segmentation continues to be a subject of great interest due to its theoretical as well as practical importance. From a theoretical perspective video segmentation serves as ground for developing pixel level video understanding algorithms. From a practical perspective, applications about downstream video understanding tasks, \eg autonomous driving, video editing resulted in continuing growth in interest from research community.

Corresponding to the recent emphasis on transformers and video segmentation, a number of related literature reviews have appeared, e.g., \cite{wang2021survey, vandenhende2021multi, selva2023video}. Still, there remains a gap, as surveys have yet to appear that provide a detailed study of transformers for video segmentation. More specifically, the following gaps need to be filled. First, recent surveys of approaches to video segmentation mainly cover ConvNet-based methods to the problem~\cite{yao2020video,wang2021survey}. Alternatively, recent surveys of video transformers focus on video classification~\cite{selva2023video}. To our knowledge, surveys of transformer-based video segmentation models have yet to be available. Second, recent surveys of video segmentation mainly focused on two categories of video segmentation: object-based and semantic-based segmentation~\cite{wang2021survey}. However, due to the wide variety of video segmentation tasks and the recent formulation of several new tasks (e.g., depth-aware video panoptic segmentation~\cite{qiao2021vip} and audio-guided video object segmentation~\cite{pan2022wnet}), there is a need for a survey with a taxonomy of task categories. Third, previous surveys do not include component-wise discussion of the segmentation approaches~\cite{yao2020video,wang2021survey}. However, recent models for different types of video segmentation exhibit several high-level components with a specialization in the design of the components. Several unified models also have been proposed to do multiple segmentation tasks using a single model. Component-wise discussion of video segmentation models can play a vital role in understanding the generalization of multiple segmentation tasks in a single model. Fourth, although there is some recent research on the interpretability of transformers in vision, there is a gap in the availability of a survey covering transformer interpretability.   

%Corresponding to the recent emphasis on transformers and video segmentation, corresponding literature reviews have appeared, e.g., \cite{wang2021survey, vandenhende2021multi, selva2023video}. Still, there remains a gap, as no surveys have appeared that provide a detailed study of transformers for video segmentation, in particular. More specifically, the following gaps need to be filled. First, recent surveys on approaches to video segmentation mainly cover ConvNet-based approaches to the problem~\cite{yao2020video,wang2021survey}. On the other hand, recent surveys on video transformers focus on video classification~\cite{selva2023video}. To our knowledge, no surveys on transformers-based video segmentation models are available. Second, recent surveys on video segmentation mainly focused on two categories of video segmentation: object-based and semantic-based segmentation~\cite{wang2021survey}. However, due to the wide variety of video segmentation tasks and the recent formulation of several new tasks (e.g., depth-aware video panoptic segmentation and audio-guided video object segmentation), there is a need for a survey with a taxonomy of task categories. Third, previous surveys~\cite{yao2020video,wang2021survey} does not include component-wise discussion of the segmentation approaches. However, recent models for different categories of video segmentation tasks exhibit several high level components with specialization on the design of the components. Several unified models has also been proposed to do multiple segmentation tasks using a single model. Component-wise discussion of video segmentation models can play a vital role in understanding the generalization of multiple segmentation tasks in a single model. Fourth, although there is some recent research on the interpretability of transformers in vision, there is a gap in the availability of a survey covering transformer interpretability.   


To address the above concerns, we present a survey on transformers for video segmentation. In this survey, we compile a taxonomy of video segmentation tasks, a component-wise analysis of recent transformer models for video segmentation and a discussion of transformer interpretability. 




\section{Overview of video segmentation}
%Definition
Video segmentation is a fundamental computer vision task that divides each frame into regions based on specific qualitative objectives, \eg delineation of objects, motion, actions and semantics. Segmentation algorithms assign each pixel a label from a finite set of classes to delineate the pixel's membership. This label set depends on the qualitative criteria that define an output space based on the application of interest. Based on the qualitative criteria, there are various categories of video segmentation tasks, e.g., object segmentation, actor-action segmentation and semantic segmentation~\cite{wang2021survey}. This inference from colour space to label space supports analysis and application for downstream objectives of an artificial intelligence processor or a human observer. Applications of interest include video surveillance~\cite{tian2005robust}, human-object interaction~\cite{zhou2020cascaded} and autonomous driving~\cite{chen2015deepdriving}. 


%Challenges
Video segmentation shares many challenges with single image segmentation (e.g., photometric and geometric variation within a segment); however, additional challenges arise in the setting of temporal image streams, as segments need to be delineated and tracked or otherwise associated across time. Attendant challenges include occlusion, motion blur, camera motion and object deformation. Moreover, operation with multiple video frames incurs additional computational expense compared to single frames.
%Video segmentation shares many challenges with single image segmentation (e.g., photometric and geometric variation within a segment); however, additional challenges arise in the setting of temporal image streams, as segments need to be delineated and tracked or otherwise associated across time. Attendant challenges include, occlusion, motion blur, camera motion and object deformation. Moreover, operation with multiple video frames incurs additional computational expense compared to single frames.



%Application
Video segmentation is important for reasons both theoretical and practical. From a theoretical perspective, association of pixels according to common attributes (e.g., colour, texture, dynamics) to form meaningful segments (\eg objects, motion, actions) is a fundamental problem in visual information processing. Video segmentation also is useful for various applications including video compression~\cite{hadizadeh2013saliency}, object tracking~\cite{kim2002fast}, activity recognition~\cite{holloway2014activity}, video surveillance~\cite{tian2005robust}, robotics~\cite{xu2016deep} and autonomous driving~\cite{chen2015deepdriving}. More generally, video segmentation allows for manipulation of each segment independently, tracking objects of interest, recognizing human activities, analyzing scene content, compressing video data and retrieving specific segments or objects from a video database based on their semantic content or visual appearance. Despite being very challenging, the theoretical interest and application areas have driven a continuing increase in research efforts on video segmentation. 





\section{Early approaches to video segmentation}
Given its theoretical and practical motivation, video segmentation has attracted much research effort for decades \cite{wang2021survey,thounaojam2014survey,zhang2006overview}. Although numerous categories of video segmentation have proliferated lately \cite{wang2021survey}, early approaches primarily focused on the most basic video segmentation task of foreground-background separation. Early proposals for video segmentation are mainly analytic approaches that apply geometric constraints along with heuristics to design a solution. In addition to their historical importance, some analytic methods or components from those approaches are still relevant in the literature. The dominant analytical techniques of the early attempts fall into four categories: background subtraction, trajectory-based, object proposal-based and saliency-based. The remainder of this subsection overviews each of these approaches.


%Given its theoretical and practical motivation, video segmentation has attracted much research effort for decades \cite{wren1997pfinder, stauffer2000learning,elgammal2002background,han2011density,brox2010object,ochs2013segmentation,chen2015video,shi2000normalized,ochs2012higher,fragkiadaki2012video,lee2011key,ma2012maximum,zhang2013video,fu2014object,koh2017primary,koh2018sequential,rahtu2010segmenting,papazoglou2013fast,faktor2014video,wang2015saliency,tsai2016semantic,hu2018unsupervised}. Video segmentation has attracted significant research attention for a long due to its wide variety of application areas. Although numerous categories of video segmentation have proliferated lately \cite{wang2021survey}, early approaches primarily focused on the most basic video segmentation task of foreground-background separation. Early proposals for video segmentation are mainly analytic approaches that apply geometric constraints along with some heuristics to design a solution. In addition to their historical importance, some of the analytic approaches or some components from those approaches are still relevant in the literature. The then dominant analytic approaches roughly fall into four categories: background subtraction approaches, trajectory-based approaches, object proposal-based approaches and saliency-based approaches. The remainder of this subsection overviews each of these approaches.


\paragraph{Background subtraction.}
Background subtraction approaches typically rely on heuristic assumptions about the background in the scene, e.g., pixels along frame boundaries are likely to be background. These approaches then attempt to detect moving objects by comparing pixel attributes to those of the hypothesized background. Connected component algorithms are used to estimate the connected region corresponding to an object or other distinctive region. Therefore, the above process is called background subtraction. Overall, video object segmentation is achieved by constructing a representation of the scene called the background model and then finding deviations from the model for each input frame. 


There are various background subtraction methods that have been proposed in the literature. The variety of the proposed approaches primarily differ in terms of the heuristics and types of background model used \eg stationary background \cite{wren1997pfinder, stauffer2000learning,elgammal2002background,han2011density}, background undergoing 2D parametric motion \cite{ren2003statistical,barnich2010vibe} and background undergoing 3D motion \cite{irani1998unified,torr1998concerning,brutzer2011evaluation}. They commonly use multi-class statistical models of colour pixels with a single Gaussian or a Gaussian Mixture Model (GMM). All of these methods rely on the restrictive assumption that the camera is stable and slowly moving; so, they are sensitive to model selection (2D or 3D) and cannot handle many challenging cases such as non-rigid objects and dynamic backgrounds. %The pioneering work using background subtraction model is based stationary background model well known as Pfinder\cite{wren1997pfinder}. They proposed an approach for real time human tracking which generates segmentation of moving humans as an intermediate step. Pfinder adopts a Maximum A-posteriori Probability (MAP) approach to detection and tracking of the human body using simple 2D models for arbitrarily complex but single-person scenario. Subsequent improvement has attempted to improve the model of this approach by using multinomial statistical model or mixture of Gaussian\cite{stauffer2000learning}. 
A detailed overview and comparison of background subtraction based video object segmentation is available elsewhere~\cite{brutzer2011evaluation}.  
         

\paragraph{Point trajectories.}
Other early analytic approaches for video segmentation initially cluster point trajectories and use them as prior information to obtain the foreground object. The common motivation of these approaches is considering motion as a perceptual cue for segmenting a video into separate objects and point trajectories have potential to support analysis of motion information over long periods~\cite{shi1998motion}. Interestingly, the notion of ``common fate'' for grouping points and objects can be traced to Gestalt psychology studies of perceptual organization \cite{kohler1970gestalt}. Point trajectory-based methods generally use optical flow~\cite{brox2010object,ochs2013segmentation,chen2015video} or feature tracking ~\cite{shi2000normalized,ochs2012higher,fragkiadaki2012video} as a way of obtaining motion information. Optical flow allows the analysis of motion information between two consecutive frames using dense motion fields. Feature tracking allows object motion analysis over a longer range by tracking a sparse set of key feature points over a larger temporal extent of a video sequence. Methods with point trajectories benefit from explicitly exploiting motion information compared to background subtraction methods. Still, they face the challenge of grouping local motion estimates into coherent segments.

%A prominent recent work using point trajectory is Video Object Segmentation via Dense Trajectories~\cite{chen2015video}. They presented an algorithm to segment moving objects in videos utilizing improved point trajectories. The proposed method has the following steps: point trajectory generation, measuring affinities between point trajectories, clustering the trajectories, obtaining graph partition from the clustering and finally, determining the object from the trajectory partitions. Their method begins with densely sampling points in multiple spatial scales and tracking them over frames using optical flow. Then they use a new affinity measure method using local and global information on point trajectories. Next, they introduced a hypothesis to identify foreground objects from the partitions. The proposed hypothesis regarded the trajectory partition with many areas near frame boundaries as background. Based on this hypothesis, they created a rectangular border and counted the number of each type of trajectory label lying within it. Then they regarded the labels with the maximum number of trajectories in the border as background trajectory labels. 



\paragraph{Object proposals.}
Object proposal based approaches generate likely regions (proposals) where objects appear based on colour, texture and motion. The proposals are then ranked based on confidence scores for subsequent aggregation across those that are highly ranked~\cite{lee2011key,ma2012maximum,zhang2013video,fu2014object,koh2017primary,koh2018sequential}. These methods vary in the information used to generate object proposals, the object proposal generation methods and the method of ranking and aggregating those proposals. By definition, these approaches are limited by their particular definitions of objects. Indeed, they typically are not applicable to segmentation tasks where the regions of interest cannot be readily considered as objects, e.g., semantic segmentation where interest may include texture and colour defined regions.


%One of the pioneering works in this category is ”KEY-SEGMENTS"~\cite{lee2011key}. They proposed a method to identify object-like segments in video frames using some static and dynamic cues. They then compute a series of binary partitions among those candidate object-like regions to discover hypothesis groups with persistent appearance and motion. Then they use each of these ranked hypotheses to estimate a pixel-level object labeling. Another approach in this category is augmentation and reduction process (ARP)~\cite{koh2017primary}. This approach generates candidate regions for the primary object using colour and motion edges and then estimates initial foreground object regions by exploiting the recurrence property of the primary objects. The recurrence property is that the primary object in a video is recurrent across frames. Finally, this approach uses an iterative refinement approach to augment those initial regions with missing parts or reduce them by excluding noisy parts of the object. Yet another approach, Sequential Clique Optimization (SCO)~\cite{koh2018sequential}, segments out primary object in a video sequence by solving the problem of finding cliques in a complete k-partite graph. They begin by extracting object instances in each frame of a video. Then they choose salient object instances in each frame to construct a salient object track through the sequence. For this purpose, they proposed a sequential clique optimization (SCO) technique to determine the cliques corresponding to salient object tracks. Then, the approach converts the object tracks to video object segmentation masks. 



\paragraph{Saliency based approaches.}
Other video segmentation approaches use saliency information as a prior or seed ~\cite{rahtu2010segmenting,papazoglou2013fast,faktor2014video,wang2015saliency,tsai2016semantic,hu2018unsupervised}. Typically, these approaches compute local salience based on feature contrast, with features being measurements of colour, texture and motion. Subsequently, local salience is aggregated across space and/or time in various ways, e.g., using Conditional Random Fields (CRFs) \cite{rahtu2010segmenting},  Non-Local Consensus voting (NLC) \cite {faktor2014video} or graph-based methods \cite{hu2018unsupervised,wang2015saliency}. Similar to object proposals, saliency approaches are limited by their definitions of salience and likely are inapplicable to cases where the regions of interest are not the most salient, e.g., small or low contrast regions.


%A notable early work~\cite{rahtu2010segmenting} proposed to segment salient objects by combining a saliency measure with a Conditional Random Field (CRF) model. This approach estimates saliency using a statistical framework with local feature contrast in illumination, colour and motion information. Then they formulate the segmentation as an energy minimization objective using a CRF model. Another notable early work using a saliency-based approach is non-local consensus voting (NLC)~\cite{faktor2014video}. This approach considers many common challenges: objects and the background scene may be highly non-rigid (e.g., waves in the sea); the camera may undergo a complex motion with 3D parallax; moving objects may suffer from motion blur, large scale and illumination changes. The approach begins with saliency votes at each pixel and iteratively refines them by ‘consensus voting’ of re-occurring regions across the video sequence. The consensus voting is non-local in space and time to enable the propagation of diverse and rich information across the entire video sequence. 



%A recent saliency-based proposal~\cite{wang2015saliency} produces the saliency maps using geodesic distances to background regions between subsequent frames and then builds global appearance models for foreground and background-based saliency maps. The features used to compute the frame-wise spatiotemporal saliency includes spatial edges and temporal motion boundaries. These spatiotemporal saliency maps work as prior information for object segmentation. Then, his approach combines the initial saliency maps, the global appearance model and the location model into a graph-cut energy minimization objective to compute the segmentation masks. Another saliency-based approach~\cite{hu2018unsupervised} proposed a new saliency map initialization method based on optical flow direction difference and minimum barrier distance. The saliency initialization technique uses the intuition that the optical flow on the boundary of an image differs significantly from the moving direction of the object of interest.  And then, this approach used a new neighborhood-graph-based diffusion method to diffuse initial saliency maps across superpixel nodes.  



\section{Overview of the transformer model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The transformer model was originally proposed for machine translation as a fully attention-based deep neural  network~\cite{vaswani2017attention}. Here, attention refers to the model performing data associations between elements of its input, i.e., attending to those elements. The model is a convolution free alternative to recurrent models for machine translation~\cite{luong2015effective,wu2016google}. The transformer model works on a sequence of tokens with the representation of each token as a feature vector ($N\times C$) where $N$ is the sequence length and $C$ is the feature dimension. The proposed model processes the entire input sequence as a whole, in contrast to the sequential processing of recurrent models. Processing the entire input at once allows better long range context aggregation in transformers compared to ConvNets. Subsequently, the transformer model was adapted to computer vision in the Vision Transformer (ViT) model \cite{dosovitskiy2020image}. In this adaptation, ViT transformed an image into a sequence of tokens by dividing it into patches and representing each patch as a single token. Further adaptation of transformers to videos operates by making spatiotemporal patches \cite{arnab2021vivit}. Following the success of ViT, there is a surge of research in the computer vision community for various image and video understanding tasks, largely outperforming the previously dominant ConvNet-based approaches, \eg \cite{selva2023video,ulhaq2022vision,tay2022efficient}.




Transformer models are constructed on self-attention and cross-attention mechanisms. Intuitively, self-attention is designed to capture the relationship among the different elements of the same sequence, while cross-attention is designed to capture the relationship among the elements of two different sequences. The transformer model follows a general encoder-decoder architecture. A transformer encoder uses self-attention and linear layers as building blocks. While, transformer decoder building blocks consist of self-attention, cross-attention and linear layers. Both the self-attention and cross-attention mechanisms use a multi-head attention mechanism. In the following, we provide a brief preliminary discussion on multi-head attention, self-attention and cross-attention. 


\begin{figure*}[ht]
  \includegraphics[width=0.96\textwidth]{Figures/transformer_fundamental/sha.png}
  \caption[Single Attention Head Mechanism]{Single Attention Head Mechanism. Single attention head with query, $\mathsf{Q}$, key, $\mathsf{K}$, and value, $\mathsf{V}$. The $\mathsf{Q}$ and $\mathsf{K}$ (with their associated weights, $\mathsf{W}^q_h$, $\mathsf{W}^k_h$) are first used to produce attention affinity matrix, $\mathsf{A}$ and then the output, $\mathsf{O}$, is computed from the attention affinity matrix and value sequence. The colours in the sequences represent different tokens and the colours in the attention affinity matrix represent the different attention affinity scores between different pairs of tokens and do not correspond to any particular numerical values.}
  \label{fig:sha}
\end{figure*}


\begin{figure*}[ht]
  \includegraphics[width=0.96\textwidth]{Figures/transformer_fundamental/mha.png}
  \caption[Multi-head Attention Mechanism]{Multi-head Attention Mechanism. Multi-head attention using $H$ attention heads is shown. The query, key and value are projected to each head, $\mathcal{A}_1, ..., \mathcal{A}_H$, and then outputs, $\mathsf{O}_1, ..., \mathsf{O}_H$, from these heads are concatenated and projected using output weights, $\mathsf{W^o}$, to produce final output, $\mathsf{O}$. The colours in the sequences represent different tokens and do not correspond to any particular numerical values.}
  \label{fig:mha}
\end{figure*}


\begin{figure*}[ht]
  \includegraphics[width=0.96\textwidth]{Figures/transformer_fundamental/self_attn.png}
  \caption[ Self-attention Mechanism]{Self-attention Mechanism. Self-attention mechanism explained in terms of multi-head attention, $\mathcal{M}$. The single input sequence $X$ is projected to produce query, $\mathsf{Q}$, key, $\mathsf{K}$, and value, $\mathsf{V}$, sequences for the multi-head attention to produce final output, $\mathsf{O}$. Position embeddings are not shown in favor of simplicity of visualization. The colours in the sequences represent different tokens and do not correspond to any numerical values.}
  \label{fig:self-attn}
\end{figure*}


\begin{figure*}[ht]
  \includegraphics[width=0.96\textwidth]{Figures/transformer_fundamental/cross_attn.png}
  \caption[Cross-attention Mechanism]{Cross-attention Mechanism. Cross-attention mechanism explained in terms of multi-head attention, $\mathcal{M}$. One input sequence, $\mathsf{X}$, is projected to produce query, $\mathsf{Q}$, while the other input, $\mathsf{Y}$, is projected to produce key, $\mathsf{K}$, and value, $\mathsf{V}$, sequences for the multi-head attention to produce final output, $\mathsf{O}$. Position embeddings are not shown in favor of simplicity of visualization. The colours in the sequences represent different tokens and do not correspond to any particular numerical values.}
  \label{fig:cross-attn}
\end{figure*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Sequences.}
Inputs to the attention function are represented as sequences. In this context, a sequence, often referred as a vector, is a list of tokens. A token is defined as a discrete unit of input with a numerical representation treated as a whole during processing. For example, a token can be a word, a sub-word or a character in language models and it can be a small spatial region or spatiotemporal volume in a vision transformer. Further details are discussed in \ref{sec:input_preprocessing}. For a single sequence, $X$, the sequence of $N$ tokens with $C$ features has the form $X^{N\times C}$. For batched data with $B$ elements in the batch, the token sequence has the form $X^{B\times N \times C}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Single-head attention.}
An attention function takes three sequences as input and produces a sequence as its output, $\mathsf{O}$. The three input sequences are called query, key and value. The terms query, key and value are used in analogy to their use in an information retrieval system, where data is retrieved based on an input ``query'', e.g., a text description, which is compared to a set of ``keys'', e.g., a set of video titles to produce ``values'', e.g., similarity scores, which are used to rank the videos with respect to the text. For transformers, the query, $\mathsf{Q}$, key, $\mathsf{K}$, and value, $\mathsf{V}$, are matrices whose rows are tokens. Single attention head, $\mathcal{A}_h$, then is defined in terms of query, key and value as 
\begin{equation}
   \hspace*{-0.2cm} \mathcal{A}_h(\mathsf{Q}, \mathsf{K}, \mathsf{V}) = \text{Softmax}\left(\frac{1}{\sqrt{d}}\mathsf{Q}\mathsf{W}^q_h(\mathsf{K}\mathsf{W}^k_h)^\top\right)\mathsf{V}\mathsf{W}^v_h,
    \label{eq:singlehead}
\end{equation} 
where $d$ is the feature dimension of $\mathsf{Q}$ and $\mathsf{K}$, while $\mathsf{W}^q_h, \mathsf{W}^k_h$ and $\mathsf{W}^v_h$ are the corresponding learned weight matrices for head $h$. Thus, $\mathsf{Q}\mathsf{W}^q_h(\mathsf{K}\mathsf{W}^k_h)^\top$ forms a matrix whose ${ij}^{th}$ element results from the inner product of row, $i$, of the (weighted) queries, $\mathsf{Q}$, and row, $j$, of the (weighted) keys, $\mathsf{K}$. Since by construction the rows of $\mathsf{Q}$ and $\mathsf{K}$ each correspond to a token, these operations systematically capture the relationships between the tokens, which subsequently are scaled and normalized by the token dimension, $d$, and the $\text{Softmax}$ to provide what is termed \textit{attention affinity}. In turn, the attention affinity is applied to the (weighted) values, $\mathsf{V}$, to capture its relationship and yield the final score. In short, an attention function first computes a global relationship score among all pairs of tokens in the input query and key sequences in the form of attention affinity and then incorporates the tokens from the value sequence to emphasize this global relationship. These operations result in a representation that captures relevance or relationship among the tokens in the input sequences. A visual depiction is shown in Figure~\ref{fig:sha}.

\paragraph{Multi-head attention.}
Multi-head attention uses multiple single-head attention mechanisms working in parallel and concatenates the outputs of all the heads. Thus, multi-head attention, $\mathcal{M}$, is defined  from~\ref{eq:singlehead} as
\begin{equation}
    \mathcal{M}(\mathsf{Q}, \mathsf{K}, \mathsf{V}) =
    \text{Concat}_{h=1}^{H} (\mathcal{A}_h(\mathsf{Q}, \mathsf{K}, \mathsf{V}))\mathsf{W}^o,
    \label{eq:multi-head}
\end{equation}
where $H$ is the number of attention heads in the multi-head attention and $\mathsf{W}^o$ is the weight matrix for the final multi-head output. By aggregating outputs from multiple attention head that operate on different projections of the inputs, the transformer model achieves increased representational capacity and enhanced generalization capability. As a result, the models can provide robust feature generation by capturing the diverse relationships among the tokens of input sequences. A pictorial depiction of the operations involved is shown in Figure~\ref{fig:mha}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Self-Attention.}
Self-attention, $\mathcal{S}$, is defined as an instance of attention with a single input, $\mathsf{X}$, and an optional positional embedding, $\mathsf{p}$. Commonly, it is instantiated in terms of multi-head attention~\eqref{eq:multi-head} as
\begin{equation}
    \mathcal{S}( \mathsf{X}, \mathsf{p})= \mathcal{M}(\mathsf{X}+\mathsf{p}, \mathsf{X}+\mathsf{p}, \mathsf{X}).
\end{equation} 
The positional embedding captures the position of tokens within a sequence~\cite{dosovitskiy2020image}. It is used as an additional input to the attention mechanism to introduce locality, since attention itself is a permutation invariant operation. Self-attention relates different positions of a single sequence to compute a representation that captures global or long range context within the sequence. A visual depiction is shown in Figure~\ref{fig:self-attn}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Cross-Attention}
Cross-attention, $\mathcal{C}$, is defined as an instance of attention with two inputs, $\mathsf{X,Y}$, and their corresponding positional embeddings, $\mathsf{p^X, p^Y}$. Commonly, it is instantiated in terms of multi-head attention~\eqref{eq:multi-head} as
\begin{equation}
    \mathcal{C}(\mathsf{X}, \mathsf{Y},
    \mathsf{p^X}, \mathsf{p}^{\mathsf{Y}})=\mathcal{M}(\mathsf{X} + \mathsf{p}^\mathsf{X},
    \mathsf{Y} + \mathsf{p}^\mathsf{Y},
    \mathsf{Y}).
\end{equation}
Hence, cross-attention is a four input operation used to mix or combine two different input sequences and their positional embeddings into a single output. Here, one input serves as query and another input is used as both key and value. In this way, cross-attention allows a combination of information from two different modalities. A visual depiction is shown in Figure~\ref{fig:cross-attn}.



\section{Summary of related surveys}
Table~\ref{tab:related_surveys} provides a list of literature surveys that are complimentary to the current presentation.

 

\begin{table}[ht]%{r}{0.4\textwidth}
    \centering
    %\begin{adjustbox}{width=0.98\textwidth}
    \begin{tabularx}{7in}{|X|c|X|}
        \toprule
        Title & Year & Remarks \\    
        \midrule
        Video Transformers: A Survey~\cite{selva2023video} & 2023 & transformers for video classification \\ \hline 
        Vision Transformers for Action Recognition: A Survey~\cite{ulhaq2022vision} & 2022 & transformers for action recognition\\ \hline
        A Survey on Deep Learning Technique for Video Segmentation~\cite{wang2021survey} & 2021 & approaches on video objects and video semantic segmentation\\ \hline
        Multi-task learning for dense prediction tasks: A survey~\cite{vandenhende2021multi} & 2021 & multitask learning for segmentation \\ \hline
        A Survey on Neural Network Interpretability~\cite{zhang2021interpretability} & 2021 &neural network interpretability \\\hline 
        Efficient Transformers: A Survey~\cite{tay2022efficient} & 2020 & transformers efficiency, e.g., factorized attention etc. \\ \hline 
        Video object segmentation and tracking: A survey~\cite{yao2020video} & 2020 & segmentation and tracking \\ \hline 
        %\bottomrule
      \end{tabularx}
    %\end{adjustbox}
    \caption{Summary of literature surveys.}
    \label{tab:related_surveys}
\end{table}




\section{Outline}
This chapter has served to motivate and provide a broad overview of video segmentation, classical approaches and transformers. Chapter~\ref{CH2} will provide a detailed discussion of different categories of video segmentation and benchmark datasets. Chapter~\ref{CH3} will provide a component-wise review of application of transformers to video segmentation. That chapter also will present the level of performance achieved by these models on the video segmentation tasks itemized in Chapter~\ref{CH2}. Chapter~\ref{CH4} will provide a review of interpretability analysis of transformer models, with a special focus on video segmentation. Finally, Chapter \ref{CH5} will provide conclusions, including suggestions for future research directions.

==> BODY/ch02_tasks_back.tex <==
\section{Overview}\label{task_overview}
The primary goal of computer vision for an intelligent autonomous system is the perception or understanding of the surrounding world from captured images, both single images as well as multiple image images acquired across time and/or space. The inferred knowledge can be used by other sub-subsystems. This might include future prediction and path planning. Depending on the granularity of the perception, video understanding tasks can be broadly categorized into video level, frame level, and pixel-level inference as shown in Figure ~\ref{fig:task_granularity}. The pixel level inference can also be of two levels of granularity: bounding box and per-pixel inference. In this survey, our focus is on the family of video understanding tasks on pixel-level inference. 

\begin{figure}[ht]
    \centering
    \begin{minipage}{.95\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{Figures/ch02task/task_continuum.png}
    \end{minipage}
\caption{Video understanding tasks by granularity.}
\label{fig:task_granularity}
\end{figure}

Dense video understanding tasks are among the fundamental problems in computer vision with a wide range of applications, including robotics, autonomous driving, video editing, and human-computer interaction. The task of pixel-level inference is to group pixels in images or video frames based on a given qualitative criteria, such as an object, action, or text reference. While all dense video understanding tasks work on the pixel level, there is a large variety of problem formulations. The diversity comes from the different possibilities of output space and qualitative objectives, such as motion, semantics, instances, action, and activity of the objects. The video segmentation inference is again of two types: offline and online. In the offline setting, all the frames are available at once, while only the past frames are available to the model in online inference. 



We begin the survey here with a taxonomy of various types of video segmentation tasks with a particular focus on those that are the focus of the recent literature. In the following sections, we will discuss a brief taxonomy of the dense video perception tasks, enumerate current research trends, and summarize the most recently used datasets. More historical details on the datasets and approaches are available in~\cite{yao2020video, wang2021survey}. We organize this chapter as follows: Section ~\ref{sec:objseg} discusses object segmentation in videos; Section ~\ref{sec:actorseg} discusses actor-action segmentation; Section ~\ref{sec:sceneseg} discusses holistic scene segmentation; Section ~\ref{sec:mmseg} discusses multi-modal video object segmentation.






\section{Objects}\label{sec:objseg}
Object-based video segmentation aims to delineate groups of pixels in an image or video frames to object masks based on qualitative criteria about some object properties in the videos. Object-based segmentation approaches are mainly two types: video object segmentation (VOS) which only segments foreground objects, and video instance segmentation (VIS), which segments all object instances along with tracking across frames. Depending on the required level of prior information or active human interaction, video object segmentation can be of three types: automatic VOS, semi-automatic VOS, and interactive VOS. Below we discuss problem formulation and state-of-the-art on all these video object segmentation tasks. 



\subsection{Automatic video object segmentation}
Automatic Video Object Segmentation(AVOS), often called Primary Object Segmentation, is defined as grouping pixels into foreground object masks representing the primary object in a video sequence, where primary is distinguished as the object showing dominant motion across the frames~\cite{yao2020video,wang2021survey}. For this reason, AVOS often has been termed foreground/background segmentation since an object with key-motion properties in a video sequence is generally the foreground object. Since no prior information is available, this kind of segmentation is also called unsupervised VOS or zero-shot VOS. 

Dominant approaches to AVOS rely on optical flow as an additional input along with color images~\cite{zhou2020motion,ren2021reciprocal,siam2019video,jain2017fusionseg}. These models generally use a two-stream architecture for extracting appearance features from color images and motion features from optical flow. There are different feature-fusing approaches available in the literature to aggregate these features, e.g., the commonly used late fusion~\cite{jain2017fusionseg} vs. recently proposed multistage fusion~\cite{zhou2020motion}. Another family of approaches considers attention~\cite{wang2019zero,lu2019see} to capture recurring objects without requiring optical flow features in a video via simple mechanisms, e.g., co-attention.



\subsection{Semi-automatic video object segmentation}
Semi-automatic Video Object Segmentation is a mask-guided object segmentation where one or more annotated frames (commonly the first frame) are available as reference masks containing one or more objects as a query. The objective is to segment the query objects throughout the video. This task is also called semi-supervised VOS or one-shot VOS due to the availability of guidance or supervision. Recently a multi-modal extension to this type of video object segmentation has become popular in the computer vision community where the reference is text or audio. We present a discussion on that in Section~\ref{sec:mmseg}. 


In general, semi-supervised VOS approaches employs feature alignment or attention-guided mechanism to propagate the mask of query objects from the reference frame to the entire video sequence. Matching-based approaches learn to match features of the target frames with the reference frame~\cite{hu2018videomatch}. The matching also includes several previous frames in some approaches~\cite{oh2018fast, voigtlaender2019feelvos,yang2020collaborative,yang2021collaborative}. Another research direction leverages a memory network to remember an embedding of previous predictions and use a memory-guided attention mechanism to segment the current frame~\cite{lu2020video,oh2019video,seong2020kernelized}. Recent approaches also use attention-based approaches~\cite{duke2021sstvos,lin2019agss,yang2021associating} for semi-supervised VOS to propagate masks. To further improve the performance of challenging multi-object scenarios, recent approaches use an attention-guided decoder~\cite{lin2019agss}. Another line of research uses a long short-term transformer for constructing hierarchical matching and propagation~\cite{yang2021associating} to associate multiple targets into a high-dimensional embedding space for simultaneous multi-object segmentation.






\subsection{Interactive video object segmentation}
Interactive Video Object Segmentation (IVOS) is semi-automatic object segmentation where there is an interaction between the system and a human providing hints to the object to be segmented(e.g., scribbles)~\cite{nagaraja2015video,bai2009video, criminisi2010geodesic, zhong2012discontinuity,fan2015jumpcut }. This interaction happens in a loop with a series of interactions beginning with initial guidance followed by some feedback.  Other forms of interaction includes contours~\cite{lu2016coherent} and points~\cite{wang2017selective}.  IVOS allows for applications requiring high-quality segmentation at the trade-off of human supervision. This approach is also used to generate datasets for automatic or other semi-automatic video segmentation tasks.

Recent IVOS approaches typically work by following an interaction-propagation approach~\cite{heo2020interactive, miao2020memory, heo2021guided, cheng2021modular}. 
AT-Net~\cite{heo2020interactive} used an annotation network (A-Net) and a transfer network (T-Net) that alternate to generate the segmentation results. The A-Net first generates a segmentation result from user scribbles on a frame and then the T-Net propagates the segmentation result bidirectionally to the other frames by employing global and local transfer modules. Another approach, the Memory Aggregation Networks (MANet)~\cite{miao2020memory} used integrated interaction and the propagation model in a single network to improve efficiency.  They used an effective memory aggregation mechanism to record the informative knowledge from the previous interaction rounds. Another approach, GIS~\cite{heo2021guided} presented a reliability-based attention module and intersection-aware propagation module. Another approach, MiVOS~\cite{cheng2021modular} decouples the interaction-propagation as interaction-to-mask and mask propagation, where an interaction module converts user interactions to an object mask and then the mask is temporally propagated. For efficient temporal mask propagation a space-time memory model is employed with a novel top-k filtering strategy to read the memory.



\subsection{Video instance segmentation}
Video instance segmentation(VIS) aims at the simultaneous detection, segmentation, and tracking of instances in videos~\cite{yang2019video}. The problem is also referred to as multi-object tracking and segmentation(MOTS)~\cite{voigtlaender2019mots}. The related task, video object detection and tracking aims at detecting(bounding boxes)
and tracking objects, while video instance segmentation additionally generates pixel-wise object segmentation masks. Again, in contrast to instance segmentation in images which involves detection and segmentation~\cite{hariharan2014simultaneous}, the requirement of tracking object instance masks across video frames makes it more challenging.  In short, VIS simultaneously predicts object bounding boxes and object masks where the bounding boxes are labeled with semantic categories and segmentation masks are based on object identities across frames. The tracking of object masks makes it especially relevant for the application of video editing, autonomous driving, and augmented reality~\cite{yang2019video}. 


Recent dominant approaches for VIS follow a simultaneous segmentation and tracking approach~\cite{wang2021end,hwang2021video,wu2022seqformer} using transformer-based attention mechanisms. VisSTG~\cite{wangtao2021gnn} proposed an end-to-end approach to simultaneously learn classification, detection, segmentation, and tracking using a graph neural network-based approach. The approach used Graph Neural Network (GNN) to model the instance-level relations in both intra- and inter-frame levels in a unified model. The graph nodes encode instance features for detection and segmentation, and the edge features represent the instance relations for tracking. Another approach, VisTR~\cite{wang2021end} used a transformer-based encoder-decoder approach followed by multiple task-heads for detection, segmentation, and matching-based tracking to work on an entire video sequence in a single inference. This formulation allows for a simple yet efficient video instance segmentation model. Another approach, Inter-frame Communication Transformers (IFC)~\cite{hwang2021video} uses a concise memory token representation as an efficient encoding of the clip context. The inter-frame tracking is achieved via an exchange of information between these memory tokens. Another approach, CrossVIS~\cite{yang2021crossover} used a crossover learning scheme for online VIS. This approach localizes an instance in other frames from the instance feature from the current frame. This approach also used an additional branch called global balanced instance embedding for a stable online instance association. SeqFormer~\cite{wu2022seqformer} used deformable attention~\cite{zhu2020deformable} in the decoder to first locate the object bounding boxes queries in each frame and then aggregated to the instance queries to predict dynamic mask head parameters. The tracking is achieved by convolving the encoded feature maps by using a mask head. TeViT~\cite{yang2022temporally} uses an efficient message passing based frame-level temporal context and query-based instance-level temporal context to achieve strong temporal consistent modeling capacity on the VIS task. 



\subsection{Benchmark datasets}
Below we present a brief discussion on the large-scale video object segmentation benchmark datasets that are commonly used in recent literature. 

\paragraph{YouTube-Objects.} The YouTube-Objects~\cite{prest2012learning} dataset 
contains a total of 155 web videos collected from YouTube. There are objects of 10 semantic classes and each class has nine to 24 videos of duration between 30 seconds and three minutes at resolution 720p. These videos are split into 1,407 clips containing around a total of 570,000 frames. For video object segmentation, a subset of this dataset is used which has 126 shots with 20,647 covering all of the 10 semantic classes. This subset provides pixel-level foreground-background annotations on every $10^{th}$ frame~\cite{jain2014supervoxel}.

This subset is used to validate the generalization ability of automatic video object segmentation models. For this purpose, model trained on other datasets are validated on the pixel-level annotated subset of the YouTube-Objects dataset. As for evaluation metric, region similarity( intersection-over-union a.k.a. Jaccard index~\cite{shi2014jaccard}) is used. The region similarity is defined as the ratio of the intersection area to the union area of the prediction and ground truth. For this reason, this is often termed as Intersection over Union (IoU). This dataset initially computes the mean of IoU over all clips in each categories and then over all categories which is referred as mean IoU or mIoU.   



\paragraph{DAVIS 2016.}
The Densely Annotated VIdeo
Segmentation(DAVIS) 2016~\cite{perazzi2016benchmark} dataset is an automatic foreground-background segmentation dataset containing 50 high-quality video sequences with a total number of 3455 annotated frames. There are 30 videos for training and 20 for testing. The videos cover multiple occurrences of common video object segmentation challenges, such as occlusions, motion blur, and appearance changes. The video sequences contain a single object or two spatially connected objects annotated in each frame as the primary  foreground object with a distinctive motion. There are also video-level attributes describing challenges present in the sequence, such as occlusions, fast-motion, non-linear deformation and motion-blur to enable a deeper understanding of the results of algorithms on this dataset.  


The DAVIS 2016 dataset proposed three complementary metrics to evaluate the performance of video object segmentation models. These metrics measure the spatial accuracy of the segmentation, the quality of the silhouette, and the temporal coherence. Spatial accuracy is measured using region similarity(a.k.a. intersection-over-union or Jaccard index), like other VOS datasets. They proposed to measure the quality of the silhouette using contour accuracy. To compute contour accuracy, the segmentation mask is considered as a set of closed contours, then the F-measure~\cite{chen2004statistical} is calculated from the contour based precision and recall between the segmentation mask and the ground truth. They proposed to measure the temporal stability between the polygon representation of the contours of the segmented masks of adjacent frames. For this purpose, polygon representation of the contours of adjacent frames are matched using dynamic time warping to minimize shape context descriptor (SCD)~\cite{belongie2002shape} distance. The temporal stability is calculated as the mean cost per matched point.



\paragraph{DAVIS 2017.} The DAVIS 2017~\cite{pont20172017,caelles20182018} dataset provides annotations for automatic video object segmentation, semi-supervised video object segmentation, and interactive video object segmentation. The DAVIS 2016 dataset was extended by adding more videos, annotations for multiple objects instances and semi-automatic video object segmentation(semi-supervised and interactive). There are 150 video sequences in total in this dataset. These are divided into train, validation, test-development, and test-challenge splits with 60, 30, 30, and 30 videos. The total number of annotated frames is 10,549 containing 376 objects. In addition to the distinctive motion of DAVIS 2016, the granularity of instances are defined by their semantics. As an example, people and animals are together segmented as a single foreground instance in DAVIS 2016. And in DAVIS 2017 they are two foreground object instance. Compared to DAVIS 2016, DAVIS 2017 contains additional challenges arising from more distractors, smaller objects, finer structures, more occlusions and faster motions.


To benchmark approaches for unsupervised video object segmentation, the metrics from DAVIS'16 are adopted. To evaluate algorithms for the semi-supervised video object segmentation task, this dataset adopted the region similarity(IoU) and boundary accuracy(F-measure) measures from the DAVIS'16 dataset (temporal stability is no longer considered). \textcolor{red}{The benchmark is to compute each metric per each object instance on each clip and take average over all instance on the entire test set . The overall performance metric for ranking in the challenge~\cite{pont20172017} is defined as the average of the two metrics.}


To evaluate interactive video object segmentation, they used a test server to simulate human inputs, and participants are needed to connect to the server to receive the scribbles. There are a maximum of eight interactions to iteratively refine the interactive segmentation result. To benchmark the algorithms, first the region similarity~\cite{caelles20182018} or the mean of region similarity and contour accuracy~\cite{caelles20192019} is plotted against the interaction time and then the Area Under the Curve (AUC) of the plot is computed.



\paragraph{YouTube-VOS.} 
The YouTube Video Object Segmentation dataset (YouTube-VOS)~\cite{xu2018youtube}
 is a large-scale benchmark for video object segmentation. The dataset contains 3,252 YouTube video clips divided into training (2,796), validation (134), and test (322) sets. The test set is further split into test-seen and test-unseen subsets to evaluate the generalization ability of segmentation models on unseen categories. They provide annotations for 94 object categories including common objects and human activities. To benchmark on this dataset, they adopted the region similarity and the contour accuracy, following ~\cite{perazzi2016benchmark}.
 

\paragraph{YouTube-VIS.} The YouTube-VIS~\cite{yang2019video} is a video instance segmentation dataset with a subset of sequences from YouTube-VOS and instance-level annotation. The dataset contains 2,883 high-resolution YouTube videos providing annotations for 131,000 high-quality instance masks covering 40 object categories selected from the YouTube-VOS~\cite{xu2018youtube}.

The benchmark metrics are adopted from the Average Precision (AP) and Average Recall (AR) metric used in image segmentation with the extension of a different region similarity(IoU) measure to account for tracking~\cite{yang2019video}. These metrics are first evaluated per category and then averaged over the category set. The AP is defined as the area under the precision-recall curve of the confidence score. Following the COCO benchmark, AP is averaged over multiple intersection-over-union (IoU) thresholds from $50\%$ to $95\%$ at step $5\%$. The maximum recall at some given fixed number of segmented instances per video is used as AR. 


\paragraph{MoCA.} The Moving Camouflaged 
Animals(MoCA)~\cite{lamdouar2020betrayed} is an especially challenging video object segmentation dataset containing camouflaged animals. Notably, in many cases the camouflage is so strong that the target animal is indistiguishable from the background in a single frame; however, it is revealed in the motion exhibited across frames. The dataset contains 141 video sequences collected from YouTube depicting various camouflaged animals(67 categories) moving in natural scenes. The annotation provides a bounding box in each frame, as well as a motion label. The motion level can be one of locomotion, deformation, or static. 

The evaluation protocol for segmentation in this dataset computes IOU between the ground truth box and the minimum box that includes the predicted segmentation mask. In addition, the evaluation protocol in MoCA includes success rate at various thresholds. The evaluation in this dataset includes only the segmentation of the animals under locomotion or deformation and excludes static frames.



\paragraph{OVIS.} The Occluded Video Instance Segmentation (OVIS)~\cite{qi2022occluded} is a large-scale video instance segmentation dataset consisting of very challenging scenarios of objects under various levels of occlusion. There are 901 videos with conditions of severe object occlusions covering 5,223 unique instances from 25 semantic categories.

To evaluate video instance segmentation, this dataset used Average Precision (AP) at different Intersection-over-Union (IoU) thresholds and Average Recall (AR), similar to YouTube-VIS~\cite{yang2019video}. In addition, to evaluate algorithms at various levels of occluded conditions, the dataset proposed to compute AP under different occlusion degrees. To facilitate this evaluation, they included occlusion level information of each object in the annotation.



\paragraph{MOSE.} coMplex video Object
SEgmentation (MOSE)~\cite{ding2023mose} is a large scale video object segmentation dataset designed for semi-supervised vos under crowded and occluded scenarios. The dataset contains 2,149 video clips and 5,200 objects from 36 categories. The target objects in most of the videos are commonly occluded by other objects and disappear in some frames. Following ~\cite{perazzi2016benchmark, pont20172017}, they used region similarity(IoU) and contour accuracy(F-measure) as the evaluation metric for this dataset.


\section{Actor and Actions}\label{sec:actorseg}
\subsection{Actor-Actions Segmentation}
Actor-action semantic segmentation is defined as delineating regions from a given video with corresponding label of an actor-action tuple~\cite{xu2015can}. Actors are objects that are participants in some actions. This task has been investigated far less intensively than object segmentation. Due to the exclusiveness of certain actor-action tuples, jointly segmenting actor-action has been found to result in better modeling than independently segmenting them in the context of action recognition. As an example, a car can not eat and a cat can not fly. The exclusiveness of these actor-action tuple helps it less likely for the model to learn to predict these tuples. On the other hand, in independent inference of actor and action can predict car as actor and climb as action without reasoning the exclusiveness of the tuple. This is evident from the quantitative experiments presented in~\cite{xu2015can}. 

Trending research on actor-action segmentation typically uses optical flow as an extra input along with raw frames localize object motion as a probable actor. Typical approaches include 2D or 3D ConvNets as feature backbones. Some approaches formulate the model as simultaneous multi-task learning~\cite{ji2018end} by adding multiple branches of task heads on top of a feature backbone. Specifically, they use separate prediction branches for mask segmentation, actor classification, and action classification on top of fused features from RGB frames and optical flow inputs. Other notable approaches~\cite {dang2018actor} include using a region of interest-based approach with region masks from an instance segmentation algorithm followed by non-maximum suppression and a classification head. Recently, SSA2D proposed~\cite{rana2021we} a simple yet effective proposal-free model using 3D convolutions to perform pixel-level joint actor-action detection in a single shot.  



\subsection{Benchmark Datasets}

\paragraph{A2D.} The A2D~\cite{xu2015can} dataset provides actor-action segmentation with annotation for seven actor classes (adult, baby, ball, bird, car, cat, and dog), eight action classes (climb, crawl, eat, fly, jump, roll, run, and walk),  and the no-action class. This dataset facilitates three specific problems including actor-action recognition with single-label, multiple-label, and actor-action semantic segmentation. The A2D dataset has 3782 unconstrained “in-the-wild” videos with varying characteristics collected from YouTube and provides pixel-level annotations. There are 43 valid actor-action tuples with at least 99 instances per tuple for joint actor-action segmentation tasks. The training split has 3036 videos and test split has 746 videos divided evenly over all actor-action tuples. They provided both the pixel level and bounding box annotation per actor-action pair.

The evaluation of actor-action semantic segmentation in this dataset includes global pixel accuracy, mean per-class accuracy, and mean pixel Intersection-over-Union (mIoU) for both separate actor, action segmentation, and joint actor-action segmentation, following prior work~\cite{xu2016actor}. The global pixel accuracy measures the overall percent of pixels with correct label prediction. The mean per-class accuracy measures the percent of pixel level accuracy first per class and then averaged across classes. The mean pixel Intersection-over-Union (mIoU) evaluates the region similarity using Intersection over Union (IoU) aggregated similarly to per-class accuracy. This is also considered in recent work as the most representative metric for correct pixel prediction over all classes~\cite{rana2021we}.    



%\paragraph{Metrics}
%\paragraph{State of the Art}


\section{Scenes}\label{sec:sceneseg}
Scene segmentation aims to segment all the pixels in the scene with labels that assign them to a particular category or instance of a category. In this context, scene categories are defined either as "things" or "stuff"~\cite{lin2014microsoft}. In general, "things" are countable objects that typically have a well defined shape, wheras "stuff" is an uncountable entity with shape typically not being a defining attribute. As examples: People and cars are countable objects, with shape being an important attribute; in contrast, sky and forest are not countable and shape is not important in their definition. Scene segmentation also is referred as scene parsing in some contexts since it aims to parse all the contents of a scene to categories or instances. Both video semantic segmentation and video panoptic segmentation aim to label all the pixels in a scene including both things and stuff. The difference is that semantic segmentation does not consider instances, while panoptic segmentation does.



\subsection{Video Semantic Segmentation}
Video semantic segmentation(VSS), also referred as video scene parsing(VSP)~\cite{yan2020video}, aims at labelling all the pixels in a scene into semantic categories of things and stuff classes, and to do so in an instance agnostic fashion~\cite{wang2021survey}. Similar to VOS, VSS also can be automatic or semi-automatic. Automatic VSS segments all the frames without using any key-frame, while semi-automatic VSS uses key-frames to segment other frames. Due to the ability of VSS to describe the high-level semantics of the physical environment, it can serve as upstream perception for many application of autonomous systems , e.g., autonomous driving, robot navigation, and human-machine interaction.  

Most common approaches in VSS follow propagation based  segmentation from a key-frame(semi-automatic) or some previous frames(automatic) to other frames. Typically, these approaches rely on optical flow based warping to propagate their labels~\cite{gadde2017semantic,liu2017surveillance,ding2020every,jain2019accel}. Recent trending research uses inter-frame feature correlation~\cite{zhuang2020video} or inter-frame attention~\cite{paul2020efficient,wang2021temporal,li2021video} to capture the temporal relations across consecutive frames without depending on optical flow. For example, Temporal Memory Attention Network (TMANet)~\cite{wang2021temporal} adaptively integrates the long-range temporal relations over a video sequence with a temporal memory attention module to capture the relation between the current frame and a memory generated from several past frames. Similar efforts propose a fast local attention mechanisms to allow semantics from recent frames, as encoded in a memory module, to attend to  the current frame~\cite{paul2021local,hu2020real} . To further address efficiency, Sparse Temporal Transformer (STT)~\cite{li2021video} used a sparse inter-frame cross-attention based on a query and key selection strategy to reduce the time complexity of attentional processing. As yet another approach, Coarse-to-Fine Feature Mining (CFFM)~\cite{sun2022coarse} used inter-frame cross-attention with coarse features on past frames for efficient cross-attention mechanism. 




\subsection{Video Panoptic Segmentation}
Panoptic segmentation of images was first proposed as a holistic segmentation of all foreground instances and background regions in a scene~\cite{kirillov2019panoptic} which was later extended for videos~\cite{kim2020video}. Video Panoptic Segmentation(VPS) unifies video instance segmentation for things classes and video semantic segmentation for stuff classes~\cite{kim2020video}. The difference between VPS with VSS is that in VSS things are segmented into semantic categories without tracking instances. Here, it also is worth noting that the difference between VPS and VIS is that the latter considers all stuff classes simply as background, while VPS distinguishes different classes of stuff. So, this is an instance-aware semantic segmentation with tracking of object IDs. Overall, VPS jointly predicts object classes, bounding boxes, masks, instance ID tracking, and semantic segmentation in video frames. 

Recent efforts on VPS use multiple branches of task heads for detection, segmentation, and tracking. The Video Panoptic Segmentation Network (VPSNet)~\cite{richter2017playing} initially aggregates warped features of past frames to the current frame, performs spatiotemporal attention followed by multi-task branches and then explicitly models cross-frame instance association specifically for tracking. Another approach, AES~\cite{woo2021learning} proposed to jointly learn coarse segment-level matching and fine pixel-level matching for dense temporal associations using a supervised contrastive learning approach. Another unified multitask mode, TubeFormer-DeepLab~\cite{kim2022tubeformer} presented a mask transformer-based approach to partitioning video a video clip into class-labeled tubes providing a general solution to Video Semantic Segmentation (VSS), Video Instance Segmentation (VIS), and Video Panoptic Segmentation (VPS). Yet another approach, Slot-VPS~\cite{zhou2022slot} proposed an end-to-end framework with an object-centric representation learning approach for video panoptic segmentation. They presented to encode all panoptic entities in a video with a unified representation called panoptic slots that capture their visual appearance and spatial information across time. They used a Video Panoptic Retriever to retrieve and encode coherent spatiotemporal object’s information into the panoptic slots.  The retriever is a three-stage pipeline that includes slot assignment, slot prediction, and slot refinement. Finally, they used three prediction heads to produce classification, mask, and object ID from the panoptic slots.



 
\subsection{Depth-aware Video Panoptic Segmentation} 
The Depth-aware Video Panoptic Segmentation (DVPS) is defined as an inverse projection problem to restore the point clouds from a video and simultaneously provide each point with instance-level semantic interpretations~\cite{qiao2021vip}. This task also can be considered as an extension to VPS that aims to jointly predict panoptic segmentation and depth in a video.  


Recent efforts on DVPS mostly extended non-depth aware panoptic segmentation approaches with an extra depth estimation head. A notable approach, ViP-DeepLab~\cite{qiao2021vip} was the first proposed unified model for DVPS that used an additional prediction head for monocular depth estimation. Another following approach, TubeFormer-DeepLab~\cite{kim2022tubeformer} proposed a unified model to combine multiple video segmentation in a single model which also extends to DVPS. They begin with partitioning a video clip into tubes with class prediction and tube embedding vector pairs which are later used to generate a tube prediction. For this purpose, they used a hierarchical structure with two types of dual-path transformer blocks with message passing between video features and a latent memory or a global memory. Yet another recent approach, PolyphonicFormer~\cite{yuan2022polyphonicformer} proposed a transformer-based query learning approach for DVPS that unifies both panoptic segmentation and depth estimation tasks. This unified modeling enables the interaction between panoptic context and depth information allowing them both to benefit from each other. Overall, the model has three components. First, a feature extractor generates features for panoptic segmentation and depth estimation. Second, a polyphonic head learns the queries for these tasks. Third, a tracking head is used to learn the feature embedding among the frames.  




\subsection{Panoramic Video Panoptic Segmentation} 
The \textbf{P}anoramic \textbf{V}ideo \textbf{P}anoptic \textbf{S}egmentation (PVPS) extends the VPS to panoramic videos generated simultaneously from multiple cameras. In addition to the multi-view setting, this task has another added challenge of tracking instance ID across multiple cameras at each time. PVPS is an important requirement for autonomous driving, where there are multiple cameras on the vehicle to capture videos of the surrounding environment. 

Currently, the single documented approach to this task worked by augmenting  ViP-DeepLab video panoptic segmentation algorithm~\cite{qiao2021vip} to accept multi-camera input~\cite{mei2022waymo}. For this purpose, this approach trains separate models for each camera view and an additional model on a panorama generated from all views. To track instance IDs across camera views, this approach follows a similar method used in ViP-DeepLab to track instance IDs across time. This instance ID tracking method is based on comparing IoU between region pairs ,e.g., two mask with high IoU overlap are re-assigned with same instance ID. 





\subsection{Benchmark Dataset}

\paragraph{VISPW.} Video Scene Parsing in the Wild (VSPW)~\cite{miao2021vspw} is a large-scale video semantic segmentation dataset containing 3,536 videos each around five seconds long. The dataset provides pixel-level annotations for 124 categories at 15 frames-per-second. There are 2,806 videos in the training split, 343 videos in the validation split, and 387 videos in the test split. The dataset covers a wide range of real-world scenarious, including both indoor and outdoor environments. The annotations are provided for both things and stuff classes. 

The evaluation metric for this dataset includes mean IoU, weighted IoU, and Temporal Consistency (TC). The mean IoU is the region similarity measure using intersection-over-union between the predicted and ground truth pixels averaged over all the classes. The weighted IoU also calculates the region similarity but is weighted by the total pixel ratio of each class. The Temporal Consistency (TC) is computed as the intersection-over-union between the predicted mask of frame t and the warped predicted mask from frame t-1 to frame t.  Optical flow-based warping is used for this purpose. 


\paragraph{VIPSeg.} \textbf{VI}deo \textbf{P}anoptic \textbf{Seg}mentation
in the Wild (VIPSeg)~\cite{miao2022large} is a large-scale video panoptic segmentation dataset that aims to assign semantic classes and track identities for all pixels in a video. The dataset contains 3,536 videos of 3-10 seconds duration sampled at 6 frames-per-second. There are total of 84,750 pixel-wise annotated frames that only focus on street view scenes. There are total of 232 scenarios with 124 categories, including 58 thing classes and
66 stuff classes.

The evaluation metric for this dataset are Video Panoptic Quality (VPQ) as well as Segmentation and Tracking Quality (STQ). VPQ is extended for videos from Panoptic Quality(PQ) used in panoptic image segmentation. VPQ computes the average quality  using tube IoU matching across a small span of frames. STQ is the geometric mean of Association Quality(AQ) and Segmentation Quality (SQ) that evaluates instance agnostic segmentation quality using semantic classes. Here AQ is a measure of the pixel-level association across an entire video and SQ is a measure of semantic segmentation quality by class-level IoU. 



\paragraph{VIPER.} The VIPER dataset~\cite{richter2017playing} is a synthetic dataset collected from the GTA-V video game~\cite{richter2016playing} and supports for video semantic segmentation, video instance segmentation, and video panoptic segmentation. The dataset was originally proposed for video semantic segmentation and video instance segmentation. Subsequently, it was extended by adding COCO-style metadata to support for video panoptic segmentation~\cite{kim2020video}. The dataset contains $1080\times 1920$ resolution ego-centric scenes of driving, riding, and walking a total of 184 kilometers in diverse ambient conditions in a realistic virtual world. There are 254k annotated frames with 10 things classes and 13 stuff classes. The evaluation metric for this dataset is Video Panoptic Quality (VPQ), as with VIPSeg~\cite{miao2022large}. 



\paragraph{Cityscapes-VPS.} The Cityscapes-VPS~\cite{kim2020video} dataset is developed for video panoptic segmentation by extending the annotations in the popular image panoptic segmentation dataset Cityscapes~\cite{cordts2016cityscapes}. Provided are pixel-level panoptic annotations for 3000 frames at $1024\times 2048$ resolution with 19 classes, and temporally consistent instance IDs to thing objects within videos. The Cityscapes-VPS also uses video panoptic quality (VPQ) metric as an evaluation measure.


 \paragraph{Cityscapes-DVPS.} ViP-DeepLab~\cite{qiao2021vip} designed the Cityscapes-DVPS dataset by adding depth annotation to the Cityscapes-VPS~\cite{kim2020video}. A new evaluation metric for DVPS named Depth aware Video Panoptic Quality (DVPQ) is introduced for this dataset extending VPQ by additionally considering the depth prediction. Two parameters, $k$ and $\lambda$ is used with DVPQ to define $DVPQ^k_\lambda$ for this purpose. Here $\lambda$ is used to refer to the threshold of relative depth error used for calculating VPQ. And $k$ is used to refer to the number of frames in the video clip is used to calculate the VPQ. Specifically, they used three different values of $\lambda$ ,e.g., $(0.10,0.25,0.50)$ and four different values of $k$ ,e.g., $1,2,3,4$. The $DVPQ^k_\lambda$ is calculated for things and stuff classes separately and jointly.   


 
\paragraph{SemKITTI-DVPS.} SemKITTI-DVPS~\cite{qiao2021vip} extends the SemanticKITTI dataset~\cite{behley2019semantickitti} by adding depth annotation. The dataset consists total 22 sequences of which 11 are for training and 11 are for testing. One of the training sequences is used for validation. The original dataset has perspective images and panoptic-labeled 3D point clouds with annotation for 8 things and 11 stuff  classes. The dataset is converted for DVPS by projecting the 3D point clouds into the image plane followed by some additional post-processing to remove sampled points that exhibit large relative errors due to sensor alignment issues. Similar to Cityscapes-DVPS, $DVPQ^k_\lambda$ is used as the benchmark metric for the SemanticKITTI-DVPS dataset. 




\paragraph{WOD-PVPS.} The \textbf{W}aymo \textbf{O}pen \textbf{D}ataset: \textbf{P}anoramic \textbf{V}ideo \textbf{P}anoptic \textbf{S}egmentation 
 (WOD-PVPS)~\cite{mei2022waymo} is a very large scale panoramic video panoptic segmentation dataset of driving scenarios. The dataset contains 2,860 temporal
sequences of driving scenarios in three different geographical locations, as captured by five cameras mounted on autonomous vehicles. They provide annotations consistent over time and across multiple  cameras views to facilitate full panoramic scene understanding. Overall, there are total of 100,000 labeled camera images with 28 semantic categories. 

The PVPS evaluation metric for this dataset is weighted Segmentation and Tracking Quality(wSTQ) adopted from the Segmentation and Tracking Quality(STQ) metric for VPS. In particular, they weight each pixel by the camera coverage fraction before calculating association quality and segmentation quality. Camera coverage fraction for a pixel is calculated as the ratio of the number of cameras where that pixel is present to the total number of cameras.

\section{Multimodal Video Segmentation}\label{sec:mmseg}
Multimodal Video Object Segmentation, often termed as Referring Expression Object Segmentation uses input query in another mode (e.g., text or audio) to indicate the segmentation target. This formulation is similar to semi-supervised VOS, where reference is given as a mask annotation on the first frame. In contrast, in multimodal video segmentation, reference to the object is given by text or audio. State-of-the-art solutions to referring video object segmentation learn the multi-modal representation using an interaction network layer and then employ this representation to guide the segmentation mask generation.

\subsection{Text-Guided Video Object Segmentation}
Text-Guided video object segmentation is defined as automatically separating foreground objects from the background in a video sequence based on referring text expressions. Since this is the most common referring video objects segmentation, this problem is widely known as referring video object segmentation(RVOS). There are two types of annotations used for text-guided video object segmentation. The first is based on reference to an object description based on the first frame, which is very similar to semi-supervised VOS except the reference is text. This kind of reference text mostly describes the object appearance, e.g., 'A man wearing a white cap'. The second type of referring text expression is based on the full video clip and also includes temporal dynamics of the object in the referring expression, e.g., 'A person showing his skateboard skills on the road'.   

Early efforts on RVOS generally follow a two stage pipeline: First, a referring bounding box is tracked across a video; second, the box is segmented to indicate the object of interest on a pixel-wise basis~\cite{khoreva2018video}. Another notable approach, URVOS~\cite{seo2020urvos} presented an efficient and unified model to initially segment some masks guided by the referring expressions, followed by a propagation based semi-supervised VOS to produce the final results. Yet another approach, YOFO~\cite{li2022you} presented a multiscale cross-modal feature mining structure and an augmented memory based meta-transfer mechanism that learns target specific features. Recently, transformer based model has been proposed for RVOS that uses an encoder-decoder architecture. A recently proposed transformer based approach, Multimodal Tracking Transformer (MTTR)~\cite{botach2022end} initially extracts features from the text and video for subsequent concatenated multimodal feature sequences. Then, a  multimodal transformer encoder is used as feature relation encoder followed by a transformer decoder to decode instance-level queries. Finally, corresponding mask and reference labels are generated. Another transformer based approach, ReferFormer~\cite{wu2022language} presented a simple and unified end-to-end transformer based framework that uses object queries conditioned on language expressions. Overall, the model has four components. First, a backbone feature extractor with a visual encoder and a text encoder that are used to extract visual features and text features. Second, a transformer encoder-decoder is applied: The encoder operates on the visual features to encode their relations; the decoder uses both visual and text features to generate shared object queries that are transformed into dynamic kernels. Third, high resolution visual features are generated by a cross-modal feature pyramid network~\cite{ghiasi2019fpn} that facilitates for multi-scale vision-language fusion. Fourth, the segmentation component uses the dynamic kernels from the transformer decoder as convolution kernels to extract the segmentation masks from the high resolution feature maps. The tracking of objects across frames is achieved by linking the object queries across frames. 



\subsection{Audio-Guided Video Object Segmentation}
Audio-Guided Video Object Segmentation (AGVOS) is defined as automatically separating foreground objects from the background in a video sequence based on referring audio expressions~\cite{pan2022wnet}. \textcolor{red}{It is to note that the authors of ~\cite{pan2022wnet} referred this as AVOS, while we use AGVOS to avoid confusion with automatic VOS.} The motivation for audio-guided VOS is that audio often contains additional information compared to text e.g., the accent, emotion and speed.

Currently, it appears that there is only a single effort that has considered audio-guided VOS. In particular, Wnet~\cite{pan2022wnet} used a cross-modal denoising network to clean the audio signal and a wavelet-based encoder network to learn the cross-modal representations of the target video and query audio.
Overall, the model is composed of five modules: visual encoder, audio encoder, transformer encoder, transformer decoder and segmentation module. The visual encoder is a ConvNet which is used to extract features from the input video clip. The audio encoder uses a pretrained acoustic feature extractor network ~\cite{bouchakour2018mfccs}, followed by convolution. 

Following feature extraction, a transformer encoder is used to encode the cross-modal features. Here, a wavelet based cross-modal module is used to fuse the multi-modal features in a de-noised joint representation. Next, a transformer decoder is used to learn object instance queries. Finally, the queries are used together with the cross-modal features to segment instances with a segmentation head. 




\subsection{Benchmark Datasets}
\paragraph{A2D Sentence~\cite{gavrilyuk2018actor}.} This dataset is designed for pixel-level segmentation of actors and their actions in videos from a natural language query sentence. %This problem formulation distinguish between fine-grained actors in the same super-category, identify actor and action instances, and segment pairs that are outside of the actor and action vocabulary. 
This dataset extended actor and action datasets A2D~\cite{xu2015can} natural language descriptions. The natural language description contain information about what each actor is doing in the videos. An example of a referring expression is 'red ball is rolling on a bowling floor'. There are 3,036 training videos and 746 testing videos.

The standard evaluation protocol in A2D-sentence includes overall IoU, mean IoU,  precision at 5 different intersections from 0.5 to 0.9, and the mean average precision at intersection over thresholds from 0.50 to 0.95 at interval of 0.05. The overall IoU is the ratio of total intersection area of all test data and the total union area. Since this measure of overall IoU over the whole test data favors large segmented regions, the mean IoU is also used as an additional metric to treat large and small regions equally. The precision at threshold K also called Precision@K is the percentage of test samples with IoU above the threshold K.

\paragraph{J-HMDB Sentence~\cite{gavrilyuk2018actor}.} This dataset is designed with extending J-HMDB dataset~\cite{jhuang2013towards} by adding natural language expression describing various actions. There are s 928 video clips of 21 different actions in J-HMDB dataset. The annotations are available with a 2D articulated human puppet that provides scale, pose, segmentation and a coarse viewpoint
for the humans involved in each action. The added natural language description contains information about what the target object is doing in each video. An example text expression is 'boy in gray shirt and black shorts swinging baseball'. The evaluation protocol for this dataset is same as in A2D Sentence~\cite{gavrilyuk2018actor}. 


\paragraph{Ref-DAVIS.}  Referring Expressions for DAVIS 2016 and 2017 (Ref-DAVIS)~\cite{khoreva2019video} is an extension of the DAVIS 2016 and DAVIS 2017 datasets by adding referring text expressions. The referring expression is generated to describe the object in the first frame mask of the semi-supervised setting. All objects annotated with mask labels in DAVIS16 and DAVIS17 are augmented with non-ambiguous referring expressions. Overall, the augmented DAVIS16/17 dataset contains over a thousand referring expressions for more than 400 objects on 150 videos with approximately 10,000 frames. The evaluation metrics for this dataset are region similarity, contour accuracy, and their average value. 


\paragraph{Ref-YouTube-VOS.} Refer-YouTube-VOS, also known as RVOS~\cite{seo2020urvos}, is a large scale referring video object segmentation dataset with referring expressions added to the Youtube-VOS~\cite{xu2018youtube} dataset. The dataset provided two kinds of annotations to describe the highlighted object: full-video expression and  first-frame expression. The evaluation metric for this dataset is similar to Ref-DAVIS, i.e., region similarity, contour accuracy, and their average. 


\paragraph{Audio-Guided-VOS Dataset (AGVOS).} The AGVOS~\cite{pan2022wnet} is a large-scale audio-guided VOS dataset developed by extending the Refer-YouTube-VOS~\cite{seo2020urvos}, A2D~\cite{xu2015can} and J-HMDB~\cite{jhuang2013towards} datasets. \textcolor{red}{Originally, the author used acronym AVOS for this dataset. Here we use acronym AGVOS for Audio-Guided-VOS Dataset to avoid confusion with automatic VOS.} They employed 36 speakers to generate the audio by reading provided sentences. The sampling rate is 44,100K or above, the sampling number is 16 bits, and the speaking speed is 100-150 words per minute. The average length of each recording is 5 to 6 seconds, approximately 28 hours in total. The train, test and validation split ratio is 75 : 15 : 10. Notably, the audio guidance is not in terms of sounds of the target objects, but rather audio recordings of text descriptors.


\section{Summary}
We summarize various categories of video segmentation tasks in Table~\ref{tab:dense_perception_tasks}. \textcolor{red}{Add a table for performance on various datasets.}


\begin{table}[t]%{r}{0.4\textwidth}
    \centering
    \begin{adjustbox}{width=0.98\textwidth}
    \begin{tabular}{c|c|c|c|c|c}
        \toprule
        Category & Task & Target & Instances & Tracking & Datasets \\    
        \midrule
        \multirow{4}{*}{Objects} & Automatic VOS, AVOS & Primary moving object & - & - & DAVIS'2016~\cite{perazzi2016benchmark}, MoCA~\cite{lamdouar2020betrayed}, YouTube-VOS~\cite{xu2018youtube}, YouTube-Objects~\cite{prest2012learning} \\   
             & Semi-automatic VOS, SVOS & Mask-guided object & - & - & DAVIS'2017~\cite{pont20172017,caelles20182018} \\    
             & Interactive VOS, IVOS & Scribble-guided object & - & - &  DAVIS'2017~\cite{pont20172017,caelles20182018} \\    
             & Video Instance Segmentation, VIS & All Objects & \checkmark & \checkmark & YouTube-VIS~\cite{yang2019video}, OVIS~\cite{qi2022occluded} \\    
        \midrule
        Actor-Action & Actor-Action Segmentation & Primary Object related to actions & - & - & A2D~\cite{xu2015can} \\
        \midrule
        \multirow{4}{*}{Scene} & Video Semantic Segmentation/video Scene Parsing, VSS/VSP & All things and stuff  &  - & - & VIPER~\cite{richter2017playing}, VSPW~\cite{miao2021vspw} \\   
             & Video Panoptic Segmentation, VPS & All things and stuff  & \checkmark & \checkmark &  Cityscapes-VPS~\cite{kim2020video},VIPER~\cite{richter2017playing},VIPSeg~\cite{miao2022large} \\
             & Depth-aware Video Panoptic Segmentation, DVPS & All things and stuff  and depth & \checkmark & \checkmark & Cityscapes-DVPS~\cite{qiao2021vip}, SemanticKITTI-DVPS~\cite{qiao2021vip}  \\
             & Panoramic Video Panoptic Segmentation, PVPS & All things and stuff  & \checkmark & \checkmark & WOD:PVPS~\cite{mei2022waymo} \\ 
        \midrule
         \multirow{2}{*}{Multi-modal} & Text-Guided-VOS/Referring-VOS, RVOS & Text reference guided object &  - & - & A2D-Sentence~\cite{gavrilyuk2018actor}, RE-DAVIS~\cite{khoreva2019video}, RVOS~\cite{seo2020urvos} \\  
             & Audio-Guided-VOS, AGVOS & Audio reference guided object & - & - & AVOS~\cite{pan2022wnet} \\           
        \bottomrule
      \end{tabular}
    \end{adjustbox}
    \caption{\scriptsize{Summary of Video Segmentation Tasks.}}
    \label{tab:dense_perception_tasks}
\end{table}


\iffalse
\section{Multi-task Learning}
Since all of the above dense video understanding tasks require a representation of the qualitative properties of pixels, some recent efforts have worked towards unified model for all the tasks. 
TubeFormer-DeepLab~\cite{kim2022tubeformer} presented a mask transformer based approach for a unified general solution to Video Semantic Segmentation (VSS), Video Instance Segmentation (VIS), and Video Panoptic Segmentation (VPS). They formulated the problem as partitioning video a video clip into class-labeled tubes.
\fi 

\pagebreak


==> BODY/ch03_notes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Model Overview

Transformer-based models have been proposed for video segmentation tasks. These models combine Transformers and convolutional neural networks (CNNs) to extract global contexts and enhance finer details by recovering localized spatial information 1.

One such model is TransVOS, which introduces a vision transformer to fully exploit and model both the temporal and spatial relationships 2. Another model is SeqFormer, which follows the principle of vision transformer that models instance relationships among video frames 3.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Position Embedding
------------------------------------------
Positional encoding is a technique used in transformer-based models to encode the position of elements in a sequence. It enables valuable supervision for dependency modeling between elements at different positions of the sequence 1. This is important because the transformer model does not use recurrence or convolution and treats each data point as independent of the other 2.

There are various methods to integrate positional information into the learning process of transformer-based language models. One such method is Rotary Position Embedding (RoPE) which encodes the absolute position with a rotation matrix and incorporates the explicit relative position dependency in self-attention formulation 1.

Would you like more information on this topic?

Received message. Positional encoding is a technique used in transformer-based models to encode the position of elements in a sequence. It enables valuable supervision for dependency modeling between elements at different positions of the sequence . This is important because the transformer model does not use recurrence or convolution and treats each data point as independent of the other . There are various methods to integrate positional information into the learning process of transformer-based language models. One such method is Rotary Position Embedding (RoPE) which encodes the absolute position with a rotation matrix and incorporates the explicit relative position dependency in self-attention formulation . Would you like more information on this topic?
Learn more:






==> Figures/ch02task/tasks.tex <==

\begin{tikzpicture}[every pin/.append style={text width=16em},
    every pin edge/.style={draw},node distance=5em]
\begin{scope}[local bounding box=bb]
\setlist{topsep=0em,itemsep=0.2ex}
 \node[pin=below:{\begin{itemize}
  \item[~] Syntax
 \end{itemize}}](COP){COP};
 \node[right=of COP,pin=below:{\begin{itemize}
  \item[~] Syntax
  \item[+] Normal
 \end{itemize}}](PAR){PAR};
 \node[right=of PAR,pin=below:{\begin{itemize}
  \item[~] Syntax
  \item[+] Normal
  \item[+] obc
 \end{itemize}}](LOT){LOT};
\end{scope}
\draw[thick,-stealth] 
 ([yshift=1em]bb.north west) node[above right]{$-$}
 -- ([yshift=1em]bb.north east) node[above left,align=center]{Change\\ $+$};
\end{tikzpicture}

